Fast Verification of Strong Database Isolation (Extended Version)

Strong isolation guarantees, such as serializability and snapshot isolation, are essential for maintaining data consistency and integrity in modern databases. Verifying whether a database upholds its claimed guarantees is increasingly critical, as these guarantees form a contract between the vendor and its users. However, this task is challenging, particularly in black-box settings, where only observable system behavior is available and often involves uncertain dependencies between transactions. In this paper, we present VeriStrong, a fast verifier for strong database isolation. At its core is a novel formalism called hyper-polygraphs, which compactly captures both certain and uncertain transactional dependencies in database executions. Leveraging this formalism, we develop sound and complete encodings for verifying both serializability and snapshot isolation. To achieve high efficiency, VeriStrong tailors SMT solving to the characteristics of database workloads, in contrast to prior general-purpose approaches. Our extensive evaluation across diverse benchmarks shows that VeriStrong not only significantly outperforms state-of-the-art verifiers on the workloads they support, but also scales to large, general workloads beyond their reach, while maintaining high accuracy in detecting isolation anomalies.

==> algs/consistency-check.tex <==
\begin{algorithm}
  \caption{Detect cycle} 
  \label{algo:consistency-check}
  \begin{algorithmic}[1]
    \State{\zhiheng{seems unnecessary, merge it into alg2?; now merged}}
    \Function{DetectCycle }{$\cedges$}
      \If{$\eug \cup \cedges$ is cyclic} \Comment{use PK algorithm}
        \State{\Return \true}
      \Else
        \State{$\eug \gets \eug \cup \cedges$}
        \State{\Return \false}
      \EndIf
    \EndFunction
  \end{algorithmic}
\end{algorithm}

==> algs/exactly-one-encoding-theory-propagation.tex <==
\begin{algorithm}
  \footnotesize
  \caption{Theory Propagate}
  \label{algo:theory-propagate}
  \begin{algorithmic}[1]
    \Function{TheoryPropagate }{$\pa$}
      \ForAll{$\cwrvar{x}_{T, S} \in \pa$ for some $x, T$ and $S$}
        \State{$\pa \gets \pa \cup 
                \set{\lnot \cwrvar{x}_{T', S} \mid 
                     \exists \ccons \in \wrcons.\;T' \rel{\WR(x)} S \in \ccons 
                \land T \neq T' \land \cwrvar{x}_{T', S} \text{ is unassigned}}$}
      \EndFor
      \State{\Return $\pa$}
    \EndFunction
  \end{algorithmic}
\end{algorithm}

==> algs/monosat-solver.tex <==
\begin{algorithm}[t]
  \caption{Solving Process of MonoSAT \nobi{(i) can you highlight the two bottlenecks in the pseudo code? (ii) to save space, also for better presentation, is that possible to construct the pseudo code in a way that our optimizations can be placed ``side by side"? } \zhiheng{(i) \yes (ii) todo later if we decided to put this pseudo code}}
  \label{algo:monosat-solver}
  \begin{algorithmic}[1]
    \Function{SATSearch}{Variables $\cvars$, SAT Constraints $\cclauses$}
      \State{$\pa_{total} \gets \set{}$}
      \While{$\cardinality{\pa_{total}} \neq \cardinality{\cvars}$}
        \State{$\clit \gets $ \Call{PickNewDecisionChoice}{$\pa_{total}$}}
        \State{\textcolor{red}{$\pa \gets $ \Call{Propagate}{$\clit$}}}
        \State{$(ret, \cconflictcl) \gets $ \Call{TheorySolverMain}{$\pa$}} 
        \If{$ret = \true$}
          \State{$\pa_{total} \gets \pa_{total} \cup \pa$}
        \Else
          \If{$\lnot$ \Call{ResolveConflict}{$\cconflictcl$}}
            \State{\Return $\false$} 
          \Else
            \State{$\pa_{total} \gets $ \Call{BackTrack}{$\pa_{total}$}} 
          \EndIf
        \EndIf
      \EndWhile
      \State{\Return $\true$}
    \EndFunction

    \Function{TheorySolverMain}{Partial Assignment $\pa$} 
      \State{$\cedges \gets $ \Call{BindEdges}{$\pa$}}
      \If{\textcolor{red}{\Call{HasCycle}{$\ug, \cedges$}}} \Comment{PK Topological Algorithm}
        \State{\Return $(\true, \_)$} 
      \Else
        \State{\Return $(\false, $ \Call{GenConflictClause}{$\ug, \cedges$} $)$} 
      \EndIf
    \EndFunction
  \end{algorithmic}
\end{algorithm}

==> algs/overall.tex <==
% overall.tex

\begin{algorithm}[t]
  \footnotesize
  \caption{Overview of \ourtool}
  \label{alg:overall}
  \begin{algorithmic}[1]
    \Function{VerifySER}{$\H$} \Comment{\small $\H$: the history}
      \label{procedure:checkser}
      \State $\G \gets \Call{Construct}{\H}$
        \label{line:checkser-call-construct}
        \Comment{\small see Alg.~\ref{algo:construct} in Section~\ref{section:appendix-alg} of Appendix
      \If{$\lnot \Call{Prune}{\G}$}
        \label{line:checkser-call-prune}
  \Comment{\small see Alg.~\ref{algo:fast-prune} in~\cite[Appendix C]{tech-rpt} and  Section~\ref{sss:prune-1-width-cycles}}
        \State \Return \false
      \EndIf
      \State $\formula \gets \Call{Encode}{\G}$
        \label{line:checkser-call-encode}
 \Comment{\small see Alg.~\ref{algo:encode} in~\cite[Appendix C]{tech-rpt} and  Section~\ref{sss:encode-2-width-cycles}}
        % \State \Call{EncodeCyclesOfWidth2}{$G$}
        %   \label{line:checkser-call-encode-cycles}
      \State \Return $\Call{Solve}{\formula, \G}$
        \label{line:checkser-call-solve}
        \Comment{\small Alg.~\ref{alg:overall}; Section~\ref{sec:alg}}
    \EndFunction
  \end{algorithmic}
\end{algorithm}

==> algs/prune-one-pass-backup.tex <==
\begin{algorithm}
  \caption{Pruning One Pass}
  \begin{algorithmic}[1]
    \Function{PruneOnePass}{Known Graph $\mathcal{KG}$, Constraints $\mathcal{C}$}
      \State{$changed \gets$ \false}
      \State{$reachability \gets$ \Call{Reachability} {$\mathcal{KG}$}}
      \ForAll{$cons \gets \langle either, or\rangle \in \mathcal{C}$}
        \State{$add\_either \gets$ \Call{CycleDetection} {$reachability, or$}}
        \State{$add\_or \gets$ \Call{CycleDetection} {$reachability, either$}}
        \If{$add\_either \land add\_or$}
          \Return$false$ % \Comment {conflict found in pruning}
        \ElsIf{$add\_either$}
          \State{$changed$ $\gets$ \true}
          \State{$\mathcal{C}$ $\gets$ $\mathcal{C} \setminus \{cons\}$}
          \State{$E_{\mathcal{KG}}$ $\gets$ $E_{\mathcal{KG}} \cup either$}
        \ElsIf {$add\_or$}
          \State{$changed$ $\gets$ \true}
          \State{$\mathcal{C}$ $\gets$ $\mathcal{C} \setminus \{cons\}$}
          \State{$E_{\mathcal{KG}}$ $\gets$ $E_{\mathcal{KG}} \cup or$}
        \EndIf
      \EndFor
      \Return $changed$
    \EndFunction

    \Function{CycleDetection} {$reachability, edges$}
    \ForAll{$(from, to)$ $\in$ $edges$}
      \If{$(to, from) \in reachability$}
        \Return \true
      \EndIf
    \EndFor
    \Return \false
  \EndFunction
  \end{algorithmic}
\end{algorithm}

==> algs/prune-one-pass.tex <==
\begin{algorithm}
  \caption{Prune One Pass}
  \label{algo:one-pass-pruning}
  \begin{algorithmic}[1]
    \Function{PruneOnePass}{\null}
      \State $\caccept \gets \true,\; \cchanged \gets \false$
      \State $\creachability \gets $ \Call{Reachability}{\null}

      \ForAll{$cons \in \wwcons$}
        \State{$cons \gets \set{\chvar \mid \chvar \in cons \land \lnot \Call{CycleDetection}{\chvar}}$ }
        \If{$cons = \emptyset$}
          \State{$\caccept \gets \false$}
          \State{\textbf{break}}
        \EndIf
        \If {$\cardinality{cons} = 1$}
          \State{$\set{\chvar} \gets cons$}
          \State{\Call{AddEdges }{$\chvar$}}
          \State{$\wwcons \gets \wwcons \setminus \set{cons}$}
          \State{$\cchanged \gets \true$}
        \EndIf
      \EndFor

      \ForAll{$cons \in \wrcons$}
        \State{$\cdots$} \Comment{enumerate constraints in $\wrcons$, similar to $\wwcons$}
      \EndFor

      \State{\Return $(\caccept,\; \cchanged)$}
    \EndFunction

    \Function{CycleDetection}{$\creachability, (T, S, L, K)$}
      \State{$edges \gets $ \Call{RWComplete }{$(T, S, L, K)$}}
      \ForAll{$(x, y, \_, \_) \in edges$}
        \If{$(y, x) \in \creachability$}
          \State{\Return \true}
        \EndIf
      \EndFor
      \State{\Return \false}
    \EndFunction

    \Function{AddEdges }{$(T, S, L, K)$}
      \State{$\cedges \gets $ \Call{RWComplete }{$(T, S, L, K)$}}
      \State{$\E \gets \E \cup \cedges$}
    \EndFunction

    \Function{RWComplete}{$(T, S, L, K)$}
      \State{$\cedges \gets \set{(T, S, L, K)}$}
      \If{$L = \wwlabel$}
        \ForAll{$(T, R, \wrlabel, K') \in \E$}
          \If{$K \cap K' \neq \emptyset$}
            \State{$\cedges \gets \cedges \cup \set{(R, S, \rwlabel, K \cap K')}$}
          \EndIf
        \EndFor
      \ElsIf{$L = \wrlabel$}
        \State{$\cdots$} \Comment{enumerate known edges typed $\WW$ and derive $\RW$ edges,
          similar to the $L = \wwlabel$ case}
        % \ForAll{$(T, R, \wwlabel, K') \in \E$}
        %   \If{$K \cap K' \neq \emptyset$}
        %     \State{$\cedges \gets \cedges \cup \set{(S, R, \rwlabel, K \cap K')}$}
        %   \EndIf
        % \EndFor
      \EndIf
      \State{\Return $\cedges$}
    \EndFunction
  \end{algorithmic}
\end{algorithm}

==> algs/prune.tex <==
\begin{algorithm}
  \caption{约束剪枝}
  \label{algo:prune}
  \begin{algorithmic}[1]
    \Function{Prune}{Known Graph $\cknowngraph$, Constraints $\C$}
      \State{$\caccept \gets \true, \cchanged \gets \true$}
      \While{$\cchanged$}
        \State{$(\caccept, \cchanged) \gets$ \Call{PruneOnePass}{$\cknowngraph, \C$}}
        \If{$\lnot \caccept$}
          \State{\textbf{break}}
        \EndIf
      \EndWhile
      \State{\Return $\caccept$}
    \EndFunction
  \end{algorithmic}
\end{algorithm}

==> algs/solver-init.tex <==
\begin{algorithm}
  \caption{Initialize theory solver}
  \label{algo:solver-init}
  \begin{algorithmic}[1]
    \Function{InitTheorySolver }{$\V, \E$}
      \State{$\vug \gets \V$} \Comment{$\T$}
      \ForAll{$T \rel{\typevar(x)} S \in \E$}
        \State{$\eug \gets \eug \cup \set{T \rel{\true} S}$}
      \EndFor
    \EndFunction
  \end{algorithmic}
\end{algorithm}

==> figs/algs/ser-mono-framework.tex <==
% ser-mono-framework.tex

\begin{figure}[t]
	\centering
	\includegraphics[width = 0.95\columnwidth]{figs/isolation-mono-framework-2.pdf}
	\caption{Workflow of MonoSAT Checking.}
	\label{fig:ser-monosat-framework}
\end{figure}

==> figs/cycle-width/cycle-width-minimal.tex <==
% cycle-width-minimal.tex

\pgfplotsset{height=140pt, width=240pt}
\pgfplotsset{tick style={draw=none}}
\begin{figure}[t]
	\centering
	\resizebox{0.40\textwidth}{!}{
	\begin{scaletikzpicturetowidth}{0.46\textwidth}
		\begin{tikzpicture}[scale=\tikzscale]
			\begin{axis}[
				% title={C-Twitter 10K},
				xlabel={width},
				ylabel={proportion \%},
							xlabel near ticks,
							ylabel near ticks,
        ymax=100,
				ytick={10,20,30,40,50,75,100},
				xtick={1,2,3,4,5,6,7,8,9,10,15,20},
				legend pos=north east,
				legend style={draw=none}
				]
				\addplot[color=teal,mark=o,mark size=2pt] table [x=param, y=gtpcc, col sep=comma] {figs/cycle-width/data/minimized-data.csv};
				\addplot[color=blue,mark=square,mark size=2pt] table [x=param, y=gtwitter, col sep=comma] {figs/cycle-width/data/minimized-data.csv};
				\addplot[color=green!50!black,mark=triangle,mark size=2pt] table [x=param, y=grubis, col sep=comma] {figs/cycle-width/data/minimized-data.csv};
				\addplot[color=red!65!black,mark=diamond,mark size=2pt] table [x=param, y=grh, col sep=comma] {figs/cycle-width/data/minimized-data.csv};
				\addplot[color=brown,mark=pentagon,mark size=2pt] table [x=param, y=grw, col sep=comma] {figs/cycle-width/data/minimized-data.csv};
				\addplot[color=orange,mark=asterisk,mark size=2pt] table [x=param, y=gwh, col sep=comma] {figs/cycle-width/data/minimized-data.csv};

				% \addplot[color=teal,mark=o,mark size=1pt] table [x=param, y=gtpcc, col sep=comma] {figs/cycle-width/data/data.csv};
				% \addplot[color=blue,mark=o,mark size=1pt] table [x=param, y=gtwitter, col sep=comma] {figs/cycle-width/data/data.csv};
				% \addplot[color=green!50!black,mark=o,mark size=1pt] table [x=param, y=grubis, col sep=comma] {figs/cycle-width/data/data.csv};
				% \addplot[color=red!65!black,mark=o,mark size=1pt] table [x=param, y=grh, col sep=comma] {figs/cycle-width/data/data.csv};
				% \addplot[color=brown,mark=o,mark size=1pt] table [x=param, y=grw, col sep=comma] {figs/cycle-width/data/data.csv};
				% \addplot[color=orange,mark=o,mark size=1pt] table [x=param, y=gwh, col sep=comma] {figs/cycle-width/data/data.csv};
        \legend{\small G-TPCC, \small G-Twitter,\small G-RUBiS,\small RH,\small BL,\small WH}
      \end{axis}
		\end{tikzpicture}
	\end{scaletikzpicturetowidth}
	}
	        		\captionsetup{skip=0pt}
  \caption{Distribution of minimal cycle widths across conflicts.}
	\label{fig:cycle-width-minimal}
\end{figure}

==> figs/cycle-width/cycle-width.tex <==
% cycle-width.tex

\pgfplotsset{height=140pt, width=240pt}
\begin{figure}[t]
	\centering
	\resizebox{0.40\textwidth}{!}{
	\begin{scaletikzpicturetowidth}{0.46\textwidth}
		\begin{tikzpicture}[scale=\tikzscale]
			\begin{axis}[
				% title={C-Twitter 10K},
				xlabel={cycle width},
				ylabel={propability \%},
        ymax=100,
				ytick={10,20,30,40,50,100},
				xtick={1,2,3,4,5,6,7,8,9,10,15,20},
				legend pos=north east,
				]
				% \addplot[color=teal,mark=o,mark size=1pt] table [x=param, y=gtpcc, col sep=comma] {figs/cycle-width/data/minimized-data.csv};
				% \addplot[color=blue,mark=o,mark size=1pt] table [x=param, y=gtwitter, col sep=comma] {figs/cycle-width/data/minimized-data.csv};
				% \addplot[color=green!50!black,mark=o,mark size=1pt] table [x=param, y=grubis, col sep=comma] {figs/cycle-width/data/minimized-data.csv};
				% \addplot[color=red!65!black,mark=o,mark size=1pt] table [x=param, y=grh, col sep=comma] {figs/cycle-width/data/minimized-data.csv};
				% \addplot[color=brown,mark=o,mark size=1pt] table [x=param, y=grw, col sep=comma] {figs/cycle-width/data/minimized-data.csv};
				% \addplot[color=orange,mark=o,mark size=1pt] table [x=param, y=gwh, col sep=comma] {figs/cycle-width/data/minimized-data.csv};

				\addplot[color=teal,mark=o,mark size=1pt] table [x=param, y=gtpcc, col sep=comma] {figs/cycle-width/data/data.csv};
				\addplot[color=blue,mark=o,mark size=1pt] table [x=param, y=gtwitter, col sep=comma] {figs/cycle-width/data/data.csv};
				\addplot[color=green!50!black,mark=o,mark size=1pt] table [x=param, y=grubis, col sep=comma] {figs/cycle-width/data/data.csv};
				\addplot[color=red!65!black,mark=o,mark size=1pt] table [x=param, y=grh, col sep=comma] {figs/cycle-width/data/data.csv};
				\addplot[color=brown,mark=o,mark size=1pt] table [x=param, y=grw, col sep=comma] {figs/cycle-width/data/data.csv};
				\addplot[color=orange,mark=o,mark size=1pt] table [x=param, y=gwh, col sep=comma] {figs/cycle-width/data/data.csv};
        \legend{G-TPCC,G-Twitter,G-RUBiS,GeneralRH,GeneralRW,GeneralWH}
      \end{axis}
		\end{tikzpicture}
    \hspace{1ex}
	\end{scaletikzpicturetowidth}
	}
	
  \caption{Discrete Distribution of Cycle Counts by Width.}
	\label{fig:cycle-width}
\end{figure}


==> figs/eval/ablation/ablation.tex <==

% ablation order I, O2 -> O1
% \begin{figure*}[t]
%   \centering
%   \begin{scaletikzpicturetowidth}{0.96\textwidth}
%     \begin{tikzpicture}[scale=\tikzscale]
%       \begin{axis}[
%         % title={Differencial Analysis, \#txns/session=15, \#keys=1000},
%         width=15cm,
%         height=6cm,
%         % xlabel={},
%           % legend style={at={(0.02, 0.7)}, anchor=west, nodes={scale=0.8, transform shape}},
%           legend style={at={(1.02, 0.8)}, anchor=west},
%         x tick style={draw=none},
%         % x tick label style={rotate=20, anchor=north east, yshift=0.5ex},
%         scale only axis,
%         ylabel={Time (s) in log scale},
%         % ymax=12000,
%         ybar,
%         log origin=infty,
%         ymin=0.1,
%         ymode=log,
%         bar width=4,
%         area legend,
%         xtick=data,
%         xtick distance=5,
%         xticklabels={G-TPCC,G-Twitter,G-RUBiS,GeneralRH,GeneralRW,GeneralWH,GeneralRV}
%         ]
%         \addplot[color=ps6green, pattern color=ps6green, pattern=crosshatch] table [x expr=\coordindex, y=ours, col sep=comma] {figs/eval/ablation/data.csv};
%         \addplot[color=ps5green, pattern color=ps5green, pattern=crosshatch] table [x expr=\coordindex, y=o23, col sep=comma] {figs/eval/ablation/data.csv};
%         \addplot[color=ps4green, pattern color=ps4green, pattern=crosshatch] table [x expr=\coordindex, y=o22, col sep=comma] {figs/eval/ablation/data.csv};
%         \addplot[color=ps3green, pattern color=ps3green, pattern=crosshatch] table [x expr=\coordindex, y=o21, col sep=comma] {figs/eval/ablation/data.csv};
%         \addplot[color=ps2green, pattern color=ps2green, pattern=crosshatch] table [x expr=\coordindex, y=o12, col sep=comma] {figs/eval/ablation/data.csv};
%         \addplot[color=ps1green, pattern color=ps1green, pattern=crosshatch] table [x expr=\coordindex, y=o11, col sep=comma] {figs/eval/ablation/data.csv};
%         \legend{
%           \ourtool, 
%           \ourtool w/o H, 
%           \ourtool w/o CH,
%           \ourtool w/o O2(PCH) ,
%           \ourtool w/o O2 and T,
%           \ourtool w/o O2 and O1(RT),
%         }
%       \end{axis}
%     \end{tikzpicture}
%   \end{scaletikzpicturetowidth}
%   \caption{Ablation Study of \ourtool's optimization steps.
%   O1 and O2 represent our optimization clue I and II.
%   O1 = R(Reducing encoding space) + T(Theory propagation).
%   O2 = P(Pruning) + C(preComputing 2-witdh cycles) + H(Heuristical polarity selecting)}
%   \label{fig:ablation}
% \end{figure*}


% ablation order II: O1 -> O2
% \begin{figure*}[t]
%   \centering
%   \begin{scaletikzpicturetowidth}{0.96\textwidth}
%     \begin{tikzpicture}[scale=\tikzscale]
%       \begin{axis}[
%         % title={Differencial Analysis, \#txns/session=15, \#keys=1000},
%         width=15cm,
%         height=6cm,
%         % xlabel={},
%           % legend style={at={(0.02, 0.7)}, anchor=west, nodes={scale=0.8, transform shape}},
%         legend style={at={(1.02, 0.68)}, anchor=west},
%         x tick style={draw=none},
%         % x tick label style={rotate=20, anchor=north east, yshift=0.5ex},
%         ytick={0.1,1,10,100,1000,5000},
%         yticklabels={$0$,$1$,$10$,$100$,$1000$,$5000$}, % 定义刻度上的标签
%         scale only axis,
%         ylabel={Time (s) in log scale},
%         ymax=10000,
%         ybar,
%         log origin=infty,
%         ymin=0.1,
%         ymode=log,
%         bar width=4,
%         area legend,
%         xtick=data,
%         xtick distance=5,
%         xticklabels={G-TPCC,G-Twitter,G-RUBiS,GeneralRH,GeneralRW,GeneralWH,GeneralRV}
%         ]
%         \addplot[color=ps6green, pattern color=ps6green, pattern=crosshatch] table [x expr=\coordindex, y=ours, col sep=comma] {figs/eval/ablation/data2.csv};
%         \addplot[color=ps5green, pattern color=ps5green, pattern=crosshatch] table [x expr=\coordindex, y=o12, col sep=comma] {figs/eval/ablation/data2.csv};
%         \addplot[color=ps4green, pattern color=ps4green, pattern=crosshatch] table [x expr=\coordindex, y=o11, col sep=comma] {figs/eval/ablation/data2.csv};
%         \addplot[color=ps3green, pattern color=ps3green, pattern=crosshatch] table [x expr=\coordindex, y=o23, col sep=comma] {figs/eval/ablation/data2.csv};
%         \addplot[color=ps2green, pattern color=ps2green, pattern=crosshatch] table [x expr=\coordindex, y=o22, col sep=comma] {figs/eval/ablation/data2.csv};
%         \addplot[color=ps1green, pattern color=ps1green, pattern=crosshatch] table [x expr=\coordindex, y=o21, col sep=comma] {figs/eval/ablation/data2.csv};

%         \legend{
%           \ourtool, 
%           \ourtool w/o T, 
%           \ourtool w/o O1(TR),
%           \ourtool w/o O1 and H ,
%           \ourtool w/o O1 and HC,
%           \ourtool w/o O1 and O2(HCP),
%         }
%       \end{axis}
%     \end{tikzpicture}
%   \end{scaletikzpicturetowidth}
%   \caption{Ablation Study of \ourtool's optimization steps.
%   O1 and O2 represent our optimization clue I and II.
%   O1 = R(Removing $\uniqueencodings$) + T(Theory propagation).
%   O2 = P(Pruning) + C(preComputing 2-witdh cycles) + H(Heuristical polarity selecting)}
%   \label{fig:ablation}
% \end{figure*}


\begin{figure}[t]
  \centering
  \begin{scaletikzpicturetowidth}{0.48\textwidth}
    \begin{tikzpicture}[scale=\tikzscale]
      \begin{axis}[
        % title={Differencial Analysis, \#txns/session=15, \#keys=1000},
        width=15cm,
        height=6cm,
        % xlabel={},
          % legend style={at={(0.02, 0.7)}, anchor=west, nodes={scale=0.8, transform shape}},
        legend style={at={(0.02, 0.98)}, anchor=north west},
        x tick style={draw=none},
        % x tick label style={rotate=20, anchor=north east, yshift=0.5ex},
        ytick={0.1,1,10,100,1000,10000},
        yticklabels={$0$,$1$,$10$,$100$,$1000$,$10000$}, % 定义刻度上的标签
        scale only axis,
        ylabel={Time (s) in log scale},
        ymax=100000,
        ybar,
        log origin=infty,
        ymin=0.1,
        ymode=log,
        bar width=8,
        % bar shift=3,
        area legend,
        xtick=data,
        xtick distance=3,
        xticklabels={G-TPCC,G-Twitter,G-RUBiS,GeneralRH,GeneralRW,GeneralWH,GeneralRV},
        % nodes near coords={
        % \pgfmathprintnumber{\rawy} % Change this line
        %   \pgfmathparse{int(\rawy)}
        %   \ifnum\pgfmathresult=10000
        %     TO
        %   \else
        %     \pgfmathprintnumber{\rawy}
        %   \fi
        % },
        % nodes near coords align={vertical}, % 垂直对齐数值标签
        % nodes near coords style={rotate=90, anchor=west}, % 旋转90度并调整锚点
        % point meta=explicit symbolic, % 使用显式的符号元数据
        % visualization depends on={value \thisrow{wo-o1-o2} \as \rawy} % 获取原始的y值   
        ]
        % \addplot[color=ps6green, pattern color=ps6green, pattern=crosshatch] table [x expr=\coordindex, y=ours, col sep=comma] {figs/eval/ablation/data3.csv};
        % \addplot[color=ps4green, pattern color=ps4green, pattern=crosshatch] table [x expr=\coordindex, y=wo-o2, col sep=comma] {figs/eval/ablation/data3.csv};
        % \addplot[color=ps2green, pattern color=ps2green, pattern=crosshatch] table [x expr=\coordindex, y=wo-o1-o2, col sep=comma] {figs/eval/ablation/data3.csv};

        \addplot+[
          color=ps6green, 
          pattern color=ps6green, 
          pattern=crosshatch,
          point meta=explicit symbolic,
          visualization depends on={value \thisrow{ours} \as \rawy},
          nodes near coords={
            \pgfmathparse{int(\rawy)}
            \ifnum\pgfmathresult=10000
              TO
            \else
              \pgfmathprintnumber{\rawy}
            \fi
          },
          nodes near coords align={vertical},
          nodes near coords style={rotate=90, anchor=west}
        ] table [x expr=\coordindex, y=ours, col sep=comma] {figs/eval/ablation/data3.csv};

        \addplot+[
          color=ps4green, 
          pattern color=ps4green, 
          pattern=crosshatch,
          point meta=explicit symbolic,
          visualization depends on={value \thisrow{wo-o2} \as \rawy},
          nodes near coords={
            \pgfmathparse{int(\rawy)}
            \ifnum\pgfmathresult=10000
              TO
            \else
              \pgfmathprintnumber{\rawy}
            \fi
          },
          nodes near coords align={vertical},
          nodes near coords style={rotate=90, anchor=west}
        ] table [x expr=\coordindex, y=wo-o2, col sep=comma] {figs/eval/ablation/data3.csv};

        \addplot+[
          color=ps2green, 
          pattern color=ps2green, 
          pattern=crosshatch,
          point meta=explicit symbolic,
          visualization depends on={value \thisrow{wo-o1-o2} \as \rawy},
          nodes near coords={
            \pgfmathparse{int(\rawy)}
            \ifnum\pgfmathresult=10000
              TO
            \else
              \pgfmathprintnumber{\rawy}
            \fi
          },
          nodes near coords align={vertical},
          nodes near coords style={rotate=90, anchor=west}
        ] table [x expr=\coordindex, y=wo-o1-o2, col sep=comma] {figs/eval/ablation/data3.csv};
                    
        \legend{
          \ourtool, 
          \ourtool w/o O2,
          \ourtool w/o O1 and O2
        }
      \end{axis}
    \end{tikzpicture}
  \end{scaletikzpicturetowidth}
  \caption{Ablation Study of \ourtool's optimization steps.
  O1 and O2 represent our optimization I and II.
  TO = $10^4$ s.}
  \label{fig:ablation}
\end{figure}


==> figs/eval/encode-cycle-width/encode-cycle-width-each.tex <==
% encode-cycle-width-each.tex

\pgfplotsset{height=140pt, width=100pt}
\begin{figure}[h]
  \begin{scaletikzpicturetowidth}{0.4\columnwidth}
		\begin{tikzpicture}[scale=\tikzscale]
			\begin{axis}[
				title={},
				xlabel={$w$},
				ylabel={Time (s)},
				ymax=1000,
        ymode=log,
        xtick={1,2,3,4},
				cycle multiindex* list={
								color       \nextlist
								mark list*  \nextlist
						},
        legend style={
          at={(1.05,0.98)}, % 调整图例的横纵坐标
          anchor=north west, % 锚点设为西南方向
          % 也可以添加其他样式，比如背景颜色等
          column sep=1ex,
          legend columns=1 % 可以选择是否需要单列或多列
        },
				]
				\addplot[color=blue,mark=o,mark size=3pt] table [x=param, y=grubis, col sep=comma] {figs/eval/encode-cycle-width/runtime-each.csv};
				\addplot[color=brown,mark=square,mark size=3pt] table [x=param, y=gtwitter, col sep=comma] {figs/eval/encode-cycle-width/runtime-each.csv};
				\addplot[color=violet,mark=triangle,mark size=3pt] table [x=param, y=grh, col sep=comma] {figs/eval/encode-cycle-width/runtime-each.csv};
				\addplot[color=green!50!black,mark=diamond,mark size=3pt] table [x=param, y=grw, col sep=comma] {figs/eval/encode-cycle-width/runtime-each.csv};
				\addplot[color=teal,mark=pentagon,mark size=3pt] table [x=param, y=gwh, col sep=comma] {figs/eval/encode-cycle-width/runtime-each.csv};
				\addplot[color=orange,mark=asterisk,mark size=3pt] table [x=param, y=gdv, col sep=comma] {figs/eval/encode-cycle-width/runtime-each.csv};
        
				\addplot[color=teal,mark=pentagon*,mark size=3pt] (3,600);
				\addplot[color=green!50!black,mark=diamond*,mark size=3pt] (3,600);
				\addplot[color=orange,mark=10-pointed star,mark size=3pt] (3,600);
				
        \addplot[color=brown,mark=square*,mark size=3pt] (4,600);
				\addplot[color=blue,mark=*,mark size=3pt] (4,600);

				\legend{G-RBUiS, G-Twitter, GeneralRH, GeneralRW, GeneralWH, GeneralDV}
			\end{axis}
		\end{tikzpicture}

		% \begin{tikzpicture}[scale=\tikzscale]
		% 	\begin{axis}[
		% 		title={},
		% 		width=9cm,
		% 		height=6cm,
		% 		xlabel={$w$},
		% 		ylabel={Time (s)},
		% 		ymax=1000,
    %     % ymode=log,
    %     xtick={1,2,3,4},
		% 		xticklabels={1,2,3,4},
		% 		ybar, % 添加 ybar 样式来画柱状图
   	% 		bar width=4pt, % 控制柱的宽度
    % 		% enlarge x limits=0.15, % 增加x轴两端的留白
		% 		cycle multiindex* list={
		% 						color       \nextlist
		% 						mark list*  \nextlist
		% 				},
		% 		area legend,
    %     legend style={
    %       at={(1.05,0.98)}, % 调整图例的横纵坐标
    %       anchor=north west, % 锚点设为西南方向
    %       % 也可以添加其他样式，比如背景颜色等
    %       column sep=1ex,
    %       legend columns=1 % 可以选择是否需要单列或多列
    %     },
		% 		]
		% 		\addplot[color=blue] table [x=x, y=grubis, col sep=comma] {figs/eval/encode-cycle-width/runtime-each.csv};
		% 		\addplot[color=brown] table [x=x, y=gtwitter, col sep=comma] {figs/eval/encode-cycle-width/runtime-each.csv};
		% 		\addplot[color=violet] table [x=x, y=grh, col sep=comma] {figs/eval/encode-cycle-width/runtime-each.csv};
		% 		\addplot[color=green!50!black] table [x=x, y=grw, col sep=comma] {figs/eval/encode-cycle-width/runtime-each.csv};
		% 		\addplot[color=teal] table [x=x, y=gwh, col sep=comma] {figs/eval/encode-cycle-width/runtime-each.csv};
		% 		\addplot[color=orange] table [x=x, y=gdv, col sep=comma] {figs/eval/encode-cycle-width/runtime-each.csv};
				
		% 		\legend{G-RBUiS, G-Twitter, GeneralRH, GeneralRW, GeneralWH, GeneralDV}
		% 	\end{axis}
		% \end{tikzpicture}
		\hspace{1ex}
	\end{scaletikzpicturetowidth}

  \caption{Encoding time of different cycle width $w$}
	\label{fig:encode-cycle-width}
\end{figure}

==> figs/eval/encode-cycle-width/encode-cycle-width.tex <==
% encode-cycle-width.tex

\pgfplotsset{height=100pt, width=80pt}
\pgfplotsset{tick style={draw=none}}
\begin{wrapfigure}{right}{4.1cm}
	\vspace{-3ex}
%\begin{figure}
  \begin{scaletikzpicturetowidth}{0.23\textwidth}
		\begin{tikzpicture}[scale=\tikzscale]
			\begin{axis}[
				tick label style={font=\scriptsize},  
				title={},
				xlabel={\scriptsize $w$},
				ylabel={\scriptsize Time (s)},
				ymax=1000,
        ymode=log,
        				ylabel near ticks,
        				xlabel near ticks,
        xtick={1,2,3,4},
				cycle multiindex* list={
								color       \nextlist
								mark list*  \nextlist
						},
        legend style={
        draw=none,
        font={\tiny},
        legend image post style={scale=0.8},
          at={(1.1,1)}, % 调整图例的横纵坐标
          anchor=north west, % 锚点设为西南方向
          % 也可以添加其他样式，比如背景颜色等
          %column sep=.5ex,
          legend columns=1 % 可以选择是否需要单列或多列
        },
				]
				\addplot[color=blue,mark=o,mark size=2pt] table [x=param, y=grubis, col sep=comma] {figs/eval/encode-cycle-width/runtime-large-to.csv};
				\addplot[color=brown,mark=square,mark size=2pt] table [x=param, y=gtwitter, col sep=comma] {figs/eval/encode-cycle-width/runtime-large-to.csv};
				\addplot[color=violet,mark=triangle,mark size=2pt] table [x=param, y=grh, col sep=comma] {figs/eval/encode-cycle-width/runtime-large-to.csv};
				\addplot[color=green!50!black,mark=diamond,mark size=2pt] table [x=param, y=grw, col sep=comma] {figs/eval/encode-cycle-width/runtime-large-to.csv};
				\addplot[color=teal,mark=pentagon,mark size=2pt] table [x=param, y=gwh, col sep=comma] {figs/eval/encode-cycle-width/runtime-large-to.csv};
				\addplot[color=orange,mark=asterisk,mark size=2pt] table [x=param, y=gdv, col sep=comma] {figs/eval/encode-cycle-width/runtime-large-to.csv};
        
				% \addplot[color=teal,mark=pentagon*,mark size=3pt] (3,600);
				% \addplot[color=green!50!black,mark=diamond*,mark size=3pt] (3,600);
				% \addplot[color=orange,mark=10-pointed star,mark size=3pt] (3,600);
				
        % \addplot[color=brown,mark=square*,mark size=3pt] (4,600);
				% \addplot[color=blue,mark=*,mark size=3pt] (4,600);

				\legend{G-RBUiS,   G-Twitter,  RH,  RW,  WH,  HD}
			\end{axis}
		\end{tikzpicture}
	%	\hspace{1ex}
	\end{scaletikzpicturetowidth}
		\captionsetup{skip=2pt}
  \caption{Runtime of Variant (i) under varying encoded cycle widths ($w$). Timeout (600s) data points are not plotted. }
	\label{fig:encode-cycle-width}
%\end{figure}
		\vspace{-2ex}
\end{wrapfigure}

==> figs/eval/gpu-wo-pro6000/gpu.tex <==
% gpu.tex

\pgfplotsset{height=140pt, width=240pt}
\pgfplotsset{tick style={draw=none}}
\begin{figure}[h]
	\centering
	\resizebox{.5\linewidth}{!}{
%		\begin{minipage}{0.31\textwidth}
		\begin{scaletikzpicturetowidth}{\textwidth}
			\begin{tikzpicture}[scale=\tikzscale]
				\begin{axis}[
					font=\LARGE,
%					title={(a) End-to-End Checking Time},
					xlabel={\#txns},
					xtick={1000,4000,6000,8000,10000,12000,14000,16000},
					xticklabels={1k,4k,6k,8k,10k,12k,14k,16k},
					xticklabel style={/pgf/number format/fixed},
					scaled x ticks=false,
					ylabel={Time (s)},
					ymax=51,
					ytick={0,10,20,50},
					cycle multiindex* list={
									color       \nextlist
									mark list*  \nextlist
							},
						legend pos=north west,
            legend style={xshift=1pt, yshift=1pt,draw=none},
					height=170pt,
					]
					\addplot[color=blue,mark=o,mark size=3pt] table [x=param, y=ours, col sep=comma] {figs/eval/gpu/end-to-end.csv};
					% \addplot[color=brown,mark=square,mark size=3pt] table [x=param, y=cobra(w/pro6000), col sep=comma] {figs/eval/gpu/end-to-end.csv};
					\addplot[color=brown,mark=square,mark size=3pt] table [x=param, y=cobra(w/v100), col sep=comma] {figs/eval/gpu/end-to-end.csv};
					\addplot[color=magenta,mark=Mercedes star,mark size=3pt] table [x=param, y=cobra(w/h800), col sep=comma] {figs/eval/gpu/end-to-end.csv};
					\legend{\ourtool, \cobra(\textbf{V100}), \cobra(\textbf{H800})}
				\end{axis}
			\end{tikzpicture}
		\end{scaletikzpicturetowidth}
%	\end{minipage}
	
%	\begin{minipage}{0.31\textwidth}
%		\begin{scaletikzpicturetowidth}{\textwidth}
%			\begin{tikzpicture}[scale=\tikzscale]
%				\begin{axis}[
%					font=\LARGE,
%					title={(b) Avg. Time of Computing Reachability},
%					xlabel={\#txns},
%					xtick={1000,4000,6000,8000,10000,12000,14000,16000},
%					xticklabels={1k,4k,6k,8k,10k,12k,14k,16k},
%					xticklabel style={/pgf/number format/fixed},
%					scaled x ticks=false,
%					ylabel={Time (s)},
%					ymax=5,
%					% ytick={0,10,20,50,100},
%					cycle multiindex* list={
%									color       \nextlist
%									mark list*  \nextlist
%							},
%						legend pos=north west,
%            legend style={xshift=1pt, yshift=1pt,draw=none},
%					height=170pt,
%					]
%					\addplot[color=blue,mark=o,mark size=3pt] table [x=param, y=ours, col sep=comma] {figs/eval/gpu/reachability.csv};
%					% \addplot[color=brown,mark=square,mark size=3pt] table [x=param, y=cobra(w/pro6000), col sep=comma] {figs/eval/gpu/reachability.csv};
%					\addplot[color=green!50!black,mark=asterisk,mark size=3pt] table [x=param, y=cobra(w/h800), col sep=comma] {figs/eval/gpu/reachability.csv};
%					\addplot[color=violet,mark=triangle,mark size=3pt] table [x=param, y=cobra(w/v100), col sep=comma] {figs/eval/gpu/reachability.csv};
%					% \legend{\ourtool, \cobra(\textbf{PRO6000}), \cobra(\textbf{H800}), \cobra(\textbf{V100})}
%					\legend{\ourtool, \cobra(\textbf{H800}), \cobra(\textbf{V100})}
%				\end{axis}
%			\end{tikzpicture}
%		\end{scaletikzpicturetowidth}
%	\end{minipage}


	}
	\captionsetup{skip=2pt}
	\caption{Verification time: \ourtool vs Cobra with different GPU capabilities.} 
	% on the BlindW-RW dataset of 10k keys.}
	
	\label{fig:gpu}
	\vspace{-2ex}
\end{figure}


==> figs/eval/gpu/gpu.tex <==
% gpu.tex

\pgfplotsset{height=140pt, width=240pt}
\pgfplotsset{tick style={draw=none}}
\begin{figure}[h]
	\centering
	\resizebox{\linewidth}{!}{
	\begin{minipage}{0.31\textwidth}
		\begin{scaletikzpicturetowidth}{\textwidth}
			\begin{tikzpicture}[scale=\tikzscale]
				\begin{axis}[
					font=\LARGE,
					title={(a) Avg. Time of Computing Reachability},
					xlabel={\#txns},
					xtick={1000,4000,6000,8000,10000,12000,14000,16000},
					xticklabels={1k,4k,6k,8k,10k,12k,14k,16k},
					xticklabel style={/pgf/number format/fixed},
					scaled x ticks=false,
					ylabel={Time (s)},
					ymax=5,
					% ytick={0,10,20,50,100},
					cycle multiindex* list={
									color       \nextlist
									mark list*  \nextlist
							},
						legend pos=north west,
            legend style={xshift=1pt, yshift=1pt,draw=none},
					height=170pt,
					]
					\addplot[color=blue,mark=o,mark size=3pt] table [x=param, y=ours, col sep=comma] {figs/eval/gpu/reachability.csv};
					\addplot[color=brown,mark=square,mark size=3pt] table [x=param, y=cobra(w/pro6000), col sep=comma] {figs/eval/gpu/reachability.csv};
					\addplot[color=green!50!black,mark=asterisk,mark size=3pt] table [x=param, y=cobra(w/h800), col sep=comma] {figs/eval/gpu/reachability.csv};
					\addplot[color=violet,mark=triangle,mark size=3pt] table [x=param, y=cobra(w/v100), col sep=comma] {figs/eval/gpu/reachability.csv};
					\legend{\ourtool, \cobra(\textbf{PRO6000}), \cobra(\textbf{H800}), \cobra(\textbf{V100})}
				\end{axis}
			\end{tikzpicture}
		\end{scaletikzpicturetowidth}
	\end{minipage}

	\begin{minipage}{0.31\textwidth}
		\begin{scaletikzpicturetowidth}{\textwidth}
			\begin{tikzpicture}[scale=\tikzscale]
				\begin{axis}[
					font=\LARGE,
					title={(b) End-to-end Checking Time},
					xlabel={\#txns},
					xtick={1000,4000,6000,8000,10000,12000,14000,16000},
					xticklabels={1k,4k,6k,8k,10k,12k,14k,16k},
					xticklabel style={/pgf/number format/fixed},
					scaled x ticks=false,
					ylabel={Time (s)},
					ymax=51,
					ytick={0,10,20,50},
					cycle multiindex* list={
									color       \nextlist
									mark list*  \nextlist
							},
						legend pos=north west,
            legend style={xshift=1pt, yshift=1pt,draw=none},
					height=170pt,
					]
					\addplot[color=blue,mark=o,mark size=3pt] table [x=param, y=ours, col sep=comma] {figs/eval/gpu/end-to-end.csv};
					\addplot[color=brown,mark=square,mark size=3pt] table [x=param, y=cobra(w/pro6000), col sep=comma] {figs/eval/gpu/end-to-end.csv};
					\addplot[color=green!50!black,mark=asterisk,mark size=3pt] table [x=param, y=cobra(w/h800), col sep=comma] {figs/eval/gpu/end-to-end.csv};
					\addplot[color=violet,mark=triangle,mark size=3pt] table [x=param, y=cobra(w/v100), col sep=comma] {figs/eval/gpu/end-to-end.csv};
					% \legend{\ourtool, \cobra(PRO6000), \cobra(H800), \cobra(V100)}
				\end{axis}
			\end{tikzpicture}
		\end{scaletikzpicturetowidth}
	\end{minipage}
	}
	\captionsetup{skip=0pt}
	\caption{Comparison to Cobra with different GPU capabilities.} 
	% on the BlindW-RW dataset of 10k keys.}
	
	\label{fig:gpu}

\end{figure}


==> figs/eval/list-rw/list-rw.tex <==
% list-rw.tex

\pgfplotsset{height=140pt, width=240pt}

\begin{figure}[h]
	\centering
	\begin{scaletikzpicturetowidth}{0.31\textwidth}
		\begin{tikzpicture}[scale=\tikzscale]
			\begin{axis}[
				title={},
				xlabel={dup key proportion \%},
				xtick={0,0.25,0.5,0.75,1},
				xticklabels={0,25,50,75,100},
				xticklabel style={/pgf/number format/fixed},
				scaled x ticks=false,
				ylabel={Time (s)},
				ymax=3000,
        ymode=log,
				cycle multiindex* list={
					color       \nextlist
					mark list*  \nextlist
				},
				legend pos=south east,
			]
				\addplot[color=blue,mark=o,mark size=3pt] table [x=param, y=ours-rw, col sep=comma] {figs/eval/list-rw/data.csv};
				\addplot[color=brown,mark=o,mark size=3pt] table [x=param, y=ours-list, col sep=comma] {figs/eval/list-rw/data.csv};
				\addplot[color=green!50!black,mark=triangle,mark size=3pt] table [x=param, y=elle, col sep=comma] {figs/eval/list-rw/data.csv};
				% \addplot[color=violet,mark=triangle,mark size=3pt] table [x=param, y=dbcop, col sep=comma] {figs/eval/uv/runtime/ser.csv};
				\legend{\ourtool-RW,\ourtool-list,Elle}
			\end{axis}
		\end{tikzpicture}
	\end{scaletikzpicturetowidth}
  \caption{Runtime Comparison of list-append and RW-register modes in \ourtool with Elle.}
	\label{fig:list-rw}
\end{figure}


==> figs/eval/o1/o1.tex <==
% o1.tex

\pgfplotsset{height=140pt, width=240pt}

\begin{figure}[t]
	\centering
	\begin{scaletikzpicturetowidth}{0.23\textwidth}
		\begin{tikzpicture}[scale=\tikzscale]
			\begin{axis}[
				title={(a) },
				xlabel={\# keys},
				% xtick={1000,4000,6000,8000,10000,12000,14000,16000},
				% xticklabels={1k,4k,6k,8k,10k,12k,14k,16k},
				% xticklabel style={/pgf/number format/fixed},
				% scaled x ticks=false,
				ylabel={Time (min)},
				% ymax=100,
        % ymode=log,
				cycle multiindex* list={
								color       \nextlist
								mark list*  \nextlist
						},
				legend pos=north east,
				]
				\addplot[color=blue,mark=o,mark size=3pt] table [x=param, y=w-o1, col sep=comma] {figs/eval/o1/data.csv};
				\addplot[color=brown,mark=o,mark size=3pt] table [x=param, y=wo-o1, col sep=comma] {figs/eval/o1/data.csv};
        \legend{\ourtool, \ourtool(w/o O1)}
			\end{axis}
		\end{tikzpicture}
		\hspace{1ex}
	\end{scaletikzpicturetowidth}
	% \begin{scaletikzpicturetowidth}{0.23\textwidth}
	% 	\begin{tikzpicture}[scale=\tikzscale]
	% 		\begin{axis}[
	% 			title={(b) \si},
	% 			xlabel={\# txns},
	% 			xtick={2000,4000,6000,8000,10000},
	% 			xticklabels={2k,4k,6k,8k,10k},
	% 			xticklabel style={/pgf/number format/fixed},
	% 			scaled x ticks=false,
	% 			ylabel={Time (s)},
	% 			ymax=50,
	% 			cycle multiindex* list={
	% 							color       \nextlist
	% 							mark list*  \nextlist
	% 					},
	% 			legend pos=north east,
	% 			]
	% 			\addplot[color=blue,mark=o,mark size=3pt] table [x=param, y=ours, col sep=comma] {figs/eval/uv/runtime/si.csv};
	% 			\addplot[color=teal,mark=diamond,mark size=3pt] table [x=param, y=polysi, col sep=comma] {figs/eval/uv/runtime/si.csv};
	% 			\addplot[color=orange,mark=asterisk,mark size=3pt] table [x=param, y=viper, col sep=comma] {figs/eval/uv/runtime/si.csv};
	% 			\addplot[color=violet,mark=triangle,mark size=3pt] table [x=param, y=dbcop, col sep=comma] {figs/eval/uv/runtime/si.csv};
	% 			\legend{\ourtool, \polysi, \viper, \dbcop}
	% 		\end{axis}
	% 	\end{tikzpicture}
	% \end{scaletikzpicturetowidth}
	% }
	
	\caption{Comparison of \ourtool and \ourtool(w/o O1)'s runtime on extreme workloads.}
	\label{fig:extreme-o1}
\end{figure}

==> figs/eval/repeat-ratio/repeat-ratio.tex <==
% repeat-ratio.tex

\pgfplotsset{height=140pt, width=240pt}
\begin{figure}[t]
	\centering
	\resizebox{0.46\textwidth}{!}{
	\begin{scaletikzpicturetowidth}{0.46\textwidth}
		\begin{tikzpicture}[scale=\tikzscale]
			\begin{axis}[
				% title={C-Twitter 10K},
				xlabel={\#Transactions},
				ylabel={Time (s)},
        % ymax=60,
				xtick={2000,4000,6000,8000,10000},
				xticklabels={2k,4k,6k,8k,10k},
        xticklabel style={/pgf/number format/fixed},
				scaled x ticks=false,
				legend pos=north west,
				]
				\addplot[color=diverge1,mark=o,mark size=3pt] table [x=param, y=uv, col sep=comma] {figs/eval/repeat-ratio/data.csv};
				% \addplot[color=diverge2,mark=o,mark size=3pt] table [x=param, y=0.5, col sep=comma] {figs/eval/repeat-ratio/data.csv};
				\addplot[color=diverge3,mark=o,mark size=3pt] table [x=param, y=0.7, col sep=comma] {figs/eval/repeat-ratio/data.csv};
				% \addplot[color=diverge4,mark=o,mark size=3pt] table [x=param, y=0.9, col sep=comma] {figs/eval/repeat-ratio/data.csv};
				\addplot[color=diverge5,mark=o,mark size=3pt] table [x=param, y=1.1, col sep=comma] {figs/eval/repeat-ratio/data.csv};
				\addplot[color=diverge6,mark=o,mark size=3pt] table [x=param, y=1.3, col sep=comma] {figs/eval/repeat-ratio/data.csv};
				\addplot[color=diverge7,mark=o,mark size=3pt] table [x=param, y=1.5, col sep=comma] {figs/eval/repeat-ratio/data.csv};
        % \legend{UV,s=0.5,s=0.7,s=0.9,s=1.1,s=1.3,s=1.5}
        \legend{UV,$\theta$=0.5,$\theta$=0.9,$\theta$=1.3,$\theta$=1.5}
      \end{axis}
		\end{tikzpicture}
    \hspace{1ex}
	\end{scaletikzpicturetowidth}
	}
	
  \caption{Comparison of history size(number of transactions) and \ourtool's verification time under different repeating rate.
  Write values of non-\uniqueval{} workloads for each key are in zipfian distribution($\theta$ is shown in the figure, $N = 100$)}
	\label{fig:repeat-ratio}
\end{figure}

==> figs/eval/scalability/dup/dup.tex <==
% dup.tex


\pgfplotsset{height=140pt, width=240pt}
\begin{figure}[t]
	\centering
	\resizebox{\linewidth}{!}{
	\begin{scaletikzpicturetowidth}{0.27\textwidth}
		\begin{tikzpicture}[scale=\tikzscale]
			\begin{axis}[
				title={},
				xlabel={$\theta$},
				ylabel={Time (h)},
				ymax=10,
				cycle multiindex* list={
								color       \nextlist
								mark list*  \nextlist
						},
				legend pos=north west,
				legend style={yshift=2pt},
        xtick={0, 0.25, 0.5, 0.75, 1}
				]
				\addplot[color=blue,mark=o,mark size=3pt] table [x=param, y=grh, col sep=comma] {figs/eval/scalability/dup/runtime.csv};
				\addplot[color=brown,mark=o,mark size=3pt] table [x=param, y=grw, col sep=comma] {figs/eval/scalability/dup/runtime.csv};
				\addplot[color=violet,mark=o,mark size=3pt] table [x=param, y=gwh, col sep=comma] {figs/eval/scalability/dup/runtime.csv};
				\legend{GeneralRH, GeneralRW, GeneralWH}
			\end{axis}
		\end{tikzpicture}
		\hspace{1ex}
	\end{scaletikzpicturetowidth}
  \begin{scaletikzpicturetowidth}{0.27\textwidth}
		\begin{tikzpicture}[scale=\tikzscale]
			\begin{axis}[
				title={},
				xlabel={$\theta$},
				ylabel={Memory (GB)},
				ymax=70,
				cycle multiindex* list={
								color       \nextlist
								mark list*  \nextlist
						},
				legend pos=north east,
				legend style={yshift=-12pt},
        xtick={0, 0.25, 0.5, 0.75, 1}
				]
				\addplot[color=blue,mark=o,mark size=3pt] table [x=param, y=grh, col sep=comma] {figs/eval/scalability/dup/mem.csv};
				\addplot[color=brown,mark=o,mark size=3pt] table [x=param, y=grw, col sep=comma] {figs/eval/scalability/dup/mem.csv};
				\addplot[color=violet,mark=o,mark size=3pt] table [x=param, y=gwh, col sep=comma] {figs/eval/scalability/dup/mem.csv};
				% \legend{GeneralRH, GeneralRW, GeneralWH}
			\end{axis}
		\end{tikzpicture}
		\hspace{1ex}
	\end{scaletikzpicturetowidth}
	}
	
  \caption{\ourtool's overhead under large-sized workloads of 100k transactions and over 2 million operations}
	\label{fig:scala-dup-theta}
\end{figure}

==> figs/eval/scalability/rate/rate.tex <==
% rate.tex


\pgfplotsset{height=140pt, width=240pt}
\begin{figure}[t]
	\centering
	\resizebox{\linewidth}{!}{
	\begin{scaletikzpicturetowidth}{0.27\textwidth}
		\begin{tikzpicture}[scale=\tikzscale]
			\begin{axis}[
				title={},
				xlabel={dup key proportion\%},
				ylabel={Time (h)},
				ymax=5.5,
				cycle multiindex* list={
								color       \nextlist
								mark list*  \nextlist
						},
				legend pos=north east,
				legend style={yshift=-12pt},
        xtick={0, 0.25, 0.5, 0.75, 1}
				]
				\addplot[color=blue,mark=o,mark size=3pt] table [x=param, y=grh, col sep=comma] {figs/eval/scalability/rate/runtime.csv};
				\addplot[color=brown,mark=o,mark size=3pt] table [x=param, y=grw, col sep=comma] {figs/eval/scalability/rate/runtime.csv};
				\addplot[color=violet,mark=o,mark size=3pt] table [x=param, y=gwh, col sep=comma] {figs/eval/scalability/rate/runtime.csv};
				\legend{GeneralRH, GeneralRW, GeneralWH}
			\end{axis}
		\end{tikzpicture}
		\hspace{1ex}
	\end{scaletikzpicturetowidth}
  \begin{scaletikzpicturetowidth}{0.27\textwidth}
		\begin{tikzpicture}[scale=\tikzscale]
			\begin{axis}[
				title={},
				xlabel={dup key proportion\%},
				ylabel={Memory (GB)},
				ymax=70,
				cycle multiindex* list={
								color       \nextlist
								mark list*  \nextlist
						},
				legend pos=north east,
				legend style={yshift=-12pt},
        xtick={0, 0.25, 0.5, 0.75, 1}
				]
				\addplot[color=blue,mark=o,mark size=3pt] table [x=param, y=grh, col sep=comma] {figs/eval/scalability/rate/mem.csv};
				\addplot[color=brown,mark=o,mark size=3pt] table [x=param, y=grw, col sep=comma] {figs/eval/scalability/rate/mem.csv};
				\addplot[color=violet,mark=o,mark size=3pt] table [x=param, y=gwh, col sep=comma] {figs/eval/scalability/rate/mem.csv};
				% \legend{GeneralRH, GeneralRW, GeneralWH}
			\end{axis}
		\end{tikzpicture}
		\hspace{1ex}
	\end{scaletikzpicturetowidth}
	}
	
  \caption{\ourtool's overhead under large-sized workloads of 100k transactions and over 2 million operations
	}
	\label{fig:scala-dup-key-proportion}
\end{figure}

==> figs/eval/width-revisit/width-revisit.tex <==
% width-revisit.tex

\pgfplotsset{height=140pt, width=240pt}
\begin{figure}[h]
	\centering
	\resizebox{\linewidth}{!}{
  \begin{scaletikzpicturetowidth}{0.33\textwidth}
		\begin{tikzpicture}[scale=\tikzscale]
			\begin{axis}[
				title={(a)},
				xlabel={G-RUBiS},
				ylabel={$\sscw$},
				% ymax=30,
				cycle multiindex* list={
								color       \nextlist
								mark list*  \nextlist
						},
				legend pos=north west,
        ytick={10,50,100,400,800},  
        ymax=100,
        xtick={1,2,3,4,14},
				]
				\addplot[color=ps3green,mark=*,mark size=1pt] table [x=param, y=ours-hc, col sep=comma] {figs/eval/width-revisit/grubis.csv};
				\addplot[color=ps1green,mark=*,mark size=1pt] table [x=param, y=ours-hcp, col sep=comma] {figs/eval/width-revisit/grubis.csv};
				\addplot[color=ps5green,mark=*,mark size=1pt] table [x=param, y=ours-h, col sep=comma] {figs/eval/width-revisit/grubis.csv};
				\addplot[color=ps7green,mark=*,mark size=1pt] table [x=param, y=ours, col sep=comma] {figs/eval/width-revisit/grubis.csv};
			\end{axis}
		\end{tikzpicture}
		\hspace{1ex}
	\end{scaletikzpicturetowidth}
  \begin{scaletikzpicturetowidth}{0.33\textwidth}
		\begin{tikzpicture}[scale=\tikzscale]
			\begin{axis}[
				title={(b)},
				xlabel={GeneralRH},
				ylabel={$\sscw$},
				% ymax=30,
				cycle multiindex* list={
								color       \nextlist
								mark list*  \nextlist
						},
				legend pos=north west,
        legend style={font=\tiny, yshift=-12pt},
        ytick={0,20,40},  
        ymax=50,
        extra y tick style={tick label style={anchor=west}}, % 自定义刻度标签位置  
        xtick={1,17},
        unbounded coords=discard,
				]
				\addplot[color=ps1green,mark=*,mark size=1pt] table [x=param, y=ours-hcp, col sep=comma] {figs/eval/width-revisit/grh.csv};
				\addplot[color=ps3green,mark=*,mark size=1pt] table [x=param, y=ours-hc, col sep=comma] {figs/eval/width-revisit/grh.csv};
				\addplot[color=ps5green,mark=*,mark size=1pt] table [x=param, y=ours-h, col sep=comma] {figs/eval/width-revisit/grh.csv};
				\addplot[color=ps7green,mark=*,mark size=1pt] table [x=param, y=ours, col sep=comma] {figs/eval/width-revisit/grh.csv};
        
        \legend{
          {\ourtool w/o \textbf{H}, \textbf{C} and \textbf{P}},
          {\ourtool w/o \textbf{H} and \textbf{C}},
          {\ourtool w/o \textbf{H}},
          {\ourtool},
        }
			\end{axis}
		\end{tikzpicture}
		\hspace{1ex}
	\end{scaletikzpicturetowidth}
	 
  \begin{scaletikzpicturetowidth}{0.33\textwidth}
		\begin{tikzpicture}[scale=\tikzscale]
			\begin{axis}[
				title={(c)},
				xlabel={GeneralRW},
				ylabel={$\sscw$},
				% ymax=30,
				cycle multiindex* list={
								color       \nextlist
								mark list*  \nextlist
						},
				legend pos=north east,
        ytick={5,25,50,100,150},  
        ymax=200,
        xtick={1,2,3,4,5,10,15,21},
				]
				\addplot[color=ps1green,mark=*,mark size=1pt] table [x=param, y=ours-hcp, col sep=comma] {figs/eval/width-revisit/grw.csv};
				\addplot[color=ps3green,mark=*,mark size=1pt] table [x=param, y=ours-hc, col sep=comma] {figs/eval/width-revisit/grw.csv};
				\addplot[color=ps5green,mark=*,mark size=1pt] table [x=param, y=ours-h, col sep=comma] {figs/eval/width-revisit/grw.csv};
				\addplot[color=ps7green,mark=*,mark size=1pt] table [x=param, y=ours, col sep=comma] {figs/eval/width-revisit/grw.csv};
        
			\end{axis}
		\end{tikzpicture}
		\hspace{1ex}
	\end{scaletikzpicturetowidth}
  \begin{scaletikzpicturetowidth}{0.33\textwidth}
		\begin{tikzpicture}[scale=\tikzscale]
			\begin{axis}[
				title={(d)},
				xlabel={GeneralWH},
				ylabel={$\sscw$},
				% ymax=30,
				cycle multiindex* list={
								color       \nextlist
								mark list*  \nextlist
						},
				legend pos=north east,
        ytick={0,50,100,400},  
        ymax=500,
        xtick={1,5,8,21},
        unbounded coords=discard,
				]
				\addplot[color=ps1green,mark=*,mark size=1pt] table [x=param, y=ours-hcp, col sep=comma] {figs/eval/width-revisit/gwh.csv};
				\addplot[color=ps3green,mark=*,mark size=1pt] table [x=param, y=ours-hc, col sep=comma] {figs/eval/width-revisit/gwh.csv};
				\addplot[color=ps5green,mark=*,mark size=1pt] table [x=param, y=ours-h, col sep=comma] {figs/eval/width-revisit/gwh.csv};
				\addplot[color=ps7green,mark=*,mark size=1pt] table [x=param, y=ours, col sep=comma] {figs/eval/width-revisit/gwh.csv};
        
        % \legend{
        %   {\ourtool},
        %   {\ourtool w/o \textbf{H}},
        %   {\ourtool w/o \textbf{H} and \textbf{C}},
        %   {\ourtool w/o \textbf{H}, \textbf{C} and \textbf{P}}
        % }
			\end{axis}
		\end{tikzpicture}
		\hspace{1ex}
	\end{scaletikzpicturetowidth}
  }

  \caption{Suffix sums of encountered cycles by width}
	\label{fig:width-revisit}
\end{figure}

==> figs/exactly-one-encoding.tex <==
% exactly-one-encoding.tex

\begin{figure}[t]
  \centering
  \begin{subfigure}[b]{0.20\textwidth}
    \centering
    \includegraphics[width=0.8\textwidth]{plot/encoding-ww-case.pdf}
       		        		\captionsetup{skip=2pt}
    \caption{For $\WW$ constraints}
    \label{fig:exactly-one-encoding-ww}
  \end{subfigure}
\hspace{4ex}
  \begin{subfigure}[b]{0.2\textwidth}
    \centering
    \includegraphics[width=0.8\textwidth]{plot/encoding-wr-case.pdf}
       		        		\captionsetup{skip=2pt}
    \caption{For $\WR$ constraints}
    \label{fig:exactly-one-encoding-wr}
  \end{subfigure}
     		        		\captionsetup{skip=4pt}
  \caption{Illustration of the ``at-most-one''
    parts of $\WW$ and $\WR$ constraints.}
  \label{fig:exactly-one-encoding}
\end{figure}

==> figs/list-append.tex <==
% list-append.tex

\begin{figure}[t]
  \centering
  \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plot/list-append-checking-general-false-positive.pdf}
    \caption{A general list-append history.}
    \label{fig:list-append-history}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plot/list-append-checking-general-false-positive.pdf}
    \caption{Unfolded list-append history.}
    \label{fig:unfolded-list-append-history}
  \end{subfigure}
  \begin{subfigure}[b]{0.25\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plot/list-append-checking-general-solution.pdf}
    \caption{Unfolded universal polygraph.}
    \label{fig:list-append-uupg}
  \end{subfigure}
  \caption{Illustration of list-append history
    and unfolded universal polygraph.}
  \label{fig:list-append-example}
\end{figure}

==> figs/overview-example.tex <==
% overview-example.tex

\begin{figure*}[t]
  \centering
  \begin{subfigure}[b]{0.46\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plot/overview-example-constraint.pdf}
    \caption{A history with constraints}
    \label{fig:overview-eg-constraints}
  \end{subfigure}
  \hfill % 在子图间填充空白
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plot/overview-example-pruning.pdf}
    \caption{The dependency graph after pruning}
    \label{fig:overview-eg-pruning}
  \end{subfigure}
  \hfill % 填充空白
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plot/overview-example-solving-step1.pdf}
    \caption{The dependency graph after solving step 1}
    \label{fig:overview-eg-solving-step1}
  \end{subfigure}
  \hfill % 填充空白
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plot/overview-example-solving-step2.pdf}
    \caption{The dependency graph after solving step 2}
    \label{fig:overview-eg-solving-step2}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plot/overview-example-solving-step3.pdf}
    \caption{The dependency graph after solving step 3(a valid solution)}
    \label{fig:overview-eg-solving-step3}
  \end{subfigure}
  % 确保最后没有超出边界的 \hfill

  \caption{%Illustration of constraints in
  A motivating example of \ourtool's workflow}
  \label{fig:overview-eg}
\end{figure*}


==> figs/propagate-eg.tex <==
% propagate-eg.tex

\begin{figure}[t]
  \centering
  \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plot/search-wo-prop.pdf}
    \caption{w/o propagate}
    \label{fig:search-example-wo-prop}
  \end{subfigure}
  \hfill % 在子图间填充空白
  \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plot/search-w-prop.pdf}
    \caption{w/ propagate}
    \label{fig:search-example-w-prop}
  \end{subfigure}

  \caption{An example: the effectiveness of propagation 
    \zhiheng{(i) visualize some medium states? (ii) rotate this figure}
  }
  \label{fig:search-example}
\end{figure}


==> figs/propagate.tex <==
% propagate.tex

\begin{figure}[t]
  \centering
  \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plot/search-tree-wo-prop.pdf}
    \caption{w/o propagate}
    \label{fig:search-tree-wo-prop}
  \end{subfigure}
  \hfill % 在子图间填充空白
  \begin{subfigure}[b]{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plot/search-tree-w-prop.pdf}
    \caption{w/ propagate}
    \label{fig:search-tree-w-prop}
  \end{subfigure}

  \caption{The effectiveness of propagation \nobi{is that possible to instantiate these trees with concrete examples?}}
  \label{fig:propagate}
\end{figure}


==> figs/rw-checking.tex <==
% rw-checking.tex

\begin{figure*}[h]
  \centering
  \begin{subfigure}[b]{0.18\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plot/RW-checking-general2-hist.pdf}
    		\captionsetup{skip=2pt}
    \caption{General history $\H$.}
    \label{fig:history-h2}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.24\textwidth}
    \centering
    \includegraphics[width = 0.85\textwidth]{plot/RW-checking-general2-constraints.pdf}
    		\captionsetup{skip=2pt}
    \caption{Hyper-polygraph $\G$ of $\H$.}
    \label{fig:rw-checking-h2-constraints}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.28\textwidth}
    \centering
    \includegraphics[width = 0.70\textwidth]{plot/RW-checking-general2-solution.pdf}
    		\captionsetup{skip=2pt}
    \caption{An acyclic graph compatible with $\G$.}
    \label{fig:rw-checking-h2-solution}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.26\textwidth}
    \centering
    \includegraphics[width = 0.8\textwidth]{plot/RW-checking-general2-conflict.pdf}
    		\captionsetup{skip=2pt}
    \caption{A cyclic graph compatible with $\G$.}
    \label{fig:rw-checking-h2-conflict}
  \end{subfigure}
  		\captionsetup{skip=6pt}
  \caption{A general history $\H$, along with its hyper-polygraph $\G$
    and two compatible graphs.}
  \label{fig:rw-checking}
\end{figure*}

==> sections/background.tex <==
\section{Preliminaries} \label{section:pre}

\hfwei{Move list-append to Section~\ref{section:list}???
  Not sure about this.}

\input{sections/notations}
\input{sections/history}
\input{sections/ser}
\input{sections/ser-depgraph}
\input{sections/ser-checking}

==> sections/conclusion-nobi-0424.tex <==
\section{Conclusion}

==> sections/conclusion.tex <==
\section{Conclusion}

We first lift the common \uniqueval{} assumption 
in database isolation level testing and 
present \ourtool, 
a checker for verifying various isolation levels. 
\ourtool incorporates a dedicated SMT solver based on MonoSAT, 
with enhancements into every checking stages.
\blue{Histories can be encoded into SMT formulas based on universal polygraphs, 
an intermediate representation of various isolation levels across different fomalisms.}
\blue{[list append]}
Our extensive experiments have demonstrated 
the effectiveness and efficiency of \ourtool
across a wide range of general workloads.
Furthermore, 
our empirical analysis underlying each key optimization reveals 
distinctive patterns in real-world workload characteristics. 
These findings extend beyond our specific context, 
potentially informing solutions to related optimization problems.

% One limitation to note is that
% the performance of \ourtool 
% demonstrates sensitivity to workload characteristics 
% (i.e., the write proportion and the duplication rate). 
% The efficiency degrades when these parameters reach certain thresholds.
% Our future work will focus on improving algorithmic stability
% across various workloads.


==> sections/discussion.tex <==
\section{Discussion}
\nobi{lessons learned?}

\inlsec{Understanding the Efficiency of \listappend}
\zhiheng{TODO}

\inlsec{Uncovering Characteristics of Real-world Workloads through SMT Solving}
We propose two optimizations for accelerating the SMT solving process: 
small cycle optimization (\textbf{C}) and polarity picking heuristics (\textbf{H}). 
These optimizations are based on careful observations of the SMT solving process.

Specifically, 
\textbf{C} is motivated on our observation that 
the width of encountered cycles is typically small, 
with 2-width cycles being predominant. 
\textbf{H} is motivated on our observation that despite frequent cycle detection attempts, 
successful cycle discoveries are rare. 
These patterns appear to be inherent characteristics of real-world workloads, 
and remain consistent across different workload parameters (see section~\ref{sss:workloads}).

While these characteristics are inherently complex and 
require deep analysis to fully understand, 
they emerge during the solving process and 
may provide valuable insights for other execution and checking tasks 
beyond the immediate solving problem 
(e.g. concurrency control~\cite{OCC:TODS1981}).

\inlsec{Understanding the Rationale of Optimization \textbf{H} and \textbf{C}}
In addition to empirically validating the efficiency of 
optimizations \textbf{C} and \textbf{H}, 
we seek to elucidate their underlying mechanisms. 
This investigation is inherently complex due to 
the limited interpretability of SMT solving processes. 
A fundamental aspect is the branching strategy of SMT solving, 
which implements a variant of depth-first search and significantly influences solving efficiency. 
Both \textbf{C} and \textbf{H} affect this branching strategy. 
Prior research has demonstrated~\cite{Grasp:ICCAD96,SMT:JACM2006} the effectiveness of unit propagation, 
providing partial theoretical support for optimization \textbf{C}. 
The theoretical foundation of \textbf{H}, however, 
requires further investigation. 
A significant theoretical gap exists between our empirical observation of cycle rarity 
and the proposed heuristic, 
particularly regarding the fundamental question of graph traversal preference. 
This theoretical challenge may be intrinsically connected to underlying \npc properties.

\inlsec{Limitations and Future Work}
Currently, \ourtool lacks support for complex operations 
such as range queries~\cite{Viper:EuroSys2023} and predicates~\cite{Emme:EuroSys2024}, 
which constrains its bug detection capabilities. 
Additionally, \ourtool is limited in generating comprehensible counter-examples, 
failing to meet the \textbf{I}nformative criterion of SIEGE+ principles~\cite{PolySI:VLDB2023}.
Our future research directions will focus on 
extending our verification approach along multiple dimensions: 
enhancing algorithmic stability, 
supporting complex query operations, 
and generating informative counter-examples.

\brown{[(vi) migarate to other isolation level]}
  Moreover,
  we extend our UP-based characterization of \ser,
  under Adya's formalism~\cite{Adya:PhDThesis1999}
  to \si under Gotsman's formalism~\cite{AnalysingSI:JACM2018}
  and weaker isolation levels under Enea's formalism~\cite{Complexity:OOPSLA2019},
  offering a unified framework for checking general histories
  across formalisms.
  This approach provides a comprehensive solution
  beyond the scope of a single isolation level or formalism.
  \blue{[discuss more about our approaches, and list append]}

==> sections/evaluation.tex <==
\section{Evaluation} \label{section:evaluation}

We have implemented our algorithm in a tool called \ourtool{} on top of \minisat \cite{MiniSAT:SAT2004} in around 5k LOC in C++.
We conduct a comprehensive evaluation of \ourtool and the state-of-the-art tools,
and answer the following research questions.

\begin{enumerate}
  \item How effective is \ourtool{} in identifying bugs? 
	Specifically,
  can \ourtool reproduce known bugs in production databases?
	Can \ourtool detect new isolation bugs related to duplicate write values?
  \item How efficient is \ourtool and its components? 
  How does \ourtool perform under general workloads?
  Can \ourtool outperform the state of the art under \uniqueval{} workloads?
  Can \ourtool scale up to large workloads?
\end{enumerate}

\subsection{Workloads, Benchmarks, and Setup}

\subsubsection{Workloads}	\label{sss:workloads}

To introduce duplicate write values,
we design a parametric workload generator
on top of PolySI~\cite{PolySI:VLDB2023,Complexity:OOPSLA2019}.
We assume that the write values to the same key
follow a Zipfian distribution ($\theta = 0.5$ and $N = 100$ by default),
because:
(i) A Zipfian distribution models certain real-world patterns effectively~\cite{HumanBA:Language1950}; 
(ii) Compared to distributions with more uniform value frequencies, 
Zipfian introduces higher checking overhead due to the frequent occurrence of dominant values; and
(iii) The "duplication" rate can be controlled by adjusting the parameters $\theta$ and $N$.

The parameters are:
\begin{itemize}
	\item the number of client sessions (\#sess=20 by default),
	\item the number of transactions per session (\#txns/sess=100 by default),
	\item the number of read/write operations per transaction (\#opt/txn=20 by default),
	\item the read proportion\footnote{\red{for the whole history, not per transaction}} (50\% by default),
	\item the total number of keys (5k by default),
	\item the proportion of keys with duplicate write values (50\% by default).
\end{itemize}
% default config: 20_100_15_5000_0.5_r_0.5_0.5_100

\subsubsection{Benchmarks} \label{sss:benchmarks}

We consider seven benchmarks used by
existing black-box isolation level checkers~\cite{Cobra:OSDI2020,Viper:EuroSys2023,PolySI:VLDB2023,Plume:OOPSLA2024}.
These include three macro-benchmarks,
comprising only serializable histories of at least 10k transactions
\red{[\uniqueval???]}.
TPC-C~\cite{TPCC} is a standard benchmark for online transaction processing,
with a configuration involving one warehouse, 10 districts, 30k customers,
and five types of transactions.
C-RUBiS~\cite{CRUBis} is an eBay-like bidding system,
compring 20k users and 200k items.
C-Twitter~\cite{CTwitter} is a Twitter clone
where key accesses follow the zipfian distribution.

Our benchmark generator produces general histories
on top of TPC-C, C-RUBiS, and C-Twitter,
as opposed to that of Cobra~\cite{Cobra:OSDI2020}.
(renamed as G-TPCC, G-RUBiS and G-Twitter, respectively)
\footnote{After removing the unique identifier,
we found G-TPCC still meets the \uniqueval{} assumption,
whereas G-RUBiS and G-Twitter both contain duplicate write values.}.

In addition, four representive general datasets are also included:
GeneralRH (read-heavy with 95\% reads),
GeneralWH (write-heavy with 70\% writes),
GeneralRW (balanced, 50\% reads),
and, to simulate extreme scenarios,
GeneralDV (50\% reads, write values are in zipfian($\theta = 1.5, N = 100$)).
Each benchmark contains at least 10k transactions and 80k operations.

\subsubsection{Experimental Setup} \label{sss:setup}

We use a PostgresSQL (v15 beta 1) instance to produce general histories.
All experiments are conducted on a local machine with Intel(R) 13th i5 CPU and 32GB memory,
unless explicitly stated otherwise.



\subsection{Performance Evaluation}

\subsubsection{Comparison with baselines on general histories}

To our knowledge, \ourtool is the first checker
capable of handling duplicate write values.
We compare it to the baseline described in Section~\ref{section:baseline}
in terms of performance.
We also enhance the baseline with an existing pruning techinique
of \WW{} edges from~\cite{Cobra:OSDI2020} as a stronger competitor 
(refered to as baseline+P).
\zhiheng{TODO: need this enhanced baseline?}

\input{figs/eval/various/runtime.tex}
\input{figs/eval/various/mem.tex}

% Figures~\ref{fig:various-runtime} and~\ref{fig:various-memory}
% show the runtime and memory consumption, respectively.
As shown in Figures~\ref{fig:various-runtime} 
and~\ref{fig:various-memory},
baseline can only handle a limited range of histories smaller than the default configuration 
and quickly ran out of time.
While the existing pruning technique extends the baseline's capacity 
to process larger histories, 
its impact is limited.
In contrast, 
\ourtool demonstrates the ability to handle significantly larger histories in less time 
while consuming less memory than the baselines.
Furthermore, 
subfigures (a), (b) and (c) of Figure~\ref{fig:various-runtime} and Figure~\ref{fig:various-memory} 
depict three different patterns of history size growth, 
illustrating that \ourtool remains notably more stable 
than the baselines under varying conditions;
\blue{Subfigures (d), (e), and (f) present three scenarios of history configuration changes, 
highlighting the relative efficiency of \ourtool compared to the baselines.}

\subsubsection{Comparison with the state-of-the-art on \uniqueval{} histories}

We conduct a comprehensive performance analysis of \ourtool on \uniqueval{} histories 
taken from \cobra~\cite{Cobra:OSDI2020} and \viper~\cite{Viper:EuroSys2023}
under both \ser and \si isolation level,
alongwith five the-state-of-the-art baselines.
\begin{itemize}
	\item \cobra \cite{Cobra:OSDI2020}, as the state-of-the-art tool for \ser.
	Given that \cobra employs an expansive V100 GPU to accelerate its pruning process,
	while \ourtool does not rely on GPU acceleration,
	we include both \cobra(w/o GPU) and \cobra(w/ V100 GPU) as two baselines.
	\footnote{Due to resource limitations, 
	we can only run \cobra(w/ V100 GPU) on a network server,
	which differs from the test environment for other baselines.
	}

	\item \polysi \cite{PolySI:VLDB2023} and \viper \cite{Viper:EuroSys2023}, as the state-of-the-art tool for \si.
	
	\item \dbcop \cite{Complexity:OOPSLA2019}, as the representative of non-SMT methods.
	\dbcop is capable of verifying both \ser and \si.
\end{itemize}

\input{figs/eval/uv/runtime/runtime.tex}

As Figure~\ref{fig:uv-runtime} shows, 
\ourtool surpasses all competitors under both \ser and \si.
Specifically, 
under \ser,
\ourtool performs extraordinarily better than \cobra(w/o GPU).
Even compared to \cobra(w/ V100 GPU), \ourtool achieves up to 4.4x speedup.
Under \si, \ourtool achieves up to 4x speedup compared to \polysi and up to 34x speedup compared to \viper.
Given that \cobra, \polysi, \viper all utilize the pruning technique and leverage MonoSAT as their backend solver, 
these results solidly demonstrate that our optimizations effectively accelerate the solving procedure.

\subsubsection{Comparison of list-append and RW-register modes in \ourtool with Elle}

We conduct a comprehensive performance analysis of the list-append and RW-register modes in \ourtool. 
To this end, we generate workloads consisting of $10^4$ transactions with varying proportions of keys with duplicate write values. 
These workloads are then executed in both RW-register and list-append modes 
(i.e., write operations are translated into corresponding append operations). 
In this setup, a duplicate key proportion of $0$ corresponds to the \uniqueval{} condition, 
enabling a comparison with Elle~\cite{Elle:VLDB2020}.

\input{figs/eval/list-rw/list-rw.tex}

As shown in Figure~\ref{fig:list-rw}, 
\ourtool-list outperforms \ourtool-RW across all benchmarks. 
This is because \ourtool-list is capable to recover a portion of $\WW$ relations 
while \ourtool-RW has to solve them all. 
While Elle is the most efficient tool for \uniqueval{} histories, 
it raises an exception and then exits on histories containing duplicate write values, 
which it cannot handle due to its design.

\subsection{Decomposition Analysis}

\input{figs/eval/decomposition/decomposition.tex}

We decompose \ourtool's checking time into four stages:
construting, pruning, encoding and solving.
The results are presented in Figure~\ref{fig:decomposition}.
Among the seven benchmarks, 
G-TPCC is special as all constraints can be pruned~\cite{Cobra:OSDI2020},
allowing it to skip the encoding and solving stages.
For other benchmarks,
constructing and pruning are generally inexpansive.
In many cases (except G-RUBiS and GeneralDV),
solving time is relatively short 
while encoding time is longer than anticipated.
This behavior is due to our small-width cycles optimization, 
which shifts some solving overhead to pruning and encoding, 
while keeping the pruning and encoding overhead moderate and reduing the overall checking time.
For certain "complex" benchmarks (G-RUBiS and GeneralDV), 
solving remains computationally expensive.

\subsection{Ablation Analysis}

To investigate the contributions of \ourtool's three major optimizations,
we experiment with four variants: 
(i) \ourtool itself; 
(ii) \ourtool without the polarity picking \underline{h}euristic(\textbf{H});
(iii) \ourtool without \textbf{H}, and the encoding of small width \underline{c}ycles(\textbf{C});
(iv) \ourtool without \textbf{H} and \textbf{C}, and \underline{p}runing(\textbf{P}).

\subsubsection{General Ablation Analysis}
\input{figs/eval/new-ablation/ablation.tex}

% \input{tables/ablation.tex}

Figure~\ref{fig:ablation} shows the ablation results of the variants discribed above.
It appears that \textbf{H} and \textbf{C} do not affect G-TPCC at all.
Given the aforementioned fact that
all contraints can be pruned in G-TPCC,
the solving process is bypassed.
This also explained why \textbf{P} has a noticeable impact on G-TPCC.

Optimization step \textbf{H} works well on G-RUBiS, GeneralRW, GeneralWH and GeneralDV,
achieving around 1.8x speedup on GeneralWH, G-RUBiS and GeneralDV, 
but it does not make a difference on G-Twitter and GeneralRH.
In fact, G-Twitter is also a read-heavy history.
During the solving process of read-heavy histories, 
cycles are rarely found, 
which limits the ability of \textbf{H} to avoid conflict resolutions.

One may question the effect of \textbf{C}, 
for \cite{Cobra:OSDI2020} and \cite{PolySI:VLDB2023} has demonstrated the significant efficiency of pruning.
By comparing Variant (iii) and Variant (iv),
we found the effect of \textbf{C} is similar to \textbf{H}.
\textbf{C} enables \ourtool achieve up to 2.7x speedup on GeneralDV.
Notice that \textbf{C} decreases the solving speed on GeneralRH.
This is attributed to the enumeration of small width cycles. 
However, the overhead is relatively minor, 
and the difference is only noticeable with such short solving times.

\subsubsection{Revisiting width of cycles}
\label{sss:revisit-width-of-cycles}

To better illustrate the effectiveness of \textbf{P}, \textbf{C} and \textbf{H} in reducing the frequency of conflict resolution,
we record the width of encountering cycles in the solving process,
as shown in Figure~\ref{fig:width-revisit}.
\footnote{In this experiment, the number of transactions is reduced to 1k, due to the inefficiency of the unoptimized tools.}

\input{figs/eval/width-revisit/width-revisit.tex}

In Figure~\ref{fig:width-revisit}, 
we record the widths of all encountered cycles
\emph{w/o minimizing} 
and present the suffix sum of the cycle counts by width, denoted as $\mathbb{S}(\cdot)$.
Specifically, $\sscw(k) = \sum\limits_{i = k}^{\infty} (\text{the number of cycles with width } i)$.
$\sscw(\cdot)$ has two key properties:
(1) $\sscw(1)$ represents the total number of cycles detections,
(2) $\Delta \sscw(k) = \sscw(k) - \sscw(k + 1)$ gives the number of detections of width $k$.
In general, 
the closer the curve of $\sscw$ is to the coordinate axis, 
the fewer cycles are detected, 
indicating a faster solving speed.

As shown in Figure~\ref{fig:width-revisit}(b),
Variant (i), (ii) and (iii) decect no cycles during solving, 
consistent with the result in Figure~\ref{fig:ablation}.
Notably, in (a), (b), (c) and (d) of Figure~\ref{fig:width-revisit},
all $\Delta \sscw(1) = 0$, indicating the correctness of pruning.
Figure~\ref{fig:width-revisit}(a), (c) and (d) demonstrate the effectiveness of \textbf{H}, \textbf{C} and \textbf{P} 
in reducing the frequency of detecting cycles.  
Additionally, the results in Figure~\ref{fig:width-revisit} highlight the robustness of \textbf{H}, \textbf{C} and \textbf{P},
as these optimization steps prove effective across various read-write scenarios ((b), (c) and (d)) and real-world histories ((a)). 

\subsubsection{Revisiting Statistics of PK algorithm}
\label{sss:revisit-statistics-of-pk}
\zhiheng{TODO}

\subsubsection{Choosing the width of encoded cycles}
\label{sss:choosing-encode-width}

In optimization step \textbf{C}, we encode 2-width cycles
(refer to Section~\ref{sss:encode-2-width-cycles}). 
One may wonder about the performance implications of extending our method to accommodate larger cycle widths.
To investigate this, 
we conduct a comparative experiment with variants of Variant (ii) by varying the encoding width $w$.

\input{figs/eval/encode-cycle-width/encode-cycle-width.tex}

In Figure~\ref{fig:encode-cycle-width}, 
$w = 1$ indicates that only pruning is applied, 
while $w \geqslant 2$ signifies that cycles with width $w$ are encoded.
We mark the timeout (TO) points by filling the masks, 
which are set at 600 seconds.
As shown in Figure~\ref{fig:encode-cycle-width}, 
$w = 2$ emerges as the optimal choice for all six benchmarks (excluding G-TPCC), 
except for GeneralRH.
However, the solving time for GeneralRH is relatively small compared to other histories, 
suggesting that encoding small-width cycles introduces only moderate overhead in solving time.

% \subsubsection{Ablation with the combination of our optimizations and MonoSAT}

% Since the optimization \textbf{P} and \textbf{C} are ``outside'' of the solver itself,
% one may be curious about what if we applying \textbf{P} and \textbf{C} to MonoSAT\cite{MonoSAT:AAAI2015}.
% To investigate this, we introduce two enhanced baselines based on MonoSAT:
% \begin{enumerate}
% 	\item MonoSAT+\textbf{P}, MonoSAT with the enhanced pruning techinique,
% 	\item MonoSAT+\textbf{P}+\textbf{C}, MonoSAT with \textbf{P} and the encoding of small width cycles.
% \end{enumerate}

% \zhiheng{Results of this experiment: MonoSAT cannot be integrated with \textbf{P}}

\subsection{Scalability}

To evaluate \ourtool's scalability, 
we generate workloads of 100k tracsactions and over 2 million operations, 
and we simulate two scenarios when the "duplicatation" rate grows 
by increasing the proportion of keys with duplicate write values 
and $\theta$ as a parameter of the Zipfian distribution.

% \input{figs/eval/scalability/rate/rate.tex}
% \input{figs/eval/scalability/dup/dup.tex}
\input{figs/eval/scalability/scala.tex}

As Figure~\ref{fig:scalability} shows
\footnote{
This experiment is conducted on a server with large memory.
The single-core clock speed of the CPU is reduced compared to the local machine,
so the runtimes are not comparable.
}, 
\ourtool completes checking large histories in under 6 hours 
while using less than 64GB of memory.
However, 
the runtime and memory usage increase significantly 
as the proportion of read operations decreases. 
This behavior is primarily due to the increase in the number of SAT variables 
when the proportion of writes rises, 
as additional $\WR$ edges must be encoded $k$ (the number of keys) times 
according to our UP-based characterization.
As shown in Subfigure (c) of Figure~\ref{fig:scalability}, 
the checking time grows largely with an increase in the "duplication" rate, 
particularly under high write proportions.
We acknowledge the scalability limitations of \ourtool in extreme duplicate scenarios. 
Nevertheless, 
real-world workloads such as G-RUBiS and G-Twitter suggest that 
such situations are rare in practice.

% \input{figs/eval/repeat-ratio/repeat-ratio.tex}

% \begin{table}[h]
% 	\centering
% 	\caption{Number of constraints and unknown dependencies before and after optimization clue I (O1) in the four benchmarks(w basic pruning).
%   \zhiheng{complete with max memory}}\label{benchmark-stat-equals-1}
% 	\begin{tabular}{c|rr|rr|}
% 		% \hline
% 		Benchmark  & \multicolumn{2}{c|}{\#encoding formulae.}  & \multicolumn{2}{c|}{Max Memory(MB)} \\
% 		           & before O1             & after O1            & before O1  &  after O1 \\
% 		\hline

%     G-TPCC     & 0                     & 0                   &            &  \\
% 		G-Twitter  & 12194                 & 2926                &            &  \\
% 		G-RUBiS    & 722.5K                & 5358                &            &  \\

% 		GeneralRH  & 2895                  & 1213                &            &   \\
% 		GeneralRW  & 43005                 & 15485               &            &  \\
% 		GeneralWH  & 66137                 & 26206               &            &  \\
% 		GeneralRV  & 2481.8k               & 40141               &            &  \\
% 		%\hline

% 	\end{tabular}
% 	\vspace{-3ex}
% \end{table}

% \begin{table}[h]
% 	\centering
% 	\caption{Number of $\WW$ and $\WR$ constraints before and after  pruning (P) in the four benchmarks.}\label{benchmark-stat-pruning}
% 	\begin{tabular}{c|rr|rr|}
% 		% \hline
% 		Benchmark  & \multicolumn{2}{c|}{\#$\WW$ cons.} & \multicolumn{2}{c|}{\#$\WR$ cons.} \\
% 		           & before P        & after P           & before P       & after P      \\
% 		\hline

% 		% TPC-C      & 386k     & 0       & 3628k        & 0            \\
% 		% RUBiS      & 14k      & 149     & 171k         & 839          \\
% 		% C-Twitter  & 59k      & 277     & 307k         & 776          \\
% 		% Courseware & 156k     & 3352    & 761k         & 10359       \\

%     G-TPCC     & 10.5k      & 0       & 10.3k         & 0        \\
% 		G-Twitter  & 26.6k      & 162     & 35.7k         & 455        \\
% 		G-RUBiS    & 30.1k      & 233     & 39.3k         & 1045        \\
    
% 		GeneralRH  & 6602       & 17      & 76.0k         & 69           \\
% 		GeneralRW  & 384.1k     & 5190    & 39.9k         & 312         \\
% 		GeneralWH  & 720.5k     & 13.9k   & 23.9k         & 282        \\
% 		GeneralRV  & 367.1k     & 8483    & 39.9k         & 4678        \\
% 		%\hline

% 	\end{tabular}
% 	\vspace{-3ex}
% \end{table}

\subsection{Effectiveness}

% \ourtool have reproduced all \uniqueval{} isolation bugs from \cite{Cobra:OSDI2020,PolySI:VLDB2023,Viper:EuroSys2023,Complexity:OOPSLA2019}\dots
% For general bugs, we set the isolation level of \si, and \ourtool found xxx bugs.

\inlsec{Reproduing Known \uniqueval{} Bugs} 
\ourtool has reproduced \emph{all} known bugs 
in a substantial collection of 2076 anomalous histories % 2076 = 3(polysi) + 7(cobra) + 2066(dbcop)
archived by prior works~\cite{Cobra:OSDI2020,Complexity:OOPSLA2019,PolySI:VLDB2023}.
These histories, collected from earlier versions of databases 
such as CockroachDB, YugabyteDB, Galera, and Dgraph, 
were generated under isolation levels \ser and \si.
All of these histories meet the \uniqueval{} assumption.


\inlsec{Discovering Bugs with Duplicate Write Values}
Inspired by bug reports~\cite{MySQL-Bug,MariaDB-Bug}, 
we integrated \ourtool into the Jepsen framework 
with a modified workload generator to produce duplicate write values.
Tests were conducted using this framework on MariaDB, MySQL, YugabyteDB, TiDB and others.
\ourtool successfully reproduced the reported bug in older versions of MySQL and MariaDB.
Additionally, it detected the same bug in the latest stable version of MariaDB, 
which has been reported to the developers~\blue{[TODO: cite bug report]}.
However, no isolation bugs were found in other databases. 
We believe that some databases may still be vulnerable under workloads with duplicate write values, 
and our future work will focus on using \ourtool to identify new isolation bugs under this condition.



==> sections/impl.tex <==
\section{Implementation}

\zhiheng{maybe move this sec into evaluation}

\inlsec{\ourtool}
We have implemented \ourtool in XXX \zhiheng{count lines} lines of cpp code \footnote{see our artifact XXX}.
Our dedicated SMT solver is built on \minisat \cite{MiniSAT:SAT2004}, a simple, well-known SAT solver.
\ourtool contains many more optimizations than above descriptions.
For exmaple, \ourtool employs the compacting techinique from \polysi \cite{PolySI:VLDB2023} on $\WW$ constraints.
And \ourtool also compacts edges in $\ug$ to avoid redundant calling of ICD algorithm.
Besides, Cpp provides us powerful and convenient libraries such as \texttt{std::bitset<>} that directly supports our reachability algorithm.
These optimizations, both implementational and non-implementational, has made \ourtool performs extraordinarily well on both \uniqueval{} and general workloads.

\inlsec{Generating General Histories}
We modified the history generator of \dbcop\cite{Complexity:OOPSLA2019} that can generate repeated write values.
To better simulate real-world workloads, we also modified the history generator of \cobra \cite{Cobra:OSDI2020} to generate general TPC-C, C-RUBiS and C-Twitter workloads.
We use a PostgreSQL(v15 Beta 1) instance to produce general histories.\zhiheng{...}

==> sections/intro-nobi.tex <==
\section{Introduction}

Modern cloud databases support various isolation levels---the ``I'' in ACID (Atomicity, Consistency, Isolation, Durability)~\cite{TIS:Book2001}---to manage concurrent transaction execution. These isolation levels range from strong guarantees, such as Serializability, to weaker options, such as Read Committed, allowing databases to balance data consistency against system performance. 
When a database goes live in the cloud, its promised isolation guarantees become a binding contract between the database provider and its users. This naturally raises a critical question: 
\emph{How can we be sure that a deployed database  meets its promised isolation guarantees?}

Recent years have witnessed notable progress in addressing this question~\cite{Cobra:OSDI2020,PolySI:VLDB2023,Viper:EuroSys2023,Plume:OOPSLA2024,Elle:VLDB2020,Complexity:OOPSLA2019,MiniTransactions:ICDE2025} (a detailed discussion is provided in Section~\ref{section:related}).
For instance, Cobra~\cite{Cobra:OSDI2020} and PolySI~\cite{PolySI:VLDB2023} are sophisticated checkers designed specifically to examine  databases against strong isolation guarantees---Serializability and Snapshot Isolation (SI), respectively;
Plume~\cite{Plume:OOPSLA2024}, by contrast, focuses on checking weaker isolation levels, including more recent Read Atomicity~\cite{RAMP:TODS2016} and Transactional Causal Consistency (TCC)~\cite{Eiger:NSDI2013};
Elle~\cite{Elle:VLDB2020} leverages specialized data structures to accelerate the checking process and fault injection to trigger isolation anomalies.
All these checkers adopt a \emph{black-box} approach, without relying on knowledge of cloud database internals, which are often inaccessible or opaque. 
Specifically, they
 collect execution histories of database transactions as external observers 
 and verify whether these histories conform to the specified isolation level---a task  known as the \emph{database history verification} problem.

%These checkers have successfully identified numerous real-world isolation bugs and have demonstrated promising performance in validating transactional correctness. 


\inlsec{Challenges}
Despite recent advances, 
major challenges remain that the state-of-the-art approaches have yet to fully address.

\paragraph{Efficiency (C1)}
Verifying database histories is inherently challenging. 
In particular, the verification problem for strong isolation levels, such as Serializability or SI,  has been proven NP-hard even when verifying a single history~\cite{Complexity:OOPSLA2019}. 
This challenge is further compounded by practical constraints: given limited computational resources such as time and memory, only a finite number of histories can be verified. 
Yet, examining more histories is highly desirable---either to increase the likelihood of detecting isolation anomalies or to strengthen confidence in their absence.

Existing approaches have attempted to alleviate verification overhead by leveraging advanced techniques like SMT solving~\cite{Cobra:OSDI2020,PolySI:VLDB2023,Viper:EuroSys2023}.
However, when applied to real-world database workloads, general-purpose techniques often miss domain-specific optimization opportunities, as we will see. 
Moreover, all these approaches assume \emph{uniquely written values} (\uniqueval{}), i.e., each read can be deterministically matched to a specific write.
While this  assumption simplifies the verification problem---reducing it from NP-hardness to a polynomial-time check---and is 
a key enabler of Elle's novelty (Section~\ref{section:list}),
 it deviates from real-world practice, where 
 it is common for different transactions to write the same value.
For example, in an e-commerce application, multiple users may submit orders with identical item quantities.



\paragraph{Soundness \& Completeness (C2)}


Many existing checkers either overlook isolation bugs or produce false positives,
as shown by a recent study~\cite{Plume:OOPSLA2024}.
This suggests that some of the histories they are able to handle under limited resources contribute little to effective  bug detection or history verification. 
This is particularly concerning because isolation bugs are notoriously difficult to detect:
uncovering missed anomalies may require substantial additional verification effort. 
Moreover, debugging isolation anomalies is often labor-intensive due to their subtle semantics and the complexity of modern database codebases.

One major reason for this lack of soundness or completeness is the absence of a rigorous connection between the theoretical characterizations of isolation levels and the algorithms used for their verification. 
For example, when checking TCC, Elle searches for a mixture of isolation anomalies derived from different formalizations~\cite{Adya:PhDThesis1999,Framework:CONCUR2015}, which are not known to soundly or completely characterize the property.
In addition, as recently reported~\cite{MariaDB-Bug,MySQL-Bug},  certain  isolation anomalies can  be triggered \emph{only} in the presence of duplicate written values (\duplicateval{}).
However, all existing checkers are designed to operate on \uniqueval{} histories; applying them to \duplicateval{} histories could result in either false positives or false negatives.

\paragraph{Generality (C3)}
The family of isolation levels has been growing since the last century~\cite{si,RAMP:TODS2016,ua,Eiger:NSDI2013,psi,ser,hat,Regular:SOSP2021}, driven by the evolving needs of diverse cloud applications.
In response, a variety of formal models~\cite{Adya:PhDThesis1999,Framework:CONCUR2015,Complexity:OOPSLA2019,AnalysingSI:JACM2018,Plume:OOPSLA2024,Seeing:PODC2017,Centralised:ECOOP2020,RAMP:TODS2016} have been proposed to capture and reason about these  guarantees. 
These formalisms often complement one another by covering different isolation levels. 
% or modeling distinct variants of the same level. 
For example, compared to Adya's theory~\cite{Adya:PhDThesis1999}, the formalism proposed by Cerone et al.~\cite{Framework:CONCUR2015} supports TCC but not  Read Committed.


Additionally,
modern databases and applications  offer users multiple isolation guarantees to accommodate varying requirements. 
In practice, 
system developers 
often do not adhere strictly to a single formalism
 due to 
 divergent interpretations of isolation levels across  formalisms.
For instance,
 Cerone  and Gotsman~\cite{AnalysingSI:JACM2018} formalize Strong Session SI, which differs from Adya's SI~\cite{Adya:PhDThesis1999};
  Biswas and Enea~\cite{Complexity:OOPSLA2019} offer a different interpretation of Read Atomicity than that of Bailis et al.~\cite{RAMP:TODS2016}. 
As a result, the developers may implement isolation level $X$ as defined in formalism $A$, while adopting isolation level $Y$ from a different formalism $B$.

Overall, this suggests that supporting only a single isolation level or only those defined within a single formalism, as is common in existing checkers,  may limit their applicability to databases and applications with heterogeneous  isolation semantics. 
%However, few existing approaches provide a unified solution that supports a broad spectrum of isolation levels across multiple formalisms.


\inlsec{Our Solution}
%To address all these challenges, 
We present  \ourtool, a unified, black-box verifier that soundly, completely, and efficiently  verifies
a broad range of isolation levels across multiple formalisms in deployed databases.

\input{figs/eval/encode-cycle-width/encode-cycle-width-each}
\input{tables/encoding-cycle-width-23}
\input{tables/encoding-cycle-width-1234}

%(C1): key insight / idea; specifics.

%(C2): key insight / idea; specifics.

%(C3): key insight / idea; specifics.

\inlsec{Contributions}
Overall, we make the following contributions.

\begin{itemize}
	\item 
	\item 
	\item 
\end{itemize}







==> sections/intro-old.tex <==
\section{Old Introduction}
\red{[OLD introduction]}

\inlsec{Problems}

First,   inefficient checking that stems from (i) inherent high complexity (NP-complete); (ii) ; (iii) applying SMT solving with brute force.  Even the advance  solver MonoSAT, which is optimized for checking graph properties,  is a general-purpose SMT solver.   A direction application to the isolation checking problem would miss potential optimizations.

Second,  to simplify the checking problem,  existing work restricts workloads to unique values;  this is, however, not the case in practice.  For example,  it is common for concurrent users  to set the meeting point (value) of a road trip (key)  to the same place in  realistic workloads.
\nobi{also can occur when a client or database retries a write due to abortion?}
Moreover,   unique values narrows the test-case space, rendering the checking less effective (e.g., missing bugs that would occur otherwise). \cite{MariaDB-Bug}
Lifting this assumption would however result in much more uncertain dependencies. This exacerbates the solving overhead.

Third, \nobi{Isolation guarantees are evloving, from sql-92 to TCC, RA, ... diff formalisms, incomplete mixture, ... call for unified framework for checking ...}

\red{moved from Section 3:}
General transaction workloads
are   ubiquitous in practice, e.g., two employees concurrently adjust the inventory count of a product to the same value.
Moreover, production database, such as MySQL and MariaDB, %are often data-dependent and
have been found to expose isolation bugs that only manifest when multiple transactions write the same value to a key~\cite{MariaDB-Bug,MySQL-Bug}.
Therefore, a black-box isolation checker that can efficiently verify general histories is highly desirable.

\red{On list-append histories.}
Under the \uniqueval{} assumption,
\listappend{} histories are recoverable(every read can map to the unique write) and traceable(write orders are determined by list orders)\cite{Elle:VLDB2020}.
On general histories, however, we can say histories are not recoverable and partially traceable due to the partially repeated write values.

\red{On weaker isolation levels.}

\inlsec{Our Approach}

For Problem 1,  our insight: ...

our solution: efficient pruning and encoding techniques, together with  a dedicated SMT solver for verifying general transaction histories against isolation levels

For Problem 2, our insight: ...

our solution: universal polygraphs (UPs) to characterize isolation levels with general transaction workloads

To show our approach in place, we first \ser,

Additionally, \si; \ser for list-append histories

\inlsec{Contributions} \nobi{while our approach is independent of isolation levels, this work focuses on two stronger isolation levels, namely \ser and \si, whose ... NP-complete~\cite{Complexity:OOPSLA2019}.}
Overall,  we make the following contributions.

\begin{itemize}
\item we address the problem of black-box checking isolation levels for general transaction workloads. To do so, we propose universal polygraphs to characterize ...\nobi{new characterization}
\item we devise an efficient checking algorithm,  along with optimizations covering the main stages of the entire checking process
\item we demonstrate the generality of our approach by porting it to checking histories of read-write registers against \si and list-append against \ser.
\item tool implementation and integration into Jepsen.
we also conduct
extensive evaluation
\end{itemize}

\noindent Our experimental results show ...

==> sections/intro.tex <==
\section{Introduction} \label{section:intro}

Modern production databases provide transactional consistency guarantees to clients,
commonly referred to as isolation levels~\cite{TIS:Book2001},
such as (\textsc{Conflict}) \ser, \si~\cite{CritiqueSQL:SIGMOD1995}, and \rc.
For example, \ser ensures that all transactions appear to execute sequentially.
However, as Jepsen's analyses~\cite{Jepsen-Analyses} have revealed,
these consistency guarantees often fail in practice.
This raises concerns among database users about
whether a database truly provides the promised isolation level.
To address this, black-box testing emerges as a promising approach
for two reasons:
First, modern databases are often hosted in the cloud
(e.g., Amazon Aurora~\cite{Aurora} and Azure Cosmos DB~\cite{CosmosDB}),
limiting users' visibility into their internal mechanisms~\cite{Cobra:OSDI2020}.
Second, even for open-source databases
(e.g., PostgreSQL~\cite{PostgreSQL} and MySQL~\cite{MySQL}),
analyzing their concurrency control protocols
is high demanding, laborious, and error-prone~\cite{???}.

Black-box testing typically involves three steps:
\circled{1} A client generates a transaction \emph{workload},
consisting of transactions, each represented as a sequence of operations;
\circled{2} The workload is executed in the database,
producing a \emph{history} that records the returned values
associated with the workload;
and \circled{3} The resulting history is fed to a \emph{checker},
which checks whether it satisfies a specified isolation level.
The checking problems for \ser and \si in step \circled{3}
have shown to be \npc~\cite{ser, Complexity:OOPSLA2019},
primarily due to the uncertainties about \red{version order}.
Existing checkers achieves efficiency
either by encoding the checking problem into a constraint solving task
and leveraging an off-the-shelf SMT solver to solve it,
such as Cobra~\cite{Cobra:OSDI2020}, Viper~\cite{Viper:EuroSys2023},
and PolySI~\cite{PolySI:VLDB2023},
or by incorporating extra information into the history
to infer the version order more efficiently,
such as Elle~\cite{Elle:VLDB2020}, Emme~\cite{Emme:EuroSys2024},
MTC~\cite{Mini:ICDE2025}, and Chronos and Aion~\cite{TimeKiller:ICDE2025}.
\red{hfwei: What about dbcop?}

However, \emph{all} these existing checkers
rely on a key assumption called \uniqueval{}
about transaction workloads:
for each key, every write to the key assigns a unique value.
Although this assumption help associate each read
with the transaction that issues the corresponding write,
it greatly harms the practicality of checkers,
as real-world workloads, in contrast to the artifical workloads
in controlled experiments, often violate it.
\red{hfwei: How are these benchmarks configurable?}
For example, in RUBiS~\cite{CRUBis}, Twitter~\cite{CTwitter},
Courseware~\cite{ProvingSafety:ESOP20}, and YCSB~\cite{Benchpress:SIGMOD15},
it is common for multiple clients to write the same value to a key.
Moreover, certain isolation bugs are more likely to occur
only in the presence of duplicate write values,
as evidenced by bug reports for MySQL~\cite{MySQL-Bug} and MariaDB~\cite{MariaDB-Bug}.

\hfwei{How to introduce list-append workloads?}

In this work, we present \ourtool,
the first isolation checker capable of handling \emph{general} histories
which may contain duplicate write values.
We face both the \emph{characterization} and the \emph{efficiency} challenges
posed by general histories.
Specifically, without the \uniqueval{} assumption,
it is uncertain which write operation a read operation retrieves its value from.
Therefore, we need a novel characterization to caputure such uncertainties,
besides the uncertainties about the version order,
and efficient techniques to resolve them.
To this end, we make the following contributions:

\hfwei{To Review Below}

\begin{itemize}
  \item (Section~\ref{section:characterization})
    We propose \emph{universal polygraphs} (UPs),
    a novel graph-based characterization of \ser,
    by extending polygraphs~\cite{ser,Cobra:OSDI2020}
    to additionally caputure the $\WR$ uncertainties.
    A \emph{general} history satisfies \ser{}
    if and only if its universal polygraph is acyclic.
  \item (Section~\ref{section:ser-smt-theory})
    We design a dedicated SMT solver called \ourtool{} to
    check the acyclicity of universal polygraphs.
    It \red{TODO: CDCL here}.
    For high efficiency, we employ two optimization techniques
    based on empirical observations in conflict detection.
    \begin{itemize}
      \item \red{``Conflicts are rare. Be optimistic!''}
        First, we observe that although the cycle detection algorithms
        are frequently invoked, most of them do not trigger actual graph traversals
        because the newly added edges comform to the topological order
        of the current graph.
        Meanwhile, most graph traversals end up with conflicts (i.e., cycles)
        and thus backtrackings.
        To avoid graph traversals and thus conflicts as much as possible,
        \ourtool{} picks the polarity of a decision variable optimistically
        based on the pseudo-topological order of the current graph.
      \item \red{``Conflicts are small. Be Aggressive!''}
        Second, we observe that conflicting cycles typically have small width,
        meaning involving only a few edges associated with unique decision variables.
        Notably, more than $80\%$ of cycles are of $\le 4$-width.
        To avoid unnecessary conflict detection,
        \ourtool{} is aggressive at
        not only iteratively pruning 1-width cycles before encoding
        but also enumerating all remaining 2-width cycles
        and encoding the negation of the conjunction of these two variables into SMT formulas.
    \end{itemize}
  \item (Section~\ref{section:list})
    \red{list-append workloads}
  \item (Section~\ref{section:evaluation})
    We \red{show} the effectiveness of \ourtool in finding bugs
    through integrating \ourtool into the Jepsen framework,
    and we conduct an extensive assessment of \ourtool,
    demonstrating its efficiency in general histories.
\end{itemize}

==> sections/list-new.tex <==
% list-new.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Porting to List-append Histories}
\label{section:list}

\blue{[TODO: introduce what is list-append, 
why introducing list-append~\cite{Elle:VLDB2020}]}

In this section, we adapt the characterization of \ser{}
in Theorem~\ref{thm:ser-upg} for general read-write register histories
to general list-append histories.
% Due to space limitations,
% we only present the key ideas and theorems by \red{a running example},
% and leave a more formal and detailed description
% to \red{the full version}.

%%%%%%%%%%%%%%%%%%%%
\subsection{A Motivating Example}

\begin{figure*}[t]
  \centering
  \begin{subfigure}[b]{0.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plot/list-uv.pdf}
    \caption{A \uniqueval{} list-append history}
    \label{fig:list-uv}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.30\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plot/list-dup-constraints.pdf}
    \caption{A general list-append history with constraints}
    \label{fig:list-dup-constraints}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.30\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plot/list-dup-false-positive.pdf}
    \caption{An incorrect resolution}
    \label{fig:list-dup-false-positive}
  \end{subfigure}
  \caption{A motivaing example of list-append histories}
  \label{fig:lists-motivating}
\end{figure*}

Elle~\cite{Elle:VLDB2020} first introduces lists to infer the uncertain $\WW$ orders.
List-append histories support two types of operations: 
append $(\appendevent)$, which installs a value, 
and read $(\readevent)$, which returns a list of current installed values.
The order of list elements reflects the order they are installed, 
it can help recover $\WW$ relation.

Recall how Elle~\cite{Elle:VLDB2020} checks \ser of list-append histories.
Figure~\ref{fig:list-uv} shows a \uniqueval{} history. 
To checks its serializability, 
Elle builds a dependency graph and checks its acyclicity.
First, Elle identifies the $\WR$ dependency $T_2 \rel{\WR(x)} T_3$ 
by matching the last read value $3$ of $T_3$ with the append value $3$ of $T_2$.
Then, Elle recovers the $\WW$ dependency $T_1 \rel{\WW(x)} T_2$
from the list $[1, 2, 3]$ read by $T_3$, 
since the value $1$ appended by $T_1$ precedes the value $2$ appended by $T_2$.
The $\WR$ dependency of each value in the read list of $T_3$ is shown as red edges 
labeled with $\wr$ in lower letters.
The serializability is demonstrated  
because the recovered dependency edges do not form a cycle.

In the general case, 
the $\WW$ dependency becomes intractable.
Consider the history shown in Figure~\ref{fig:list-dup-constraints}, 
we cannot determine where $T_3$ reads from based solely on the last value.
This is because both $T_1$ and $T_2$ last appends $1$.
Following the spirit of universal polygraphs, 
we can capture the $\WR$ uncertainty with 
the constraint $\set{T_1 \rel{\WR(x)} T_3, T_2 \rel{\WR(x)} T_3}$; and 
similarly, the $\WW$ uncertainty between $T_1$ and $T_2$ with 
$\set{T_1 \rel{\WW(x)} T_2, T_2 \rel{\WW(x)} T_1}$.

Unfortunately, 
resolving such constraints alone is insufficient.
Consider a possible resolution $T_2 \rel{\WW(x)} T_1 \rel{\WR(x)} T_3$ 
(shown in Figure~\ref{fig:list-dup-false-positive}), 
which constructs an acyclic compatible graph.
However, this compatible graph do not satisfy the samentics of lists.
Since $T_2$ first installs the values $[2, 1]$, followed by $T_1$ installing $1$, 
the value read by $T_3$ should be $[2, 1, 1]$.

To make the inconsistency arise in the dependency graph, 
the key is to trace the $\WR$ dependency for each value in a list.
As shown in Figure~\ref{fig:list-dup-false-positive}, 
the value $2$ is installed by $\appendevent(x, 2)$ of $T_2$ 
and the last value $1$ is installed by $\appendevent(x, 1)$ of $T_1$.
However, there is another append operation $\appendevent(x, 1)$ 
that occurs after $\appendevent(x, 2)$ of $T_2$ (by $\po$ of $T_2$)
and before $\appendevent(x, 1)$ of $T_1$ (by $T_1 \rel{\WW(x)} T_2$), 
which contradicts the semantics of lists.
Consider a pair of neighboring values, 
$v_1$ and $v_2$, in a list.
Not only must $v_1$ be appended before $v_2$, 
but there must be no other values appended between them.
The inconsistency arises from the corresponding append operations.

This motivating example provides us two insights: 
(1) the $\WR$ dependency for each read value should be recovered, 
which requires a more fine-grained modeling over operations; 
(2) the $\WW$ dependency between append operations that read neighboring values 
should be constrained to respect the semantics of lists.

%%%%%%%%%%%%%%%%%%%%
\subsection{Unfolded Universal Polygraphs}

We propose \emph{unfolded universal polygraphs} to characterize list-append histories.

For a history $\H$, we unfold each of its read operations: 
for an operation $r \triangleq \readevent(x, [v_1, v_2, \cdots, v_n])$,
we unfold it into $n$ read operations $r'_0, r'_1, \cdots, r'_{n - 1}$, 
where $r'_0 \triangleq \readevent(x, [])$, $r'_1 \triangleq \readevent(x, [v_1])$, $\cdots$, 
$r'_{n - 1} \triangleq \readevent(x, [v_1, v_2, \cdots, v_{n - 1}])$.
These unfolded operations are ordered by the \bfit{append order} $\app(x)$, 
such that $r'_0 \rel{\app(x)} r'_1 \rel{\app(x)} \cdots r'_{n - 1} \rel{\app(x)} r$. 

%%%%%%%%%%%%%%%%%%%%
% [Unfolded Universal Polygraph]
\begin{definition} \label{def:unfolded-universal-polygraph}
  An \bfit{unfolded universal polygraph} $\G = (\V, \E, \C)$
  of a history $\H = (\T, \SO)$
  is a directed labeled graph $(\V, \E)$ called the \emph{known graph},
  together with a pair $\C$ of \emph{constraint sets} such that
  \begin{itemize}
    \item $\V$ corresponds to all operations of $\H$ additional with unfolded read operations;
    \item $\E \subseteq \V \times \V \times \type \times \Key$
      is a set of edges labelled with the type from
      $\type = \bset{\so, \po, \wr, \ww, \rw, \app}$ and the key from $\Key$.
    \item The constraint set $\wwcons = \Bset{\btuple{w \rel{\ww(x)} w', w' \rel{\ww(x)} w}
      \mid w = \appendevent(x, \_) \land w' = \appendevent(x, \_) \land w \neq w'}$.
    \item The constraint set $\wrcons = \Bset{\btuple{\bigcup\limits_{w_{i} = \appendevent(x, v)} \set{w_{i} \rel{\wr(x)} r}}
      \mid s = \readevent(x, [\sim, v])}$.
    % \item The constraint set $\appcons = \Bset{\btuple{r_i \rel{\app(x)} r_{i + 1}} \mid r \text{ and } r' \text{ are unfolded from the same }}$
  \end{itemize}
\end{definition}

In Definition~\ref{def:unfolded-universal-polygraph}, 
we use lower-letter labels to denote the relation between operations in distinguishment with transactions.
Notably, $\so \triangleq \bigcup\limits_{T \rel{\SO} S} O_T \times O_S$, 
extending the session orders between transactions.

Unfolded universal polygraphs (UUPGs) model the history at the operation level, rather than the transaction level.
To recover the $\WR$ dependency of each value in a list, 
UUPGs leverage the $\WR$ constraints of each unfolded read operations, 
providing a unified approach to recover the $\WR$ dependency as the last value of a list.

%%%%%%%%%%%%%%%%%%%%

\subsection{Unfolded Universal Polygraph-based Characterization of \ser}
\label{ss:ser-uupg}

A compatible graph of an unfolded universal polygraph 
satisfies all constraints that from universal polygraphs, 
additional with the constraint from the append order.

%%%%%%%%%%%%%%%%%%%%
% [Compatible Graphs with a Universal Polygraph]
\begin{definition} \label{def:compatible-graphs-with-an-unfolded-universal-polygraph}
  A directed labeled graph $\G' = (\V', \E')$ is \bfit{compatible with
  an unfolded universal polygraph} $\G = (\V, \E, \C)$ if
  \begin{itemize}
    \item $\V' = \V$;
    \item $\E' \supseteq \E$ such that 
      \begin{enumerate}
        \item $\forall x \in \Key.\; \forall w, w', r \in \V'.\;
          w \rel{\wr(x)} r \land
          w \rel{\ww(x)} w' \implies r \rel{\rw(x)} w'$; and
        \item $\forall x \in \Key.\; \forall w, w', r, r' \in \V'.\;
          w \rel{\wr(x)} r \land 
          w' \rel{\wr(x)} r' \land 
          r \rel{\app(x)} r' \implies w \rel{\ww(x)} w'$ and 
          there is no such $w''$ that 
          $w \rel{\ww(x)} w'' \land w'' \rel{\ww(x)} w' \in \E'$
        % [This is ensured by SO.]
        % \item $\forall x \in \Key.\; \forall w, w' \in \V'.\;
        %   w' \in \opsof_{T_{\bot}} \implies (w, w', \WW, x) \notin \E'$;
      \end{enumerate}
    \item $\forall \consvar \in \wwcons.\;
      |\E' \cap \consvar| = 1$; and
    \item $\forall \consvar \in \wrcons.\;
      |\E' \cap \consvar| = 1$.
  \end{itemize}
\end{definition}
%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{plot/list-dup-solution.pdf}
  \caption{A compatible graph of UUPG of the history shown in Figure~\ref{fig:list-dup-constraints}}
  \label{fig:ex-uupg}
\end{figure}

%%%%%%%%%%%%%%%%%%%%
\begin{example}
  Figure~\ref{fig:ex-uupg} shows a compatible graph of the general history 
  presented in the motivating example
  UUPG unfolds read operation $\readevent(x, [1, 2, 3])$ into three read operations 
  and connects them via $\app(x)$.
  Each $\wr$ dependency between read operations linked by an $\app$ edge 
  requires a corresponding $\ww$ edge in the same direction
  with no interleaving write operations.
  Notably, we consider the initialization transaction $T_\bot$
  with a special value $\emptypost$, 
  from which $[]$ is read.
  $\so$ edges between $T_\bot$ and other transactions are omitted.
\end{example}
%%%%%%%%%%%%%%%%%%%%

% Note that a compatible graph with a UUPG maps to a compatible graph over transactions.
% This mapping is straightforward.

%%%%%%%%%%%%%%%%%%%%
\begin{theorem}[Unfolded Universal Polygraph-based Characterization of \ser{}]
  \label{thm:ser-uupg}
  A history $\H$ satisfies \emph{\ser{}} if and only if
  there exists a graph $\G'$ compatible with
  the unfolded universal polygraph of $\H$ 
  such that $\G'$ is acyclic and \blue{$(\G' - \unfoldedreadops) / \txnequivalence$ is acyclic}.
\end{theorem}
%%%%%%%%%%%%%%%%%%%%

To establish the correctness theorem between compatible graphs and isolation levels, 
we have to return to the $\vis$, $\ar$-based definition. 
The definition of the \ser of a list-append history 
and the proof of Theorem~\ref{thm:ser-uupg} are left in the appendix~\cite[Appendix XX]{tech-rpt}. 


==> sections/list.tex <==
% list.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Porting to List-Append Histories}
\label{section:list}

\blue{[TODO: introduce what is list-append, 
why introducing list-append~\cite{Elle:VLDB2020}]}

In this section, we adapt the characterization of \ser{}
in Theorem~\ref{thm:ser-upg} for general read-write register histories
to general list-append histories.
Due to space limitations,
we only present the key ideas and theorems by \red{a running example},
and leave a more formal and detailed description
to \red{the full version}.

\hfwei{TODO: need a more comprehensive running example}
%%%%%%%%%%%%%%%%%%%%
\subsection{Unfolded Universal Polygraphs}

\input{figs/list-append.tex}

The key difference between read-write register and list-append histories
is that the list returned by a (list) read operation in a list-append history
reflects the order of the (list) append operations
that install these list elements.
However, for general list-append histories,
i.e., without the \uniqueval{} assumption,
it is not clear a list element is installed by which append operation
when multiple append operations have installed the same element.

\begin{example}
  \label{ex:list-append-history}
  Consider the history of Figure~\ref{fig:list-append-history}.
  From the list read operation $\readevent(x, [1, 2, 1])$
  of transaction $T_{4}$,
  we know that $T_{2}$ reads the value 2 from $T_{4}$
  and $T_{2}$ happens between $T_{1}$ and $T_{3}$,
  but we cannot determine the order between $T_{1}$ and $T_{3}$.
\end{example}

To capture the order between append operations
enforced by the list elements observed by list read operations,
we introduce the \emph{unfolded universal polygraph} (UUPG)
which explicitly exposes the \emph{list order} of list elements.

\begin{example}
  \label{ex:unfolded-list-append-history}
  To expose the \emph{list order} of the list elements observed by
  the operation $\readevent(x, [1, 2, 1])$ of transaction $T_{4}$,
  we \emph{unfold} it into three operations
  (as shown in Figure~\ref{fig:unfolded-list-append-history}):
  $\readeventunfolded(x, [1])$, $\readeventunfolded(x, [1, 2])$,
  and $\readeventunfolded(x, [1, 2, 1])$,
  each per list element.
  These three operations are ordered by the list order $\lo(x)$,
  and the last one is ordered before
  the list append operation $\appendevent(y, 3)$ of transaction $T_{4}$
  by the program order $\po$.
\end{example}

Now we define the unfolded universal polygraph (UUPG)
of an unfolded list-append history,
which \red{captures}

\begin{example}
  \label{ex:unfolded-uupg}
  Figure~\ref{fig:list-append-uupg} 
  \begin{itemize}
    \item The $\WR$ constraint $\wrcons$:
      For each (\red{unfolded}) operation $\readeventunfolded(x, [\ldots, v])$
      and a set of append operations $\appendevent(x, v)$,
      add the ``exactly-one'' constraint similar to that in universal polygraphs.

      \begin{itemize}
        \item For $\readevent(y, [3])$ of transaction $T_{2}$,
          we have $T_{4} \rel{\WR(x)} \red{T_{2}}$.
        \item For $\readeventunfolded(x, [1, 2])$,
          we have $T_{2} \rel{\WR(x)} \readeventunfolded(x, [1, 2])$.
        \item For $\readeventunfolded(x, [1])$
          (and similarly for $\readeventunfolded(x, [1, 2, 1])$),
          we know that it reads 1 from either $T_{1}$ or $T_{3}$,
          but not both.
          In similar terminology as in universal polygraphs,
          we write $\set{T_{1} \rel{\WR(x)} \readeventunfolded(x, [1]),
          T_{3} \rel{\WR(x)} \readeventunfolded(x, [1])} \in \wrcons$.
          % Formally,
          % $(T_{1} \rel{\WR(x)} \readeventunfolded(x, [1]) \lor
          %  T_{3} \rel{\WR(x)} \readeventunfolded(x, [1])) \land
          %  (\lnot T_{1} \rel{\WR(x)} \readeventunfolded(x, [1]) \lor
          %  \lnot T_{3} \rel{\WR(x)} \readeventunfolded(x, [1]))$.
      \end{itemize}
    \item The $\WW$ constraint $\wwcons$:
      The three transactions that contain the append operations on list $x$
      should be totally ordered.
      For example, for the pair $T_{1}$ and $T_{3}$,
      we have $\set{T_{1} \rel{\WW(x)} T_{3}, T_{3} \rel{\WW(x)}} \in \wwcons$.
    \item The $\lo$ constraint $\locons$:
      Suppose that $T_{1} \rel{\WR(x)} \readeventunfolded(x, [1])$
      and $T_{2} \rel{\WR(x)} \readeventunfolded(x, [1, 2])$.
      Since $\readeventunfolded(x, [1]) \rel{\lo(x)} \readeventunfolded(x, [1, 2])$,
      it should be that $T_{1} \rel{\lo(x)} T_{2}$.
      Such constraints apply to all unfolded operations
      that are ordered by the list order.
    % \item The $\RW$ constraint $\rwcons$:
  \end{itemize}

\centerline{\hfwei{====================TODO====================}}

  Note that we do \emph{not} enforce the following two kinds of constraints:
  \begin{itemize}
    \item First, we do not require the list order $\lo$
      imply the \emph{immediate} 
    \item No more than one (unfold or not) operations
      in the same transaction can read from the same append operation
  \end{itemize}

  \hfwei{TODO: $\lo \subseteq \po$?}
\end{example}
%%%%%%%%%%%%%%%%%%%%
\subsection{Characterizing \ser{} for General List-Append Histories}
\label{ss:ser-uupg}

%%%%%%%%%%%%%%%
\subsubsection{Assumptions on List-Append Histories}
\label{sss:list-append-history-assumptions}

To highlight our key idea, we assume \listappend{} histories satisfy the ``\singlewrite'' assumption in this paper.
That is, each transaction contains no more than one append operation on each key.
\zhiheng{``\singlewrite'' helps avoid a complex but meaningless string-matching problem, shall we discuss it later?}
%%%%%%%%%%%%%%%
\subsubsection{Axioms for List-Append Histories}
\label{sss:list-append-history-axioms}

\paragraph*{The $\intaxiom$ Axiom}
all reads before the possible append operation read the same value $l$ (is a list),
and all reads after the possible operation read the same value $l'$ too.
If the append operation exists and it appends value $v$, then $l' = l \concat [v]$, otherwise $\intaxiom$ is violated.
Thus we reorganize transactions to a single read and a followed write form for each key,
and defined the semantics of $\vdash$ on top of the reorganized form.
$T \vdash \writeevent(\keyxvar, \valvar)$ means transaction $T$ appends $\valvar$ to key $\keyxvar$.
$T \vdash \readevent(\keyxvar, l)$ means transaction $T$ reads value $l$(is a list) from key $x$ before the possible append,
that is, if  $T$ actually reads $l \concat [v]$ after $\appendevent(x, v)$, then we also regard $T \vdash \readevent(\keyxvar, l)$.

\paragraph*{The $\listprefixaxiom$ Axiom}

\hfwei{TODO: do we need this axiom for correctness (not for performance)}
If there exists two reads on a same key in a history,
one reads $[1, 2, 3]$, but another reads $[1, 3, 2]$,
then this history must not satisfy \ser.

either $l_1$ is a prefix of $l_2$ or $l_2$ is a prefix of $l_1$.

%%%%%%%%%%%%%%%%%%%%
% [Construct Value]
\begin{definition} \label{def:construct-value}
  For a transaction $T$ in history $\H$ and a key $\keyxvar$,
  $$
  \constructvalue(T, x) =
  \left\{\begin{matrix}
    [] & T \not\vdash \readevent(\keyxvar, \_) \land T \not \vdash \writeevent(\keyxvar, \_) \\
    [v] & T \not\vdash \readevent(\keyxvar, \_) \land T \vdash \writeevent(\keyxvar, v) \\
    l & T \vdash \readevent(\keyxvar, l) \land T \not \vdash \writeevent(\keyxvar, \_) \\
    l \concat [v] & T \vdash \readevent(\keyxvar, l) \land T \vdash \writeevent(\keyxvar, v)
    \end{matrix}\right.
  $$
\end{definition}
%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%
% [Longest Value]
\begin{definition} \label{def:longest-value}
  For a history $\H = (\T, \SO)$ and a key $\keyxvar$, \\
  $\longestvalue(x) = l$ such that
  \begin{itemize}
    \item $\exists\; T. \; \constructvalue(T, x) = l$; and
    \item $\forall\; S \in \T. \; \\
      \length(\constructvalue(S, x))
      \leq \length(\constructvalue(T, x))$.
  \end{itemize}
\end{definition}
%%%%%%%%%%%%%%%%%%%%

Based on $\longestvalue$, observer transactions can be precisely defined.

For breivity, we use $\unittxn{\readevent(\keyxvar, l)}$ to represent an observer transaction
that contains the only read operation $\readevent(\keyxvar, l)$.
Formally, $\unittxn{\readevent(\keyxvar, l)} \triangleq
(\opset \triangleq
\set{\readevent(\keyxvar, l)}, \po \triangleq
\emptyset)$.
\zhiheng{taking the $(\opset, \po)$ definition of txn as PolySI}
We use $\Key(\H)$ to represent all keys that appeared in $\H$.
We use $\allprefix(l = [l_1, l_2, \ldots, l_n])$ to represent all prefixes of list $l$,
formally written in $\bset{[], [l_1], [l_1, l_2], \ldots, [l_1, l_2, \ldots, l_n]}$.

%%%%%%%%%%%%%%%%%%%%
% [Observers-Complementary History]
\begin{definition} \label{def:observers-complementary-history}
  Given history $\H = (\T, \SO)$, $\H$'s \bfit{observer-complementary history}
  $\Hplus = (\T \cup (\bigcup\limits_{\keyxvar \in \Key(\H)} \bset{\unittxn{\readevent(\keyxvar, l)} \mid l \in \allprefix(\longestvalue(\keyxvar))}), \SO)$
\end{definition}
\zhiheng{if existing read txns are required to not be added into the raw history, then more constraints on prefixes should be added here, which in turn makes the definition more complex}
%%%%%%%%%%%%%%%%%%%%

Observers-complementary histories help us establish matching relationships between appends and list elements.
To identify those obserser transactions and recover $\LO$ orders, we let $\observers(\H) = \set{T \mid T \in \T_{\Hplus} \land T \notin \T_{H}}$.

\zhiheng{example? how about draw a complete figure in overview?}

\inlsec{The Characterizing Theorem}

%%%%%%%%%%%%%%%%%%%%
% [Universal Polygraph on List-Append Histories]
\begin{definition} \label{def:universal-polygraph-list-append}
  A \bfit{universal polygraph} $G = (V, E, C)$ associated with a \listappend{} history $\H = (\T, \SO)$
  is a directed labeled graph $(V, E)$ with relating keys called the \emph{known graph}
  together with a pair of constraints set $C$ of \emph{universal constraints}
  consisting of a $\WW$ constraints set $\wwcons$ and a $\WR$ constraints set $\wrcons$
  such that
  \begin{itemize}
    \item $V$ corresponds to all transactions in the history \red{$\Hplus$};
    \item $E \subseteq V \times V \times \type \times \Key$ is a set of edges with labels (i.e., types)
    from $\type = \set{\SO, \WR, \WW, \RW, \red{\LO}}$ and relating keys from $\Key$; and
    \item $C = (\wwcons, \wrcons)$ where
    \begin{itemize}
      \item $\wwcons = \bset{\btuple{(T, S, \WW, \keyxvar), (S, T, \WW, \keyxvar)}
      \mid T \in \WriteTx_{\keyxvar} \land S \in \WriteTx_{\keyxvar} \land T \neq S}$; and
      \item $\wrcons = \bset{\btuple{(T_1, S, \WR, \keyxvar), (T_2, S, \WR, \keyxvar), \ldots, (T_n, S, \WR, \keyxvar)}
      \mid S \vdash \readevent(\keyxvar, \red{l}) \land
      \forall T \in \set{T_1, T_2, \ldots, T_n}.\; T \vdash \writeevent(\keyxvar, \red{\lastele(l)})}$.
    \end{itemize}
  \end{itemize}
\end{definition}
%%%%%%%%%%%%%%%%%%%%

The definition of compatible graph is kept, and we try to add more properties to compatible graphs of \listappend{} problem.

%%%%%%%%%%%%%%%%%%%%
% [LO-WW Property of a compatible graph]
\begin{definition} \label{def:LO-WW-property}
  A directed labeled graph with relating keys $G' = (V', E')$ satisfies \bfit{$\LOtoWW$ property} if
  \begin{itemize}
    \item $\forall\; T, S \in \observers(\H). \;
      T \vdash \readevent(\keyxvar, l) \land S \vdash \readevent(\keyxvar, l \concat [v])
      \to (T, S, \LO, \keyxvar) \in E'$; and
    \item $\forall\; T, S, T', S' \in V'.\;
      (T', T, \WR, \keyxvar) \in E' \land (S', S, \WR, \keyxvar) \in E' \land (T, S, \LO, \keyxvar) \in E'
      \to (T', S', \WW, \keyxvar) \in E'$.
  \end{itemize}
\end{definition}
\zhiheng{imprecise, for we have lost info of history here}
%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%
% [WR-Value Property of a compatible graph]
\begin{definition} \label{def:WR-value-property}
  A directed labeled graph with relating keys $G' = (V', E')$ satisfies \bfit{$\WRValue$ property} if
  $\forall\; T, S, T', S' \in V'.\;
    T \vdash \readevent(\keyxvar, l) \land S \vdash \readevent(\keyxvar, l) \land
    (T', T, \WR, \keyxvar) \in E' \land (S', S, \WR, \keyxvar) \in E' \to
    T' = S'$.
\end{definition}
%%%%%%%%%%%%%%%%%%%%

Finally we come to the characterizing theorem of \listappend{} histories,
which is associated with $\LOtoWW$ and $\WRValue$ properties.

%%%%%%%%%%%%%%%%%%%%
\begin{definition} \label{def:list-append-ser-acyclic}
  Let $G = (V, E, C)$ be a universal polygraph of a \listappend{} history $\H$.
  If there exists at least one compatible graph that satisfies $\RWDerive$, $\LOtoWW$ and $\WRValue$ properties and is acyclic when edge types and keys are ignored,
  then $G$ is \bfit{list-append-\ser-acyclic}.
\end{definition}
%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%
\begin{theorem}[Universal Polygraph-based Characterization of \ser{} on \listappend{} Histories] \label{thm:universal-polygraph-list-append-ser}
  A history $\H$ satisfies \emph{\ser{}} if and only if
  \emph{$\H \models \intaxiom$} and the universal polygraph of $\H$ is list-append-\ser-acyclic.
\end{theorem}
%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%
\subsection{Implementation and Optimizations}
\label{ss:impl-opt}

\begin{itemize}
  \item list-prefix axiom
  \item unfold only the longest list for each key?
\end{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/opt-motivation.tex <==
% opt-motivation.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Dedicated SMT Solver-based Serializability Checking}
\label{section:ser-smt-theory}

In this section, we describe our dedicated SMT solver,
called \ourtool, for serializability checking.
%%%%%%%%%%%%%%%%%%%%
\subsection{Motivation}
\label{ss:motivation}

We motivate our design of \ourtool by exploring
how MonoSAT implements cycle detection \red{into the framework of SAT solving}
and how to accelerate the solving process \red{for serializability checking}.

%%%%%%%%%%
\subsubsection{Cycle Detection in MonoSAT}
\label{sss:monosat-cycle-detection}

As shown in Figure~\ref{fig:ser-monosat-framework},
MonoSAT implements cycle detection
within the well-known CDCL(T) (Conflict-Driven Clause-Learning)
framework~\cite{Chaff:DAC01}.
MonoSAT iteratively picks a \emph{decision variable}
to obtain a current partial assignment $\pa$
for its frontend SAT solver,
and passes it to the backend theory solver.
The theory solver \red{incrementally maintains} a directed graph
corresponding to $\pa$
and performs the incremental PK algorithm~\cite{PKTopo:ACMJEA2006}
on the graph for \emph{cycle detection}.
If a cycle is detected,
the theory solver generates a conflict clause
and returns it to the SAT solver,
helping the SAT solver avoid encountering \red{the same conflict} again.
MonoSAT terminates once a valid model is found
(meaning that the history is serializable),
or an unresolvable conflict is encountered
(meaning that the history is unserializable).

The PK algorithm~\cite{PKTopo:ACMJEA2006} maintains 
a dynamic \emph{pseudo-topological} order for all vertices,
denoted as $\clevel{\cdot}$.
When an edge $(\fromvar, \tovar)$ is added, 
PK first checks if $\clevel{\fromvar} < \clevel{\tovar}$.
If this condition holds, 
then PK deems adding $(\fromvar, \tovar)$ does not create any cycle,
otherwise it performs a two-way search to 
(i) confirm that vertex $\tovar$ is actually not reachable from vertex $\fromvar$ in the current graph, and
(ii) update the $\clevel{\cdot}$ values of these visited vertices
to ensure $\clevel{\fromvar}' < \clevel{to}'$,
thus \red{preventing unnecessary future graph traversals}.

%%%%%%%%%%
\subsubsection{Accelerating Searching by Knowledges Gained from Cycle Detection}
\label{sss:cycle-detection-acceleration}

% \blue{
% \begin{itemize}
% 	\item First, 
% 	a common sense that less conflict lead to more efficient solving time 
% 	(cite some literature).
% 	To guide our solver to avoid running into a conflict, 
% 	we analyze each conflict, try to find the key (minimized) reason.
% 	We find the key reason are very "small",
% 	i.e. caused only by 1 or 2 variables.
% 	Literature xxx has demonstrated the effectiveness 
% 	of unit propagation in accelerating the solving process of SAT solving.
% 	Therefore, 
% 	we directly prune the 1-width cycles before encoding when possible and 
% 	encode most of the 2-width cycles into the SAT formula
% 	(consider how to link pruning and encoding together);
% 	\item Second,
% 	in most of calls that activates the two-way search,
% 	no cycle is found, but disrupt the pseudo-topological order.
% 	We radically prevent such calls by heuristically picking polarity 
% 	according to the dynamic maintained pseudo-topo order.
% \end{itemize}
% }

Consider the solving process of an encoded universal polygraph  
but without the $\acyclicencoding$ predicate,
the SAT solver will go directly to a valid model without encountering any conflict.
Therefore,
the key part of solving lies in the cycle detection process 
of the off-the-shelf SMT solver-based serializability checking.
\blue{[connection between encountering a conflict and efficient solving]
Although CDCL(T) perfers higher-quality conflicts over merely reducing their number, 
in this problem, we observe that a lower number of conflicts generally 
results in reduced solving time.}
\ourtool focus on accelerating the solving process
by reducing the frequency of running into a conflict.
This is based on the following two observations.

% We accelerate the solving process by 
% (i) guiding the solver to avoid running into a conflict from prodominent reasons; and 
% (ii) (radically) preventing the "drawback" reordering of the pseudo-order.

% As demonstrated in Figure~\ref{fig:monosat-cycle-detection},
% the graph traversals in cycle detection is a major performance bottleneck
% in off-the-shelf SMT solver-based serializability checking.
% \zhiheng{The bottleneck is not graph traversal.
% We have to tell a new story.}
% \ourtool focuses on accelerating cycle detection
% by reducing the frequency of graph traversals in the PK algorithm.
% This is based on the following two observations
% on the behavior of cycle detection in MonoSAT
% \red{for serializability checking}.

\begin{itemize}
  \item First, most of the cycles detected are in small width
		(the number of variables of the conflict clause, 
		defined in Section~\ref{sss:cycle-width})
	  in the sense that they are caused by only a few
		(e.g., no more than 2) \red{uncertain boolean variables}.
		Using propagation instead of conflict resolution to 
		address these conflicts has been demonstrated to be effective 
		in reducing solving time~\blue{\cite{Zord:PLDI2021,Deagle:OOPSLA2022,MMEncoding:OOPSLA2023}}.
		In \ourtool, we directly prune the 1-width cycles
		\emph{before} encoding when possible
		and encode most of the 2-width cycles
		into the SAT formula.
  \item Second, in most of calls that \red{activates} the two-way search, 
    cycles are detected; however, many of these are unnecessary to explore and can be avoided by 
		carefully selecting the corresponding decision variable.
    To minimize such calls,
		\ourtool heuristically picks a decision variable in the SAT solver
		that is \red{less likely} to \red{form a cycle},
		by utilizing the \emph{pseudo-topological order} of the current graph
		dynamically maintained by the theory solver.
	\item \hfwei{TODO: for the backend theory solver?}
\end{itemize}

\hfwei{TODO: (1) based on MonoSAT instead of from the scratch???
(2) first, second => second, first???}
%%%%%%%%%%%%%%%%%%%%

==> sections/opt-others.tex <==
% opt-others.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Other Optimizations}

\input{appendix/other-opts}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/overview.tex <==
% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=\columnwidth]{figs/isolation-solver-framework.pdf}
% 	\caption{Detailed workflow of  history verification in \ourtool.
%   Those optimized stages are specially colored.
%   A box colored \coloredbox[performanceoptcolor]{\phantom{XX}} indicates this is (mainly) a performance optimization.
%   A box colored \coloredbox[designoptcolor]{\phantom{XX}} indicates this is (mainly) a design optimization.
%   }
% 	\label{fig:hist-verif-workflow}
% \end{figure}

\begin{figure*}[t]
	\centering
	\includegraphics[width=\textwidth]{figs/isolation-solver-framework-w-cobra.pdf}
	\caption{Detailed workflow of history verification in \ourtool.
  Those optimized stages are specially colored.
  \zhiheng{revise framework, remove others}
  }
	\label{fig:mamba-w-others}
\end{figure*}



\section{Overview(Outdated)} \label{section:overview}

3.1: motivating example for general transaction workloads; summary of our solution

3.2: motivating example(s) for  missing optimization(s); summary of our solutions

\nobi{if it's hard to summarize the above two points, we can follow polysi to introduce our approach inline. For example, 3.1 would be sec 4.1}


\subsection{\ser{} Checking Against the ``\uniqueval'' Assumption}
\nobi{move to example 2.1}

Let's start with a simple \uniqueval{} history $H_1$ (Figure ~\ref{fig:rw-checking-h1}).
To check whether it satisfies some isolation level(say, \ser{}), the key problem is to figure out the happens-before order of transactions, or to judge it's impossible.
In $H_1$, $t_3$ reads the value written by $t_1$ on key $x$ and $t_2$ on key $y$.
This implies $t_3$ happens after $t_1$ and $t_2$. 
We use $t_1 \rel{\WR(x)} t_3$ and $t_2 \rel{\WR(y)} t_3$ to denote this ``read-from'' relationship.

Another relationship that cannot be determined directly is the writing order between $t_1$ and $t_2$ on key $x$. 
That is, whether $t_1 \rel{\WW(x)} t_2$ or $t_2 \rel{\WW(x)} t_1$. 
We use a constraint to capture this $\WW$ uncertainty, denoted as $\btuple{t_1 \rel{\WW(x)} t_2, t_2 \rel{\WW(x)} t_1}$.
An instantianted $\WW$ relationship can derive more precedence with $\WR$.
For example, $t_1 \rel{\WW(x)} t_2$, then it's sufficient to see $t_3$ happens before $t_2$, for $t_2$ modifies the value of key $x$ that is read by $t_3$. 
This kind of relationship is denoted as $t_3 \rel{\RW{(x)}} t_2$.
Here $t_3 \rel{\RW(x)} t_2 \rel{\WR(y)} t_3$ forms a cycle(blue edges in Figure ~ \ref{fig:rw-checking-h1}), which means it's impossible to determine whether $t_2$ or $t_3$ happens first.
Then we returns to $t_2 \rel{\WW(x)} t_1$(red edge in Figure ~\ref{fig:rw-checking-h1}), the rest choice of $\btuple{t_1 \rel{\WW(x)} t_2, t_2 \rel{\WW(x)} t_1}$. 
It would not derive any $\RW$ relationship.
After all constraints are instantianted and all $\RW$ edges are derived, a valid happens-before order $[t_2, t_1, t_3]$ is figured out by toposorting on the graph. % TODO: where's the concept of graph?
This implies $H_1$ actually satisfies \ser{}.

PolySI \cite{PolySI:VLDB2023} used generalized polygraph to capture above $\WW$ uncertainty. 

% TODO: introduce generalized polygraph, WW constaint, Adya's formal definition

\subsection{Capturing $\WR$ Uncertainty}

Now we move to the ``non-\uniqueval'' situation.
$H_2$ (Figure ~\ref{fig:rw-checking-h2-constraints}), that is slightly modified from $H_1$, violates the ``\uniqueval'' assumption, for both $t_1$ and $t_3$ writes value $1$ on key $x$.
In this case, it's unable to know where $t_3$ is read from trivially, but whether $t_1$ or $t_2$.
We use another constraint to capture this $\WR$ uncertainty, denoted as $\btuple{t_1 \rel{\WR(x)} t_3, t_2 \rel{\WR(x)} t_3}$.
Along with the retained $\btuple{t_1 \rel{\WW(x)} t_2, t_2 \rel{\WW(x)} t_1}$ constraint capturing $\WW$ uncertainty, 
it's capable to figure out whether transactions in $H_2$ can be sorted to a happens-before order that satisfies $\ser{}$.

Against the ``\uniqueval'' assumption, $\RW$ relations can be derived by $\WW$ relations directly, for all $\WR$ relations are determined.
But in general workload like $H_2$, $\RW$ relations have to be derived by $\WW$ and $\WR$ together.
For example, as Figure ~ \ref{fig:rw-checking-h2-conflict} shows, if $t_1 \rel{\WW(x)} t_2$ and $t_1 \rel{\WR(x)} t_3$ are instantianted, then $t_3 \rel{\RW(x)} t_2$ is derived.
It forms a cycle with $t_2 \rel{\WR(y)} t_3$, which drives to conflict.

Figure ~ \ref{fig:rw-checking-h2-solution} shows a valid solution to $H_2$, that is $t_2 \rel{\WW(x)} t_1$ and $t_1 \rel{\WR(x)} t_3$.
In this solution, no $\RW$ relationship would be derived and the whole graph remains acyclicity.
There may exist multiple valid happens-before orders of a history.
If there exists at least 1, then we accept this history as it satisfies $\ser{}$.
(Another concern is, if in the database, $t_3$ actually read from $t_1$ and $t_2$ actually happens after $t_1$, then we misjudges $H_2$. 
But this is somehow reasonable, for we're totally blind of database internals.)

We define universal polygraph on top of generalized polygraph to capture $\WR$ uncertainty carried out by repeat write values, see chapter XXX for specific information.

\subsection{Handling the Overwritten Problem of ``non-\uniqueval'' List-Append}
\nobi{move to later section }

Another common mode of database history is list-append.
Against the ``\uniqueval'' assumption, it can be easily reduced to a problem on RW Registers.
Taking the ``Append'' operation as ``Write'' and using the last element read from lists as the ``Read'' value, 
the known precedence and constraints can be constructed as above.
Furthur more, we can exploit writing orders from lists read, which help us solve most of the $\WW$ constraints. % TODO: solve?

% TODO: merge fig3 and fig4, rewrite this paragraph
Figure ~ 3 shows a simple list-append history $H_3$ which satisfies ``\uniqueval''.
Figure ~(3b) shows the reduction from previous list-append history $H_3$ to RW-Register history $H_3'$.
In $H_3'$, there's an explicit $\WR$ relationship $t_1 \rel{\WR(x)} t_4$ only considering the last element $3$ of read value, an inherent $\RW$ relationship $t_4 \rel{\RW(y)} t_2$
\footnote{It can be seen as an initializing transaction $t_0$ that writes $[]$ on key $y$. $t_4 \rel{\RW(x)} t_2$ is derived from $t_0 \rel{\WR(y)} t_4$ and $t_4 \rel{\WW{(y)}} t_2$. }
 and $\WW$ constraints pair-wisely between $t_1$, $t_2$ and $t_3$ on key $x$.

Additional information is the list order $[1, 2, 3]$ read in $t_4$, which implies writing order $t_3 \rel{\WW(x)} t_2 \rel{\WW(x)} t_1$.
A cycle $t_4 \rel{\RW(y)} t_2 \rel{\WW(x)} t_1 \rel{\WR(x)} t_4$ implies that $H_3$ does not satisfy $\ser{}$. 
Thanks to list orders, there's no need to guessing, trying and furthur checking constraints.

When it comes to the ``non-\uniqueval'' workload, it's not sufficient to only consider the last element, for values may be overwritten.
We show details of this overwritten problem in Figure ~(3c).
Figure ~ (3c) shows a general list-append history $H_4$.
$H_4$, that is also slightly modified from $H_3$, retains the implicit $t_4 \rel{\RW(y)} t_2$ relationship as $H_3$.
In $H_4$, whether $t_4$ reads from $t_1$ or $t_3$, it's impossible for $t_4$ to read $2$ on key $x$, which implies $H_4$ must not satisfy $\ser{}$. 
However, Figure ~(3c) also shows a possible solution of $H_4$, for making $t_4$ reads from $t_1$.
Actually, if $H_3$ runs as the topological order shown in Figure ~(3c), the value $t_4$ read is $[1]$, instead of current $[1, 2, 1]$.
When only considering the last element, previous part of list is wiped out by overwriting.
Against the ``\uniqueval'' assumption, it's sufficient to use the last element of a list to uniquely represent the whole list(or a prefix).
This reduction technique relies so much on ``\uniqueval'' that it does not stand any more under general workload. 
Another associated problem is the lost of information provided by list orders.
Given the list order $[1, 2, 1]$, it's only possible to know someone, $t_1$ or $t_3$, happens before $t_2$, and another one happens after $t_2$. 
It's hard to encode this ``someone'' constraint as well. 

To solve the overwritten problem and recover information from list orders, we introduce observer transactions into the previous history.
Intuitively, if at some point key $x$ is read as $[1, 2, 1]$, then at some other points, it's able to read $[1]$, $[1, 2]$ and $[1, 2, 1]$ on key $x$.
We make these implicit states observable by introducing transactions that contains a single read on key $x$ with read value $[1]$, $[1, 2]$ and $[1, 2, 1]$, namely $o_1$, $o_2$ and $o_3$ respectively in Figure ~(4d).
These observers would not change whether $H_4$ satisfies $\ser{}$.
A obvious type of relationships is the happens-before order between observers, for example, $o_1$ happens before $o_2$ for $o_2$ reads more elements than $o_1$.
This relationship type is called $\LO$(List Order).
To leverage the transitivity of $\LO$, only adjacent $\LO$ relationships are added. Here ``adjacent'' means the lists differ exactly 1 in length.
New read transactions would introduce more $\WR$ constraints, our target is trying to establish the matching relationship between appends and reads by $\WR$ constraints.
For example, $t_3 \rel{\WR(x)} o_1$ indicates the write in $t_3$ construct the first element of key $x$.
In this way, $\WR$ relationships toward observers is able to imply writing orders of write transactions, where information from list orders can be recovered.
For example, if $t_3 \rel{\WR(x)} o_1$, $t_2 \rel{\WR(x)} o_2$ and $o_1 \rel{\LO(x)} o_2$, then $t_3$ must happen before $t_2$, otherwise the list order $[1, 2]$ is violated.
That is the $\LOtoWW$ property, formally written in $t_i \rel{\WR(k)} o_i \land t_j \rel{\WR(k)} o_j \land o_i \rel{\LO(k)} o_j \rightarrow t_i \rel{\WW{(k)}} t_j$. 
Finally, we fix the $t_3 \rel{\WR(x)} t_4$ issue shown in Figure ~(3c) by introducing another property $\WR$-Value.
That is, as Figure ~ 4d shows, $t_3 \rel{\WR(x)} t_4$ and $t_1 \rel{\WR(x)} o_3$ cannot exist together, 
for $o_3$ and $t_4$ actually read the same list on key $x$, it's impossible to match different appends as the last element of the same list. 

With the observer-complementary history, $\LOtoWW$ and $\WRValue$ reasoning rule, we're capable to handle the general list append workload.
This model, however, poses a new ``\singlewrite'' assumption on histories, which requires each transaction contains no more than 1 append operation on each key.
Otherwise it would leads to a complex string-matching problem, which is far from our main concentration.

\subsection{Various Optimizations for Solving Efficiency}

At this point, we have a constraints-based modelling of the general history checking problem, the next step is to solve.
% TODO: citation
In previous works, the solving process can be staged into 3 steps in constructing, pruning and SMT solving.
To alleviate the excessive overhead brought by ``non-\uniqueval'' uncertainty, we designed optimizations on each stage.

\begin{itemize}
  \item \textbf{pruning}. We use an efficient reachability algorithm without the help of GPU and a data-friendly way to iterative on derived $\RW$ edges.
  \item \textbf{SMT solving}. We designed a dedicated SMT solver with various domain-specific optimizations.
  In our SMT solver, we exploit some properties of $\WW$ and $\WR$ edges to compress the encoding size.
  We made an observation on detected cycles and applied a specialized optimization on detecting short cycles.
  We used a kind of theory propagation to lessen the times of calling the expansive cycle detection algorithm.
\end{itemize}

These optimizations made our checker perform extraordinarily on both ``\uniqueval'' and general workloads.


==> sections/port.tex <==
\section{Portability}
\subsection{Snapshot Isolation}
\label{sec:port-si}

\subsection{Compatibility with Jepsen}
\label{sec:port-jepsen}

==> sections/related.tex <==
\section{Related Work} \label{section:related}

% using highly concurrent workloads:

% black-box checkers:
% \cite{PolySI:VLDB2023}
% \cite{Cobra:OSDI2020}
% \cite{Viper:EuroSys2023}
% \cite{Complexity:OOPSLA2019}
% \cite{Elle:VLDB2020}

% white-box checkers:
% \cite{Emme:EuroSys2024}
% \cite{ConsMaude:TACAS2019}


% using complex queries:

% concurrent programming community:
% Zord~\cite{Zord:PLDI2021}, Deagle~\cite{Deagle:OOPSLA2022},
% Knossos and others (see Elle related work?)

\red{========== hfwei: I just copy them from the mini work. =========}

It is known that the SI checking problem is \npc{}
for general key-value histories where
the transaction execution order is unknown,
even under the \uniqueval{} assumption~\cite{Complexity:OOPSLA2019}.
Existing SI checkers fall into two categories:
those desinged for general histories
and those tailored for histories with additional information.

\paragraph*{Checkers for General Histories}

The SI checking algorithms proposed
in~\cite{Complexity:OOPSLA2019} are polynomial time
assuming that certain input history parameters,
e.g., the number of sessions, are fixed.
However, they lack practical efficiency
as these fixed parameters can be large~\cite{PolySI:VLDB2023}.
PolySI~\cite{PolySI:VLDB2023},
influenced by both Cobra~\cite{Cobra:OSDI2020} for serializability checking
and the characterization of SI using dependency graphs~\cite{AnalysingSI:JACM2018},
encoded the SI checking problem into an SMT problem,
seeking cycles in a generalized polygraph~\cite{SER:JACM1979,Cobra:OSDI2020},
and then resolves it using the MonoSAT solver~\cite{MonoSAT:AAAI2015}.
Viper~\cite{Viper:EuroSys2023} introduces BC-polygraphs
as a new representation of transactional dependencies,
reduces the SI checking problem into
a cycle detection problem on BC-polygraphs,
and leverages MonoSAT to solve it.
Essentially, these checkers need to explore all
potential transaction execution orders,
and their computational cost grows exponentially
with the number $N$ of transactions in the history
in the worst case.

\paragraph*{Checkers for Histories with Additional Information}

Elle~\cite{Elle:VLDB2020} can infer the transaction execution order
in a history (more precisely, the version order of a history
in Adya's formalism~\cite{Adya:PhDThesis1999})
by carefully choosing data types
and utilizing the \uniqueval{} assumption
to generate recoverable and traceable histories.
% For perfectly recoverable and traceable histories,
Elle scales well to histories
with tens of thousands of transactions,
but struggles with those containing hundreds of thousands of transactions
due to expesenive cycle detection performed
on extensive dependency graphs of such large histories.
Elle works well for data types such as lists,
but for some data types such as read-write registers
(i.e., key-value pairs), counters, and sets,
it can make only limited inferences.
In contrast, our checking algorithms leverage timestamps
to infer the transaction execution order.
They are neither limited to specific data types
nor to the \uniqueval{} assumption.

% It has been noted in~\cite{Elle:VLDB2020} that
When the start and commit timestamps of transactions are available
in some snapshot-isolated database systems,
Elle~\cite{Elle:VLDB2020} can utilize them to infer the time-precedes order
among transactions in Adya's formalism of SI
and construct a start-ordered serialization graph~\cite{Adya:PhDThesis1999}.
In our timestamp-based approach,
we infer the transaction execution order
according to their commit timestamps
and check the SI axioms on the fly
while simulating the execution of transactions one by one,
without constructing extensive dependency graphs
and performing expensive cycle detection on them.
% Moreover, our \onlinetool{} algorithm supports online SI checking,
% a feature not supported by existing SI checkers.
% we have designed online SI checking algorithm,
% while none of the existing SI checkers support online checking.
% We demonstrate the feasibility of timestamp-based approach
% in our work by showing that
% \begin{inparaenum}[(1)]
% 	\item most SI implementations in practice are timestamp-based;
% 	\item transaction timestamps can be easily obtained with minimal effort; and
% 	\item the timestamp-based checking algorithm can be highly efficient.
% \end{inparaenum}

Clark et al.~\cite{SER-VO:ETH2021} introduced the concept of
version order recovery,
similar to the notion of traceability in Elle.
They demonstrated that the version order of a history
can be easily recovered from PostgreSQL and TiDB,
utilizing their CDC mechanism.
Additionally, they designed an efficient serializability checker % called Emme
based on version order recovery.
In contrast, our checking algorithms focus on SI,
for which inferring the snapshot of each transaction is also essential.
% Notably, Emme does not support online checking.

Cobra~\cite{Cobra:OSDI2020} is the only checker
that supports online checking for serializability,
claiming a throughput of 2k TPS with GPU acceleration
on workloads featuring 8 operations per transaction.
However, Cobra needs to inject ``fence transactions''
into client workloads, which is often unacceptable in production.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\inlsec{Characterizing and Checking Database Isolation Levels}
There has been extensive research on formalizing database isolation levels~
\cite{Adya:PhDThesis1999,AnalysingSI:JACM2018,Complexity:OOPSLA2019,Formal:IEEE1979,Framework:CONCUR2015,Seeing:PODC2017}
and developing isolation checkers based on these formalisms~
\cite{Cobra:OSDI2020,PolySI:VLDB2023,Viper:EuroSys2023,Plume:OOPSLA2024,Elle:VLDB2020,Emme:EuroSys2024,ConsMaude:TACAS2019}.
We focus on state-of-the-art black-box checkers and their underlying formalisms.

The dependency graph model,
introduced by~\cite{Adya:PhDThesis1999},
uses three types of directed edges to represent dependencies between transactions,
corresponding to $\WW$, $\WR$ and $\RW$ edges in our characterization.
However, checking serializability in a database history is \npc
due to uncertain $\WW$ and $\RW$ relationships.

Elle~\cite{Elle:VLDB2020} adopts Adya's formalism and
addresses this uncertainty through the \uniqueval{} assumption for determining $\WR$ relations
and the \listappend{} mode for determining $\WW$ relations,
making the checking problem polynomial.
Cobra~\cite{Cobra:OSDI2020} maintains the \uniqueval{} assumption
but reverts to the \rwregisters{} mode.
To reason $\WW$ uncertainty efficiently,
Cobra employs the MonoSAT SMT solver~\cite{MonoSAT:AAAI2015}
and implements several optimizations for serializability checking,
such as pruning.
PolySI~\cite{PolySI:VLDB2023} extends checking to \si
by building on Cerone and Gotsman~\cite{AnalysingSI:JACM2018}'s characterization
and introduces generalized polygraphs.
Concurrently, Viper~\cite{Viper:EuroSys2023} proposes BC-polygraph and
additional techniques for \si checking.
For weaker isolation levels,
Biswas and Enea~\cite{Complexity:OOPSLA2019} introduces a new characterization of emerging isolation levels
(such as \ra and \tcc) and
develops prototype checking algorithms.
Building on this work,
Plume~\cite{Plume:OOPSLA2024} introduces transactional anomalous patterns (TAPs)
and leverages vector and tree clocks~\cite{TreeClock:ASPLOS2022} for efficient checking.

These checkers employ different characterizations of isolation levels and
implement various optimizations for specific isolation levels.
They all rely on the \uniqueval{} assumption for $\WR$ relation inference,
and SMT-based checkers~\cite{Cobra:OSDI2020,PolySI:VLDB2023,Viper:EuroSys2023}
utilize MonoSAT for efficient solving.
Our work demonstrates the importance of lifting the \uniqueval{} assumption and
proposes universal polygraphs as an intermediate representation
that can encode a history into most known isolation levels.
Moreover, by mining the inner structural patterns in database histories,
we design specialized solving techniques that achieve superior performance
compared to existing approaches.

\inlsec{SMT-based Concurrent Program Verification}
Program verification through SMT formula encoding has a well-established history
in analyzing program properties.
Recent advances in SMT solver optimization~
\cite{Zord:PLDI2021,Interference:PPoPP2022,Satisfiability:TOPLAS2023,Deagle:OOPSLA2022,CAAT:OOPSLA2022,MMEncoding:OOPSLA2023}
have significantly improved solving efficiency.
Given the semantic equivalence between Sequential Consistency~\cite{SC} and Serializability,
these optimization techniques show potential for application
in database isolation verification.
Zord~\cite{Zord:PLDI2021} introduced the ordering consistency theory for efficient reasoning of ordering constraints.
A key contribution is the elimination of from-read (known as $\RW$ in database literature) variables and constraints
by incorporating them as an axiom within the theory solver.
Besides, Zord proposes strategies in conflict clause generation
and cycle detection algorithms to improve the solving efficiency.
Additionally, Zord enhanced solving efficiency through improved conflict clause generation
and cycle detection algorithms.
While \ourtool adopts the from-read technique,
it maintains other aspects consistent with MonoSAT's approach.
Deagle~\cite{Deagle:OOPSLA2022}, recognized as the winnder in SV-Comp~\cite{SVCOMP22:TACAS2022,SVCOMP23:TACAS2023},
implemented a more aggressive optimization by furthur eliminating write-serialization (known as $\WW$) variables and constraints,
introducing a consistency-preserving propagation strategy for determining $\WW$ relations.
However, this approach has been shown to be incomplete in the SC memory model,
potentially leading to false positives.
Zpre~\cite{Interference:PPoPP2022} employed integer clock encoding to
determine happening order relationships,
primarily contributing through a variable assignment branching heuristic.
In contrast, our branching selection heuristic focuses specifically on polarity,
utilizing information from the PK algorithm.
CAAT~\cite{CAAT:OOPSLA2022} and its follow-up work~\cite{MMEncoding:OOPSLA2023}
focused primarily on compact encoding across various memory models,
rather than solving process optimizations.
Although prior work has proposed various optimizations
for SMT-based concurrent program verification,
there exists a fundamental distinction between concurrent program verification
and database history verification in terms of graph node scale.
In concurrent program verification,
the graph for cycle detection typically contains a relatively small number of nodes representing shared read/write operations (usually less than $10^3$ nodes),
whereas in database history verification,
the graph contains nodes representing transactions,
which can be substantially larger (reaching $10^5$ nodes).
This significant difference in graph scale indicates that
transaction history verification poses greater computational challenges,
requiring more powerful optimization strategies.

==> sections/ser-checking.tex <==
% ser-checking.tex

\subsection{Black-box \ser Checking}
\label{ss:ser-checking}

\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{figs/arch.pdf}
	\caption{The architecture of black-box checking isolation levels. The workflow of SMT-based history verification  (\circled{4}) is commonly adopted by Cobra, Viper, and PolySI.
		For non-SMT isolation checkers like Elle, constructing a dependency graph  (\circled{5}) is  followed directly by solving with graph traversals (\circled{8}).}
	\label{fig:black-box-arch}
\end{figure}

\hfwei{Suggestion: Inline content and figure to Section~\ref{section:intro}}

Black-box checking of database  isolation guarantees typically involves four steps, as shown in Figure~\ref{fig:black-box-arch}.
Clients first stress the database under test using randomized transaction workloads 
in \circled{1},  treating it as a black box.
 Each client  records the transactional requests issued to the database along with the associated execution results received  in  \circled{2}. 
 For example, if a client performs a read-write transaction, it records the data items (or keys) of both operations, the respective values fetched and written, and whether the transaction is committed or aborted.
 Subsequently,
 the records across all clients are merged into a single history that is  fed  to an isolation checker in \circled{3}. Finally, the checker verifies whether this history meets the specified isolation guarantee in \circled{4}; 
\blue{a counterexample is often returned upon finding an isolation bug}.
Existing checkers typically checks two main types of histories.

\blue{[examples only?]}

\inlsec{Verifying Histories of Read-write Registers}
\nobi{briefly explain what read-write registers are.}
Read-write registers store the most recent written value.
For common workloads involving \emph{read-write registers}, a recent advance utilizes SMT solving to expedite history verification.
SMT solvers specialize in resolving uncertain dependencies, such as the version order of concurrent writes ($\WW$).
Representative checkers of such a kind include  Cobra~\cite{Cobra:OSDI2020} for \ser, as well as Viper~\cite{Viper:EuroSys2023} and PolySI~\cite{PolySI:VLDB2023} for \si. 
As shown in Figure~\ref{fig:black-box-arch} \circled{4},  all these checkers start by constructing a transactional dependency graph in  \circled{5}, in terms of  constraints.
\nobi{inline example 2.1?}
They then proceed to
prune constraints through domain-specific optimizations in  \circled{6}, aiming to accelerate the subsequent SMT solving.
The remaining constraints are encoded in \circled{7}, and the history verification
culminates in \circled{8} by invoking  the off-the-shelf SMT solver MonoSAT~\cite{MonoSAT:AAAI2015}, which is tailored for checking graph properties like acyclicity
(isolation bugs are often represented as cycles within dependency graphs~\cite{Adya:PhDThesis1999,AnalysingSI:JACM2018}).

\begin{example}
Figure~\ref{fig:prelim-rw} (move sec 3.1 here; shortened \hfwei{why?})
\end{example}

\hfwei{Two examples: one for the Cobra approach (\ser{} history with \uniqueval);
one for non-\ser{} history without \uniqueval{} (just bruteforce)}

\hfwei{Move to Section~\ref{section:list}??? Not sure about this.}

\inlsec{Verifying List-append Histories}
Elle~\cite{Elle:VLDB2020}, as part of the Jepsen testing framework~\cite{Jepsen}, leverages  \emph{list-append} workloads to effectively infer version orders. 
\nobi{Briefly explain what list-append is.}
Lists store all appended values in their version order.
Consequently, reading a list of values, e.g., $[1,2,3]$ from key $k$,  indicates  a strict version order of the corresponding append operations, i.e., $\mathit{append}(k,1)$, $\mathit{append}(k,2)$, $\mathit{append}(k,3)$, as well as their associated transactions.
Hence, Elle does not depend on an SMT solver for solving uncertain dependencies,  and instead uses graph traversal algorithms to identify cycles  in  \circled{8}, following the construction of an Adya's dependency graph in  \circled{5}.
Elle has been successfully applied to a range of databases, demonstrating the broad applicability 
of  the list datatype and its append operations.

\begin{example}
	Figure~\ref{fig:prelim-list} (emphasizing how to infer version orders should be enough; with a comparison to Figure 2, e.g., no blue WW) 
\end{example}

==> sections/ser-smt-hypo.backup.tex <==
% ser-smt-hypo.tex

\section{Key Solving Characteristics for Efficient SMT-based Checking \nobi{another title}}
\label{section:characteristics-of-histories}

% \zhiheng{
%   To conclude our 2 hypothesis(observations): 
%   \begin{enumerate}
%     \item 2-width cycles dominates in conflict clauses;
%     \item PK's pseudo-topological order simulates a version order.
%   \end{enumerate}
% }

In this section, 
we present two key observations on characteristics of solving histories 
based on micro-experiments, 
which provide insights to our design of dedicated solver for efficient \ser checking.
\nobi{A new transit: introduce our hypothesis; motivated by general purpose smt solving vs tailored wrt database txn workload characteristics; validated empirically }

\subsection{Prevalence of 2-width Conflict Cycles}
\label{ss:observation-small-cycles}

% \blue{
%   \begin{enumerate}
%     \item conflict clause are important, for it can help prevent unnecessary conflict;
%     \item pruning, 1-width cycles are pruned, efficiency is effectively improved;
%     \item micro experiments (minimal);
%     \item observation: 2-cycles dominates.
%   \end{enumerate}
% }

One of the key differences between CDCL(T) and brute-force enumeration lies in the ``learning'' of conflict clauses.
\brown{\sout{which help prevent the SAT solver from revisiting the same conflicts.}} 
For example, 
consider the conflict clause $\lnot \crwvar_{3, 2}^x \lor \lnot \csovar_{2, 3}$
for \statebox[sred]{2} of Figure~\ref{fig:running-example-solving}.
Since the variable $\csovar_{2, 3}$ is always $\true$,
$\crwvar_{3, 2}^x$ \blue{would be} assigned to $\false$ by unit propagation,
thus preventing the $T_2 \rel{\SO} T_3 \rel{\RW(x)} T_2$ cycle.
Since $T_3 \rel{\RW(x)} T_2$ is derived from $T_1 \rel{\WW(x)} T_2$ and $T_2 \rel{\WR(x)} T_3$ 
\blue{due to} the clause $\lnot \cwwvar_{1,2s}^x \lor \lnot \cwrvar{x}_{1,3} \lor \crwvar_{3,2}^x$, 
these two edges cannot simultaneously exist in $\ug$.
% If $\cwwvar_{1, 2}^x$ \blue{were} assigned to $\true$ before $\cwrvar{x}_{1, 3}$,
% the assignment $\lnot \cwrvar{x}_{1, 3}$ \blue{would be} propagated due to the clause 
% $\lnot \cwwvar_{1,2}^x \lor \lnot \cwrvar{x}_{1,3} \lor \crwvar_{3,2}^x$, 

% A straightforward idea is:  
% if we equip the solver with \emph{all} conflict clauses, 
% then all conflicts can be avoided, 
% the solver would directly reach a solution or conclude unsatisfiability.
% However, this is impossible.
% In the isolation checking problem, 
% conflict clauses describe possible cycles (simple or non-simple) in the dependency graph, 
% the number of which is known to be infinite. 
% Nevertheless, since the solver terminates after encountering finite cyclic states, 
% we conjecture that some conflict clauses are more effective in improving solving efficiency, 
% while others are less effective. 
% We aim to identify these influential clauses.

% \blue{[We further conjecture that their features lie in 
% the conflict clauses generated during the solving process.]}


Pruning, an effective technique to improve the checking efficiency~\cite{Cobra:OSDI2020,PolySI:VLDB2023,Viper:EuroSys2023}, 
can be understood in terms of conflict clauses.
Pruning aims to eliminate impossible choices of $\WW$ constraints 
given the known graph.
\brown{\sout{thereby reducing the searching space.}}
For example, for a $\WW$ constraint $\set{T_1 \rel{\WW(x)} T_2, T_2 \rel{\WW(x)} T_1}$, 
if $T_1$ is reachable from $T_2$ in the known graph (denoted as $T_2 \leadsto T_1$), 
then \brown{choosing $T_1 \rel{\WW(x)} T_2$ would create a cycle $T_1 \rel{\WW(x)} T_2 \leadsto T_1$}.
Thus, the choice $T_1 \rel{\WW(x)} T_2$ can be ``pruned'', 
and the $\WW$ constraint can be resolved 
by choosing the remaining choice $T_2 \rel{\WW(x)} T_1$.
This process, in terms of conflict clauses, 
amounts to incorporating the conflict clause $\lnot \cwwvar_{1, 2}^x$ 
into the SAT encoding $\Phi_{\G}$:
if $\lnot \cwwvar_{1, 2}^x$ \blue{were} first assigned, 
$\cwwvar_{2, 1}^x$ would be propagated due to the clause
$\cwwvar_{1, 2}^x \lor \cwwvar_{2, 1}^x$. 

The conflict clauses for pruning 
consists of a single ($\WW$) variable.
Their effectiveness motivates us to investigate 
the characteristics of conflict clauses generated by the theory solver, 
particularly in terms of the number of associated boolean variables.

To this end,
we adopt the nontion of \emph{cycle width}~\cite{Zord:PLDI2021, Satisfiability:TOPLAS2023}.
The width of a cycle is defined as the number of \emph{unique} $\WW$ and $\WR$ variables 
appearing in its conflict clause.
\brown{[Because ?]
Note that} $\SO$ variables are always $\true$, 
and $\RW$ variables can be derived from $\WW$ and $\WR$ variables.
We also omit duplicate appearance of the same variable.
For example, in the case of $T_1 \rel{\WR(x)} T_2 \rel{\RW(x)} T_3$, 
the variable $\cwrvar{x}_{1, 2}$ appears twice -- 
once directly and once as part of $\crwvar_{2, 3}^x$ -- 
but is counted only once. 
The width of cycles generated by pruning is $1$;
and the clause $\lnot \crwvar_{3, 2}^x \lor \lnot \csovar_{2, 3}$
is equivalent to $\lnot \cwwvar_{1, 2}^x \lor \lnot \cwrvar{x}_{1, 3}$ 
(recall that $\csovar_{2, 3}$ is $\true$), 
which has a width of $2$.

%\inlsec{Micro-experiment 1}
\inlsec{Empirical Validation}
We measure the width of cycles encountered during the solving procedure.
However, a single conflict may correspond to multiple cycles, 
depending on the specific path found by the cycle detection algorithm.
For example, in Figure~\ref{fig:minimal-width-eg}, 
after adding $T_1 \rel{\WW(x)} T_2$, 
the theory solver encounters a conflict with two cycles: 
$T_1 \rel{\WW(x)} T_2 \rel{\SO} T_3 \rel{\WR(y)} T_1$ (denoted as $\C_1$) and 
$T_1 \rel{\WW(x)} T_2 \rel{\WW(z)} T_4 \rel{\WR(w)} T_1$ (denoted as $\C_2$), 
where $\C_1$ has a width of $2$ and $\C_2$ of $3$.
To explore the effectiveness of ``small'' cycles \blue{in avoiding futile exploration of invalid branches}, 
we record the minimal width, i.e., 2 for this example, of encountered cycles.
% while do not modify the default conflict clause,  
% to keep the solving process identical to the baseline.

% In this conflict, 
% both conflict clauses of $\C_1$ and $\C_2$ are capable to 
% express this conflict and prevent the assignment of $\cwwvar_{1, 2}^x$.
% However, the theory solver may select $\C_1$ or $\C_2$ and 
% generate the conflict clause of it, 
% depending on its implementation 
% (e.g. the iteration order of outer edges of vertices).


% we consider the minimal cycle width among all cycles corresponding to this conflict.
% \blue{[why minimal? the minimal conflict clause is capable to prevent this conflict. needed here?]}
% Importantly, we do not modify the actual conflict clause 
% generated and returned by MonoSAT 
% in order to keep the solving procedure identical to the baseline,
% though it may not be minimal.

\begin{figure}
	\centering
	\begin{minipage}[b]{.35\columnwidth}
		\centering
	\includegraphics[width=\columnwidth]{plot/minimal-width.pdf}
		\captionsetup{skip=4pt}
		\caption{Selecting the minimal width cycle for a conflict.}
		\label{fig:minimal-width-eg}
	\end{minipage}
	\hspace{1.5ex}
	\begin{minipage}[b]{.55\columnwidth}
\pgfplotsset{height=140pt, width=240pt}
\pgfplotsset{tick style={draw=none}}
	\centering
	\resizebox{\textwidth}{!}{
		\begin{scaletikzpicturetowidth}{0.5\textwidth}
			\begin{tikzpicture}[scale=\tikzscale]
				\begin{axis}[
					% title={C-Twitter 10K},
					xlabel={\LARGE cycle width},
					ylabel={\LARGE proportion (\%)},
					xlabel near ticks,
					ylabel near ticks,
					ymax=100,
					ytick={10,20,30,40,50,75,100},
					xtick={1,2,3,4,5,6,7,8,9,10,15,20},
					legend pos=north east,
					legend style={draw=none}
					]
					\addplot[color=teal,mark=o,mark size=2pt] table [x=param, y=gtpcc, col sep=comma] {figs/cycle-width/data/minimized-data.csv};
					\addplot[color=blue,mark=square,mark size=2pt] table [x=param, y=gtwitter, col sep=comma] {figs/cycle-width/data/minimized-data.csv};
					\addplot[color=green!50!black,mark=triangle,mark size=2pt] table [x=param, y=grubis, col sep=comma] {figs/cycle-width/data/minimized-data.csv};
					\addplot[color=red!65!black,mark=diamond,mark size=2pt] table [x=param, y=grh, col sep=comma] {figs/cycle-width/data/minimized-data.csv};
					\addplot[color=brown,mark=pentagon,mark size=2pt] table [x=param, y=grw, col sep=comma] {figs/cycle-width/data/minimized-data.csv};
					\addplot[color=orange,mark=asterisk,mark size=2pt] table [x=param, y=gwh, col sep=comma] {figs/cycle-width/data/minimized-data.csv};
					
					% \addplot[color=teal,mark=o,mark size=1pt] table [x=param, y=gtpcc, col sep=comma] {figs/cycle-width/data/data.csv};
					% \addplot[color=blue,mark=o,mark size=1pt] table [x=param, y=gtwitter, col sep=comma] {figs/cycle-width/data/data.csv};
					% \addplot[color=green!50!black,mark=o,mark size=1pt] table [x=param, y=grubis, col sep=comma] {figs/cycle-width/data/data.csv};
					% \addplot[color=red!65!black,mark=o,mark size=1pt] table [x=param, y=grh, col sep=comma] {figs/cycle-width/data/data.csv};
					% \addplot[color=brown,mark=o,mark size=1pt] table [x=param, y=grw, col sep=comma] {figs/cycle-width/data/data.csv};
					% \addplot[color=orange,mark=o,mark size=1pt] table [x=param, y=gwh, col sep=comma] {figs/cycle-width/data/data.csv};
					\legend{G-TPCC,  G-Twitter,  G-RUBiS,  read-heavy (95\% reads),  balanced (50\% reads),  write-heavy (30\% reads)}
				\end{axis}
			\end{tikzpicture}
		\end{scaletikzpicturetowidth}
	}
	\captionsetup{skip=0pt}
	\caption{Distribution of minimal cycle widths across conflicts.}
	\label{fig:cycle-width-minimal}
	\end{minipage}
\end{figure}


%\begin{figure}[t]
%  \centering
%	\includegraphics[width=0.4\columnwidth]{plot/minimal-width.pdf}
%     \captionsetup{skip=0pt}
%	\caption{Selecting the minimal width cycle for a conflict.}
%	\label{fig:minimal-width-eg}
%\end{figure}

%\input{figs/cycle-width/cycle-width-minimal}

We conduct this micro-experiment 
on six representative benchmarks 
(see Section~\ref{ss:setup} for detail description of these benchmarks) 
of 1,000 transactions.
Figure~\ref{fig:cycle-width-minimal} shows the discrete distribution of minimal cycle widths.
Notably, 2-width cycles dominate across all benchmarks,
suggesting that a significant portion of conflicts can be captured 
by clauses consisting of only two $\WW$ or $\WR$ variables.
To avoid 2-width cycles in solving, 
we will encode them into the SAT formula $\Phi_{\G}$,
as described in Section~\ref{ss:small-width-cycles}.
% This observation highlights the potential of small-width cycles, 
% particularly those with width 2,
% as key contributors to solver behavior and performance.
% We are motivated to design specific strategies
% that selectively equip conflict clauses of 2-width cycles.
% Compared to the number of graph vertices ($1000$), 
% the widths are relatively small.

\subsection{PK's Pseudo-topological Order as Almost a Version Order} \label{ss:observation-polarity}

% \blue{
%   \begin{enumerate}
%     \item search directions are important, polarity is important;
%     \item polarity is also important in cycle detection algorithm(PK);
%     \item PK algorithm maintains a pseudo-topological order, that is natural a version order;
%     \item micro expriment on PK statistics;
%     \item observation: PK's pseudo-topological order simulates a version order.
%   \end{enumerate}
% }

CDCL(T) is essentailly a depth-first search procedure.
One key factor affecting its efficiency is the search direction.
The polarity assigned to each variable 
(i.e., $\true$ or $\false$) 
guided the SAT solver.
An incorrect polarity assignment may lead the search into a dead end, 
causing futile exploration of invalid branches before backtracking.
Moreover, incorrect polarity causes more graph traversals 
in the PK algorithm~\cite{PKTopo:ACMJEA2006}  
employed by MonoSAT for cycle detection.

The PK algorithm maintains 
a dynamic \emph{pseudo-topological order} of all vertices,
denoted as $\clevel{\cdot}$.
When adding an edge $(\fromvar, \tovar)$, 
PK first checks if $\clevel{\fromvar} < \clevel{\tovar}$.
If so, PK returns immediately, 
because adding this edge does not create any cycle.
Otherwise, it traverses the graph to 
check whether the vertex $\tovar$ is unreachable from the vertex $\fromvar$, 
and if so, 
it updates the $\clevel{\cdot}$ values of the visited vertices.
% to ensure $\clevel{\fromvar}' < \clevel{to}'$,
% thus preventing unnecessary graph traversals in the future.
% \zhiheng{inline polarity here?}

% Although originally intended to optimize graph traversal, 
% the pseudo-topological order effectively represents a possible version order of the discovered dependency graph.
% When the solver reaches the a valid model, 
% this maintained order provides a candidate version order, 
% though it may differ from the actual version order in the database.

% To make informed polarity selections, 
% we draw inspiration from 
% how Elle~\cite{Elle:VLDB2020} infers the $\WW$ dependency 
% based on the version order.
% Assuming the version order of the history is known, 
% we can rule out dependency edges that violate it.
% For a dependency edge $T \rel{} S$, 
% if $S$ precedes $T$ in the version order,
% we can conclude that this edge should not appear in the dependency graph-- 
% i.e., the corresponding variable should be assigned $\false$.

\inlsec{Empirical Validation}
%\inlsec{Micro-experiment 2}
To measure how effective it is for the pseudo-topological order 
to prevent graph traversals and cycles, 
we conduct a micro-experiment on six benchmarks 
and collect the following three metrics:
(1) the number of calls to the PK algorithm,
(2) the number of graph traversals (i.e., when the checking $\clevel{\fromvar} < \clevel{\tovar}$ fails), and
(3) the number of cycles encountered.

\input{tables/cycle-statistics-no-cycle-opt}

As shown in column 2 - 4 of Table~\ref{table:cycle-statistics}, 
a $99.7\%$ (1 $-$ \#Cycles Detected / \#Calls to PK) of the PK algorithm calls end up with no cycles.
In contrast,
when PK performs graph traversals, 
it is highly likely (\#Cycles Detected / \#Traverse; $74.4\%$ on average) to detect a cycle.
The difference between \#Traverse and \#Cycles Detected, 
denoted as \#Reorder in column 5 of Table~\ref{table:cycle-statistics},
counts the number of reorderings of the pseudo-topological order 
and the low ratio (column 7) between \#Reorder and the number of constraints 
(i.e., $|\wwcons \cup \wrcons|$ in column 6)
indicates that the very initial pseudo-topological order of the graph 
is almost a version order we are seeking for.
We will show how to pick the polarity of variables deliberately 
to further exploit the pseudo-topological order in Section~\ref{ss:polarity}.

% A further inference is that the pseudo-topological order remains stable 
% from the start of the search to the end.
% We calculate the number of reorderings (i.e., \#Traverse - \#Detect a Cycle), 
% and present it in the fourth column in Table~\ref{table:cycle-statistics}.
% Since resolving a constraint may introduce a reorder,  
% we use the ratio of \#Reorder to the total number of constraints (the sum of $\WW$ and $\WR$ constraints) 
% to measure changes in the pseudo-topological order (also shown in Table~\ref{table:cycle-statistics}).
% This ratio is very low across these benchmarks, averaging $6.53\%$.
% When the solver reaches a solution, 
% the pseudo-topological order is natural a version order of transactions.
% We therefore conjecture that PK's topological order is almost a version order.

% Another finding is the effectiveness of the pseudo-topological order in avoiding conflicts:
% an attempt to add an edge $(\fromvar, \tovar)$ 
% that satisfies $\clevel{\fromvar} < \clevel{\tovar}$ is likely to 
% correspond to a valid edge in the final dependency graph,
% whereas attempts that violate this condition often lead to conflicts.
% In general, fewer conflicts may imply shorter solving time.
% This insight suggests that the pseudo-topological order 
% can be exploited to design a polarity selection strategy 
% tailored to isolation checking.

==> sections/ser-smt-methods.tex <==
% ser-smt-methods.tex

\section{Dedicated SMT Solver-based Serializability Checking}
\label{section:ser-smt-theory-methods}



==> sections/ser-smt-theory.tex <==
% ser-smt-theory.tex

\input{sections/opt-motivation}

\input{sections/ser-smt-overview}
%%%%%%%%%%%%%%%%%%%%
\input{sections/opt-cycles}
\input{sections/opt-polarity}
\input{sections/opt-others}
%%%%%%%%%%%%%%%%%%%%


==> sections/ser-smt.tex <==
% ser-smt.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Off-the-Shelf SMT Solver-based Serializability Checking}
\label{section:baseline}

\input{figs/algs/ser-mono-framework}

Following the same spirit of~\cite{Cobra:OSDI2020,PolySI:VLDB2023,Viper:EuroSys2023},
we first present the baseline of serializability checking
based on MonoSAT~\cite{MonoSAT:AAAI2015},
a dedicated SMT solver for monotonic theories including graph acyclicity.
To check a history $\H$, it consists of three stages
(Figure~\ref{fig:ser-smt-theory-framework}):
first \emph{constructing} the universal polygraph of $\H$,
then \emph{encoding} the polygraph into an SAT formula,
and finally \emph{solving} the formula using MonoSAT.
In the following, we use the general history $\H_{2}$ in Figure~\ref{fig:rw-checking}
as a running example.

%%%%%%%%%%%%%%%%%%%%
\subsection{Constructing}
\label{ss:constructing}

The universal polygraph $G_{2}$ of $\H_{2}$ is given
in Figure~\ref{fig:rw-checking-h2-constraints}
and has been explained in Example~\ref{ex:universal-polygraph}.
%%%%%%%%%%%%%%%%%%%%
\subsection{Encoding}
\label{ss:encoding}

We use a boolean variable to indicate the existence of an edge
in the universal polygraph $G_{2} = (V_{2}, E_{2}, C_{2})$.
The variables for the edges in the known graph $E_{2}$ are set to $\top$.
The key is to encode the $\WW$ and $\WR$ constraints,
as well as the derived $\RW$ constraints, into SAT clauses.
%%%%%%%%%%%%%%%
\subsubsection{The Known Graph}

The encoding of the known graph
of the universal polygraph $G_{2}$ is given by $\Phi_{KG}$,
\[
  \Phi_{KG} = \csovar_{2, 3}.
\]

%%%%%%%%%%%%%%%
\subsubsection{The $\wwcons$ Constraints}

The encoding of the $\wwcons$ constraints
of the universal polygraph $G_{2}$ is given by $\Phi_{\wwcons}$,
\[
  \Phi_{\wwcons} = \cwwvar_{1,2} \lor \cwwvar_{2,1}
\]
where $\cwwvar_{1,2}$ and $\cwwvar_{2,1}$ denote the existence of
the directed $\WW$ edge from $T_1$ to $T_2$
and from $T_2$ to $T_1$, respectively.

Two points need to be clarified.
First, the clause $(\lnot \cwwvar_{1,2} \lor \lnot \cwwvar_{2,1})$
is unnecessary because a violation of this clause
immediately implies a cycle between $T_{1}$ and $T_{2}$.
Second, it is also unnecessary for the variables $\cwwvar_{1,2}$ and $\cwwvar_{2,1}$
to be \red{indexed by} the key, i.e., $x$, associated with the edges.
This works for two reasons:
On the one hand, according to Theorem~\ref{thm:ser-upg},
we only need to know whether a particular type of edge exists
between two transactions.
On the other hand, the existence of a $\WW$ edge
between two transactions
implies that of each $\WW$ edge associated with the key
that gives rise to the \red{conflict}
between these two transactions.
%%%%%%%%%%%%%%%
\subsubsection{The $\wrcons$ Constraints}
\label{sss:wrcons}

The encoding of the $\wrcons$ constraints
of the universal polygraph $G_{2}$ is given by $\Phi_{\wrcons}$,
\[
  \begin{aligned}
    \Phi_{\wrcons} =\; &(\cwrvar{x}_{1,3} \lor \cwrvar{x}_{2,3}) \;\land \\
      &(\lnot \cwrvar{x}_{1,3} \lor \lnot \cwrvar{x}_{2,3})
  \end{aligned}
\]
where $\cwrvar{x}_{1,3}$ denotes the existence of
the directed $\WR$ edge associated with the key $x$
from $T_1$ to $T_3$
(similarly for $\cwrvar{x}_{2,3}$).
The clauses state that
transaction $T_{3}$ reads $x$ from $T_{1}$ or $T_{2}$ but not both.
%%%%%%%%%%%%%%%
\subsubsection{The $\RW$ Constraints}
\label{sss:rwcons}

The encoding of the $\RW$ constraints
\red{of the universal polygraph} $G_{2}$ is given by $\Phi_{\RW}$,
\[
  \begin{aligned}
    \Phi_{\RW} =\;
      & (\lnot \cwwvar_{1,2} \lor \lnot \cwrvar{x}_{1,3} \lor \crwvar_{3,1}) \;\land \\
      & (\lnot \cwwvar_{2,1} \lor \lnot \cwrvar{x}_{2,3} \lor \crwvar_{3,2})
  \end{aligned}
\]
where $\crwvar_{1,3}$ and $\crwvar_{2,3}$ denote the existence of
the directed $\RW$ edge from $T_1$ to $T_3$
and from $T_2$ to $T_3$, respectively,
which are not necessarily indexed by the key $x$.
The first clause states that
$(T_{1} \rel{\WW(x)} T_{2} \land T_{1} \rel{\WR(x)} T_{3})
\implies T_{3} \rel{\RW(x)} T_{1}$,
while the second clause states that
$(T_{2} \rel{\WW(x)} T_{1} \land T_{2} \rel{\WR(x)} T_{3})
\implies T_{3} \rel{\RW(x)} T_{2}$.

The whole encoding for $G_{2}$ is thus
$\Phi_{G_{2}} = \Phi_{KG} \land \Phi_{\wwcons} \land \Phi_{\wrcons} \land \Phi_{\RW}$.
%%%%%%%%%%%%%%%%%%%%
\subsection{Solving}
\label{ss:solving}

MonoSAT supports many common graph predicates
such as reachability, shortest paths, maximum flows, and acyclicity.
To check the \red{acyclicity of $G_{2}$},
we can simply assert that the predicate
$\acyclicencoding(G_{2})$ holds.
If this is the case, then $\H_{2}$ is serializable.
Otherwise, MonoSAT returns an UNSAT core
which indicates an unavoidable cycle \red{in $G_{2}$}.


\hfwei{TODO: unsat example???}

\zhiheng{Move MonoSAT solving framework here, 
including CDCL(T) and cycle detection}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/ser-upg.tex <==
% characterization.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Characterizing Serializability Using Universal Polygraphs} \label{section:characterization}

In this section we introduce universal polygraphs
and use them to characterize \ser{} on general histories.

%%%%%%%%%%%%%%%%%%%%
\subsection{Universal Polygraphs}

Universal polygraphs extends polygraphs~\cite{Cobra:OSDI2020}
by capturing the $\WR$ uncertainties in general histores.

%%%%%%%%%%%%%%%%%%%%
% [Universal Polygraph]
\begin{definition} \label{def:universal-polygraph}
  A \bfit{universal polygraph} $\G = (\V, \E, \C)$
  of a history $\H = (\T, \SO)$
  is a directed labeled graph $(\V, \E)$ called the \emph{known graph},
  together with a pair $\C$ of \emph{constraint sets} such that
  \begin{itemize}
    \item $\V$ corresponds to all transactions in the history $\H$;
    \item $\E \subseteq \V \times \V \times \type \times \Key$
      is a set of edges labelled with the type from
      $\type = \set{\SO, \WR, \WW, \RW}$ and the key from $\Key$.\footnote{
        For an $\SO$ edge, the key component is irrelevant.
      }
    \item The constraint set $\wwcons = \Bset{\btuple{T \rel{\WW(x)} S, S \rel{\WW(x)} T}
      \mid T \in \WriteTx_{x} \land S \in \WriteTx_{x} \land T \neq S}$.
    \item The constraint set $\wrcons = \Bset{\btuple{\bigcup\limits_{T_{i} \vdash \writeevent(x, v)} \set{T_{i} \rel{\WR(x)} S}}
      \mid S \vdash \readevent(x, v)}$.
  \end{itemize}
\end{definition}

$\wwcons$ and $\wrcons$ capture the uncertainties
in the $\WW$ and $\WR$ dependencies, respectively.
For two transactions $T$ and $S$, a type $\typevar \in \type$,
and a key $x \in \Key$,
we also write an edge $(T, S, \typevar, x)$ as $T \rel{\typevar(x)} S$.
\red{Note that} a universal polygraph may contain edges of type $\RW$
such that a ``pruned'' universal polygraph (section XXX)
is still a universal polygraph.
%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%
\input{figs/rw-checking.tex}

\begin{example}%[$\WW$ and $\WR$ constraints]
  \label{ex:universal-polygraph}
  Consider the general history $\H_{2}$ of Figure~\ref{fig:history-h2}.
  It consists of three transactions $T_{1}$, $T_{2}$, and $T_{3}$ with session order $T_2 \rel{\SO} T_3$.
  Both $T_{1}$ and $T_{2}$ write the same value $1$ to the same key $x$.
  The two constraint sets of the universal polygraph $\G_{2}$
  of $\H_{2}$ are:
  \begin{itemize}
    \item $\wwcons = \Bset{\btuple{T_1 \rel{\WW(x)} T_2, T_2 \rel{\WW(x)} T_1}}$
      (shown as dashed lines in blue); and
    \item $\wrcons = \Bset{\btuple{T_1 \rel{\WR(x)} T_3, T_2 \rel{\WR(x)} T_3}}$
      (shown as dotted lines in brown).
  \end{itemize}
\end{example}
%%%%%%%%%%%%%%%%%%%%
\subsection{Universal Polygraph-based Characterization of \ser}
\label{ss:ser-upg}

A universal polygraph of a history
can be regarded as a family of graphs compatible with it,
each of which resolves the constraints
by choosing exactly one $\WW$ or $\WR$ edge
from the $\wwcons$ and $\wrcons$ constraint sets, respectively.

%%%%%%%%%%%%%%%%%%%%
% [Compatible Graphs with a Universal Polygraph]
\begin{definition} \label{def:compatible-graphs-with-a-universal-polygraph}
  A directed labeled graph $\G' = (\V', \E')$ is \bfit{compatible with
  a universal polygraph} $\G = (\V, \E, \C)$ if
  \begin{itemize}
    \item $\V' = \V$;
    \item $\E' \supseteq \E$ such that
      $\forall x \in \Key.\; \forall T, T', S \in \V'.\;
       (T', T, \WR, x) \in \E' \land
        (T', S, \WW, x) \in \E' \implies (T, S, \RW, x) \in \E'$;
    \item $\forall \consvar \in \wwcons.\;
      |\E' \cap \consvar| = 1$; and
    \item $\forall \consvar \in \wrcons.\;
      |\E' \cap \consvar| = 1$.
  \end{itemize}
\end{definition}
%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%
\begin{example}%[Compatible Graphs]
  \label{ex:compatible-graphs}
  Figures~\ref{fig:rw-checking-h2-solution} and
  \ref{fig:rw-checking-h2-conflict} show two graphs
  compatible with the universal graph $\G_{2}$ of $\H_2$.
  In Figure~\ref{fig:rw-checking-h2-solution},
  $T_{3}$ reads $x$ from $T_{1}$ which overwrites $x$ written by $T_{2}$.
  In Figure~\ref{fig:rw-checking-h2-conflict},
  $T_{3}$ reads $x$ from $T_{1}$ which is overwritten on $x$ by $T_{2}$.
  Thus, we also have $T_{3} \rel{\RW(x)} T_{2}$.
\end{example}
%%%%%%%%%%%%%%%%%%%%

By Theorem~\ref{thm:ser-depgraph}, we have
%%%%%%%%%%%%%%%%%%%%
\begin{theorem}[Universal Polygraph-based Characterization of \ser{}]
  \label{thm:ser-upg}
  A history $\H$ satisfies \emph{\ser{}} if and only if
  \emph{$\H \models \intaxiom$} and
  there exists an acyclic graph compatible with
  the universal polygraph of $\H$.
\end{theorem}

% \begin{proof} \label{proof:ser-upg}
%   \hfwei{TODO: add a proof}
% \end{proof}
%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%
\begin{example}%[Applying \ser characterizing theorem on a history]
  \label{ex:ser-characterization}
  The graph compatible with $\G_{2}$
  in Figure~\ref{fig:rw-checking-h2-conflict}
  contains a $T_3 \rel{\RW(x)} T_2 \rel{\SO} T_{3}$ cycle.
  In contrast, the compatible graph in Figure~\ref{fig:rw-checking-h2-solution} is acyclic.
  By Theorem~\ref{thm:ser-upg}, $\H_2$ satisfies \ser.
\end{example}
%%%%%%%%%%%%%%%%%%%%

A brute-force serializability checking algorithm
based on Theorem~\ref{thm:ser-upg}
is to enumerate all possible combinations of $\WR$ and $\WW$ constraints,
and check whether one of them leads to an acyclic compatible graph.
Undoubtedly, this algorithm would be prohibitively expensive for large histories.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/ser.tex <==
% ser.tex

\subsection{The \ser Isolation Level}
\label{ss:ser}

To declaratively justify each transaction of a history,
we need to establish the visibility and arbitration relations among transactions.
The visibility relation specifies
the set of transactions whose effects are visible to each transaction,
while the arbitration relation specifies
the execution order of transactions.

\begin{definition} \label{def:ae}
  An {\it abstract execution} is a tuple
  $\ae = (\T, \so, \vis, \ar)$, where
  $(\T, \so)$ is a history,
  {\it visibility} $\vis \subseteq \T \times \T$
  is a strict partial order, and
  {\it arbitration} $\ar \subseteq \T \times \T$
  is a strict total order such that $\vis \subseteq \ar$.
\end{definition}

For $\h = (\T, \so)$,
we often shorten $(\T, \so, \vis, \ar)$ to $(\h, \vis, \ar)$.
%%%%%%%%%%%%%%%%%%%%
\begin{definition}[\ser~\cite{Framework:CONCUR2015}]
  \label{def:si-axiomatic}
	A history $\h = (T, \SO)$ satisfies \ser{} if and only if
  there exists an abstract execution $\ae = (T, \SO, \vis, \ar)$
  such that the $\sessionaxiom$, $\intaxiom$, $\extaxiom$,
	and $\totalvis$ axioms (explained below) hold.
\end{definition}

Let $r \triangleq \readevent(k, \_)$ be a read operation of transaction $T$.
If $r$ is the first operation on $k$ in $T$,
then it is called an \emph{external} read operation of $T$;
otherwise, it is an \emph{internal} read operation.

The \sessionaxiom{} axiom (i.e., $\SO \subseteq \vis$),
requires previous transactions be visible to
transactions later in the same session.
The \emph{internal consistency axiom} \intaxiom{} ensures that,
within a transaction, an internal read from a key returns the same value
as the last write to or read from this key in the transaction.
The \emph{external consistency axiom} \extaxiom{} ensures that
an external read in a transaction $T$ from a key
returns the final value written by the last transaction in $\ar$
among all the transactions that precede $T$ in terms of $\vis$
and write to this key.
The \emph{total visibility axiom} $\totalvis$ requires that
the visibility relation $\vis$ is total.

\begin{example}
  \label{ex:ser}
  % \hfwei{Two histories: an \ser{} history (with \uniqueval)
  %   and a non-\ser{} history (without \uniqueval)}
  In Figure~\ref{fig:ex-ser}, 
  $\H_1$ is serializable. 
  Figure~\ref{fig:ex-ser-uv} provides a valid construction of $\vis$ and $\ar$: $T_2, T_1, T_3$.
  However, $\H_2$ is unserializable.
  We demonstrate it by attempting to construct valid $\vis$ and $\ar$.
  Consider key $y$: 
  $T_3$ reads the initial value $0$, 
  $T_2$ writes $3$ and $T_1$ reads $3$.
  Therefore we know that $T_3 \rel{\ar} T_2 \rel{\ar} T_1$.
  Since the source of $T_3$'s read value $1$ for key $x$ is unknown (from either $T_1$ or $T_2$), 
  we enumerate possible senarios (as shown by the blue dashed edges in Figure~\ref{fig:ex-nonser-dup}): 
  (1) if $T_3$ reads from $T_2$, then $T_2 \rel{\ar} T_3$, which forms a cycle with $T_3 \rel{\ar} T_2$; 
  (2) if $T_3$ reads from $T_1$, then $T_1 \rel{\ar} T_3$, which forms a cycke with $T_3 \rel{\ar} T_2 \rel{\ar} T_1$.
  Thus, there is no valid $\ar$ for $\H_2$. 
  $\H_2$ is unserializable.
\end{example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/si-upg.tex <==
% si-upg.tex

\subsection{Characterizing \si}

Based on the \bfit{induced SI graph} of PolySI\cite{PolySI:VLDB2023},
we can simply extend our characterization of general \rwregisters{} histories to \si.

%%%%%%%%%%%%%%%%%%%%
\begin{definition} \label{def:si-acyclic}
  Let $G = (V, E, C)$ be a universal polygraph of a history $\H$.
  If there exists at least one compatible graph
  and its induced SI graph is acyclic when edge types and keys are ignored,
  then $G$ is \bfit{\si-acyclic}.
\end{definition}
%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%
\begin{theorem}[Universal Polygraph-based Characterization of \si{}] \label{thm:universal-polygraph-si}
  A history $\H$ satisfies \emph{\si{}} if and only if
  \emph{$\H \models \intaxiom$} and the universal polygraph of $\H$ is \si-acyclic.
  \zhiheng{remove \intaxiom{} here and add it into implementation}
\end{theorem}
%%%%%%%%%%%%%%%%%%%%

The difference between the definition of generalized-polygraph-based and universal-polygraph-based induced SI graphs
can be found in \cite[Appendix XX]{tech-rpt}.

==> sections/tcc-upg.tex <==
% weak-isolation-upg.tex

\subsection{Characterizing Enea RC, RA and TCC \cite{Complexity:OOPSLA2019}}

In this subsection, we move to handle some weak isolation levels \cite{Complexity:OOPSLA2019},
including \rc(RC), \ra(RA) and \tcc(TCC).
They can all be polynomially checked under \uniqueval{} assumption.

%%%%%%%%%%%%%%%%%%%%
\begin{theorem}[The complexity of checking general RC, RA and TCC] \label{thm:weak-npc}
  Checking \rc, \ra and \tcc of \bfit{general} workloads are all \npc problems.
\end{theorem}
%%%%%%%%%%%%%%%%%%%%

The proof sketch can be found in \cite[Appendix XX]{tech-rpt}.

\zhiheng{Below is a copy of universal polygraphs under Enea's definitions, the one in sec3.2 is under Adya(Gotsman),
may be a higher abstraction is needed}

%%%%%%%%%%%%%%%%%%%%
% [Universal Polygraph]
\begin{definition} \label{def:universal-polygraph-enea}
  A \bfit{universal polygraph} $G = (V, E, C)$ (of weak isolation levels) associated with a history $\H = (\T, \SO)$
  is a directed labeled graph $(V, E)$ with relating keys called the \emph{known graph}
  together with a pair of constraints set $C$ of \emph{universal constraints}
  consisting of only a $\WR$ constraints set $\wrcons$
  such that
  \begin{itemize}
    \item $V$ corresponds to all transactions in the history $\H$;
    \item $E \subseteq V \times V \times \type \times \Key$ is a set of edges with labels (i.e., types)
    from \red{$\type = \set{\SO, \WR, \CO}$} and relating keys from $\Key$; and
    \item $C = \wrcons = \bset{\btuple{(T_1, S, \WR, \keyxvar), (T_2, S, \WR, \keyxvar), \ldots, (T_n, S, \WR, \keyxvar)}
          \mid S \vdash \readevent(\keyxvar, \valvar) \land
            \forall T \in \set{T_1, T_2, \ldots, T_n}.\; T \vdash \writeevent(\keyxvar, \valvar)}$.
  \end{itemize}
\end{definition}
%%%%%%%%%%%%%%%%%%%%

In Enea's definition, it's required to guess only \WR{} relations.
For RC, RA and TCC, there exists different characterizing rules of \CO{} based on instantiated \WR{} and known \SO.
\zhiheng{here we omit the definition of compatible graphs, that are almost the same as \ref{def:compatible-graphs-with-a-universal-polygraph}(except the non-existing $\wwcons$)}

%%%%%%%%%%%%%%%%%%%%
% [RW-Derive Property of a compatible graph]
\begin{definition} \label{def:co-derive-property}
  For some specific isolation levels $\I \in \set{RC, RA, TCC}$,
  a directed labeled graph with relating keys $G' = (V', E')$ satisfies \bfit{$\CODerive$ property $P(\I)$} if
  $G'$ satisfies corresponding axioms in \cite{Complexity:OOPSLA2019}.
\end{definition}
%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%
\begin{theorem}[Universal Polygraph-based Characterization of RC, RA and TCC] \label{thm:universal-polygraph-weak}
  A history $\H$ satisfies $\I \in \set{RC, RA, TCC}$ if and only if
  there exists a compatible graph $G'$ of the universal polygraph of $\H$ is acyclic and satisfies $P(\I)$.
\end{theorem}
%%%%%%%%%%%%%%%%%%%%
\zhiheng{Note this is not identical to SER and SI, maybe we should change the description of sec3.2}

==> sections/weak-isolation-upg.tex <==
% weak-isolation-upg.tex

\section{Characterizing Weak Isolation Levels}
\label{section:weak-isolation-upg}

\blue{[move this section to appendix]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{sections/si-upg}
\input{sections/tcc-upg}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tables/ablation-polarity.tex <==
% ablation-polarity.tex

\begin{wraptable}{right}{4.2cm}
		\vspace{-3ex}
%\begin{table}[h]
	\centering
			\captionsetup{skip=4pt}
	\caption{The number of conflicts encountered during solving w/ or w/o Optimization \textbf{H}.  } \label{table:conflicts-polarity}
			\footnotesize
	\begin{tabular}{ccc}
		% \hline
		\toprule
		Benchmark  & \ourtool & w/o \textbf{H} \\
	\midrule
    G-TPCC		 & 0    & 0    \\
		G-Twitter  & 79   & 99   \\
		G-RUBiS    & 89   & 246  \\
		RH         & 0    & 0    \\
		BL         & 50   & 497  \\
		WH         & 86   & 1427 \\
		HD         & 936  & 2047 \\
		\bottomrule
	\end{tabular}
%\end{table}
	\vspace{-2ex}
\end{wraptable}

==> tables/ablation.tex <==
% ablation.tex

\begin{table}[t]
	\centering
	\caption{Ablation analysis \red{in another order}} \label{table:ablation}
	\begin{tabular}{|c|c|c|c|c|}
		% \hline
		Benchmark  & \ourtool  & w/o \textbf{C} & w/o \textbf{C}\&\textbf{P} & w/o \textbf{C}\&\textbf{P}\&\textbf{H}   \\
		\hline
    G-TPCC     & 0.248   & 0.251    & 0.430       &  161.462      \\
		G-Twitter  & 1.104   & 1.014    & 72.935      &  TO (600)     \\
		G-RUBiS    & 3.453   & 7.801    & TO (600)    &  TO (600)     \\
		GeneralRH  & 0.940   & 0.683    & 2.474       &  119.080      \\
		GeneralRW  & 13.343  & 8.872    & TO (600)    &  TO (600)     \\
		GeneralWH  & 30.566  & 16.467   & TO (600)    &  TO (600)     \\
		GeneralDV  & 94.230  & 187.955  & TO (600)    &  TO (600)     \\
	\end{tabular}
\end{table}

==> tables/cycle-detection-ratio.tex <==
% cycle-detection-ratio.tex

\begin{table}[t]
	\centering
	\caption{Ratio of times of finding cycles and times of trying to find cycles } \label{table:find-cycle-ratio}
	\begin{tabular}{|c|c|}
		% \hline
		Benchmark  & Ratio \\
		\hline
    G-TPCC~\footnote{All constraints have been pruned for TPC-C~\cite{PolySI:VLDB2023,Cobra:OSDI2020}.}
		  & \diagbox[dir=NE]{}{} \\
		G-Twitter  & 7.44\%   \\
		G-RUBiS    & 3.90\%   \\
		GeneralRH  & 0        \\
		GeneralRW  & 0.10\%   \\
		GeneralWH  & 0.04\%   \\
		GeneralRV  & 0.05\%   \\
	\end{tabular}
\end{table}

==> tables/cycle-statistics-no-cycle-opt.tex <==
% cycle-statistics-no-cycle-opt.tex

\begin{table}
	\centering
			\captionsetup{skip=4pt}
	\caption{Statistics of PK algorithm in six representative histories \nobi{todo: reorg}} 
	\label{table:cycle-statistics}
	\resizebox{\columnwidth}{!}{%\scriptsize
	\begin{tabular}{ccccccc}
		% \hline
		\toprule
		Benchmark  & \#Calls to PK. &\#Traverse &\#Cycles Detected &\#Reorder & $|\wwcons \cup \wrcons|$ & \#Reorder / $|\wwcons \cup \wrcons|$ \\
		\midrule
    G-TPCC     & 13621916  & 4655   & 4061  & 594  & 39857 & 1.49\%   \\
		G-Twitter  & 26469     & 344    & 276   & 68   & 3635  & 1.87\%   \\
		G-RUBiS    & 234114    & 1399   & 878   & 521  & 4550  & 11.45\%  \\
		ready-heavy         & 521870    & 1054   & 423   & 631  & 8220  & 7.67\%   \\
		balanced         & 88963030  & 16401  & 14241 & 2160 & 31947 & 6.76\%   \\
	write-heavy         & 215366221 & 30056  & 26886 & 3170 & 53019 & 9.92\%   \\
		\bottomrule
	\end{tabular}
}
\end{table}

==> tables/cycle-statistics.tex <==
% cycle-statistics.tex

\begin{table}[t]
	\centering
	\caption{Statistics of PK algorithm in six representative histories} \label{table:cycle-statistics}
	\begin{tabular}{|c|c|c|c|}
		% \hline
		Benchmark  & \#Call PK algo. &\#Traverse &\#Detect a Cycle \\
		\hline
    G-TPCC     & 0     & 0    & 0     \\
		G-Twitter  & 35    & 9    & 2     \\
		G-RUBiS    & 1046  & 51   & 9     \\
		GeneralRH  & 92    & 28   & 0     \\
		GeneralRW  & 8880  & 256  & 44    \\
		GeneralWH  & 49376 & 420  & 104   \\
	\end{tabular}
\end{table}

==> tables/cycle-width.tex <==
% cycle-width.tex

\begin{table}[t]
	\centering
	\caption{Cycle count by width \red{after \textbf{H}}} \label{table:cycle-count-by-width}
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
		% \hline
		Benchmark  & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11   \\
		\hline
    G-TPCC     & 0 & & & & & & & & & &      \\
		G-Twitter  & 0 & 10 & 5 & 4 & & & & & & &    \\
		G-RUBiS    & 32 & 158 & 214 & 92 & 36 & 13 & & & & &   \\
		GeneralRH  & 3 & 24 & 43 & 22 & 12 & 1 & & & & &      \\
		GeneralRW  & 11 & 159 & 229 & 121 & 27 & 15 & 11 & 6 & 2 & 1 & 1     \\
		GeneralWH  & 40 & 426 & 612 & 339 & 103 & 49 & 11 & 3 & 1 & 1 & 1     \\
	\end{tabular}
\end{table}

==> tables/encoding-cycle-width-1234.tex <==
% encoding-cycle-width-1234.tex

\begin{table*}[t]
	\centering
	\caption{
		Encoding time of 1, 2, 3, and 4-width cycles (both for \ser and \si),
		\blue{where Veri. is the runtime of our baseline algo. with only Enc. 1 (Pruning), 
		Veri.2 is the runtime of baseline algo with only $\WW$ pruning~\cite{Cobra:OSDI2020}}
	} 
  \label{table:encoding-times-of-2-and-3-cycles}
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
		% \hline
		Benchmark  & Prune / Enc.1 (s) & Enc. 2 (s) & 2 vs 1 Slowdown ($\times$) & Enc. 3 (s) & 3 vs 2 Slowdown ($\times$) & Enc 4. (s) & 4 vs 3 Slowdown ($\times$) & Veri. (s) & Veri. 2 (s) \\
		\hline
		G-RUBiS    & 0.504 & 0.268 & - 0.47 & 100.738 & 374    & > 600        & > 5          & 10.628  & 5679.161  \\
		G-Twitter  & 0.283 & 0.179 & - 0.37 & 9.912   & 54     & > 600        & > 59         & 1.180   & 16.615    \\
		GeneralRH  & 0.236 & 0.212 & - 0.10 & 0.017   & - 0.92 & > 600        & > 352        & 0.694   & 4.303     \\
		GeneralRW  & 3.069 & 2.077 & - 0.32 & > 600   & > 287  & $\backslash$ & $\backslash$ & 21.101  & 142.930   \\
		GeneralWH  & 4.577 & 7.616 & 0.66   & > 600   & > 77   & $\backslash$ & $\backslash$ & 100.479 & 407.815   \\
		GeneralDV  & 3.060 & 7.758 & 1.54   & > 600   & > 76   & $\backslash$ & $\backslash$ & 456.276 & > 3h      \\
	\end{tabular}
\end{table*}

==> tables/encoding-cycle-width-23.tex <==
% encoding-cycle-width-23.tex

\begin{table}[t]
	\centering
	\caption{Encoding time of 2 and 3-width cycles} 
  \label{table:encoding-times-of-2-and-3-cycles}
	\begin{tabular}{|c|c|c|c|c|}
		% \hline
		Benchmark  & Enc. 2 (s) & Enc. 3 (s) & Slowdown ($\times$) & Veri. (s) \\
		\hline
		G-RUBiS    & 0.268  & 100.738 & 374    & 4.610   \\
		G-Twitter  & 0.179  & 9.912   & 54     & 1.528   \\
		GeneralRH  & 0.212  & 0.017   & -0.92  & 1.219   \\
		GeneralRW  & 2.077  & > 600   & >287   & 17.014  \\
		GeneralWH  & 7.616  & > 600   & >77    & 46.115  \\
		GeneralDV  & 7.758  & > 600   & >76    & 109.346 \\
	\end{tabular}
\end{table}

==> tables/reproduce.tex <==
% reproduce.tex

\begin{wraptable}{r}{4cm}
	\vspace{-3ex}
%\begin{table}
  \centering
    \captionsetup{skip=3pt}
  \caption{Avg. time on checking anomalous histories. We exclude timeout ones (900s). }
  \footnotesize
  \begin{tabular}{ccc}
    \toprule
    \textbf{Verifier} & 
    \textbf{SER} & 
    \textbf{SI} \\
    % & (CockroachDB) & (Galera) \\
    % & (disjoint writes) & (no constraints) & (disjoint writes) & (no constraints) \\
    \midrule
    Cobra      &   1293ms      &     --        \\ 
    PolySI     &     --           &   359ms     \\
    Viper      &       --       &     6559ms    \\
    dbcop      &   551ms       &   108ms     \\
    \ourtool   &   143ms       &   18ms      \\
    \midrule
    \textbf{\#histories} & 2073 & 434 \\
    \bottomrule
  \end{tabular}
  \label{table:reproduce-violations}
%\end{table}
		\vspace{-2ex}
\end{wraptable}


  % \begin{tabular}{ccc}
  %   \toprule
  %   \textbf{Verifier} & 
  %   \textbf{SER} & 
  %   \textbf{SI} \\
  %   % & (CockroachDB) & (Galera) \\
  %   % & (disjoint writes) & (no constraints) & (disjoint writes) & (no constraints) \\
  %   \midrule
  %   Cobra      &   2676.769s   &             \\ % SER: 2 TO
  %   PolySI     &               &   155.801s  \\
  %   Viper      &               &             \\
  %   dbcop      &   1130.238s   &   46.760s   \\ % SER: 4 TO
  %   \ourtool   &   297.042s    &   7.61s     \\
  %   \midrule
  %   \textbf{\#histories} & 2073 & 434 \\
  %   \bottomrule
  % \end{tabular}

==> tables/topo-init.tex <==
% topo-init.tex

\begin{table}[t]
	\centering
	\caption{Checking time ablation study on different initialization of pseudo-topo order} \label{table:pseudo-topo-init}
	\begin{tabular}{|c|c|c|c|c|}
		% \hline
		Benchmark  & by sess\_id & default & by sess\_id + \textbf{H} & default + \textbf{H} \\
		\hline
    G-TPCC     & 53.851   & 53.957   & 0.290  & 0.284  \\
		G-Twitter  & 0.136    & 0.134    & 0.037  & 0.037  \\
		G-RUBiS    & 0.539    & 0.535    & 0.220  & 0.227  \\
		GeneralRH  & 0.745    & 0.735    & 0.160  & 0.168  \\
		GeneralRW  & 304.847  & 304.001  & 15.342 & 12.094  \\
		GeneralWH  & 1042.301 & 1038.471 & 39.837 & 34.441  \\
	\end{tabular}
\end{table}
